Private DNA Sequencing: Hiding Information in Discrete Noise

When an individual's DNA is sequenced, sensitive medical information becomes available to the sequencing laboratory. A recently proposed way to hide an individual's genetic information is to mix in DNA samples of other individuals. We assume that the genetic content of these samples is known to the individual but unknown to the sequencing laboratory. Thus, these DNA samples act as "noise" to the sequencing laboratory, but still allow the individual to recover their own DNA samples afterward. Motivated by this idea, we study the problem of hiding a binary random variable $X$ (a genetic marker) with the additive noise provided by mixing DNA samples, using mutual information as a privacy metric. This is equivalent to the problem of finding a worst-case noise distribution for recovering $X$ from the noisy observation among a set of feasible discrete distributions. We characterize upper and lower bounds to the solution of this problem, which are empirically shown to be very close. The lower bound is obtained through a convex relaxation of the original discrete optimization problem, and yields a closed-form expression. The upper bound is computed via a greedy algorithm for selecting the mixing proportions.

==> additional_results.tex <==
\section{Additional Comments}

\begin{lemma} 
	For any $K \in \mathbb{N}, p \in [0, 0.5],$ we have that 
	\begin{align} 
	& I(X \; ; \; X + \sum_{i=1}^K Y_i) \\
	& = H(p) - \sum_{i=0}^{K-1} p^{K-i} (1-p)^{i+1} \binom{K+1}{i+1} H \left(\frac{i+1}{K+1}\right).
	\end{align}
\end{lemma}

\begin{lemma}
	For any $K \in \mathbb{N},$  $p = c(1 - e^{-\frac{1}{K+1}}),$ and $L \in \mathbb{N}$ such that $L \leq K$ and $c \in \mathbb{R}, \; \; 0 \leq c \leq 1,$ we have that 
	\begin{align} 
	& I(X \; ; \; X + \sum_{i=1}^K Y_i)
	\\ & \leq c \left( \frac{1}{K+1} \right) \log\left(c \left(K+2 \right) \right) 
	\\ & + \left( \frac{K+2-c}{K+2} \right) \log\left(\frac{K+1}{K+1-c} \right)
	\\ & - c\left( \frac{K-L+2}{K+2} \right)^{L} \left( \frac{1}{K+1} \right) \log \left( \frac{K+1}{L} \right) 
	\\ & \times \left(1 - \frac{c}{K+1} \right)^{K} e^c \left(1 - \frac{1}{\sqrt{2 \pi L}}  \left(\frac{ce}{L}\right)^L \right)   
	\end{align}
\end{lemma}

Substituting $L = \ln(K)$ into the bound above, we have that 

Thus, the perfomance of the uniform scheme is upper bounded by  
\begin{align}
&  c \left( \frac{1}{K+1} \right) \log\left(c \left(K+2 \right) \right) 
\\ & + \left( \frac{K+2-c}{K+2} \right) \log\left(\frac{K+1}{K+1-c} \right)
\\ & - c\left( \frac{K-\ln(K)+2}{K+2} \right)^{\ln(K)} \left( \frac{1}{K+1} \right) \log \left( \frac{K+1}{\ln(K)} \right) 
\\ & \left(1 - \frac{c}{K+1} \right)^{K} e^c \left(1 - \frac{1}{\sqrt{2 \pi \ln(K)}}  \left(\frac{ce}{\ln(K)}\right)^{\ln(K)} \right)  
\\ & \sim \frac{c\ln(\ln(K))}{\ln(2)K}
\end{align}

We also have the lower bound at $p = c (1 - e^{-\frac{1}{K+1}})$ is given by 
\begin{align}
& -\left(1 - c(1 - e^{-\frac{1}{K+1}}) \right)^{K+1} \log(1 - c(1 - e^{-\frac{1}{K+1}}))
\\ & - \left(1 - c(1 - e^{-\frac{1}{K+1}}) \right)^{K+1} \log(1 - (1 - c(1 - e^{-\frac{1}{K+1}}))^K)
\\ & + \left(1 - c(1 - e^{-\frac{1}{K+1}}) \right)^{K+1} \log(1 - (1 - c(1 - e^{-\frac{1}{K+1}}))^{K+1})
\\ & + \left(1 - c(1 - e^{-\frac{1}{K+1}}) \right) \log(1 - \left(1 - c \left(1 - e^{-\frac{1}{K+1}} \right) \right)^{K})
\\ & -\log(1 - (1 - c(1 - e^{-\frac{1}{K+1}}))^{K+1})
\\ & \sim \frac{c e^{-c}}{K \ln(2)}
\\ & - \frac{(c-3)c e^{-c}}{2(e^c-1)K \ln(2)} + \frac{(c-1)c e^{-c} \ln(1 - e^{-c})}{2K \ln(2)} 
\\ & + \frac{(c-1)c e^{-c}}{2(e^c-1)K \ln(2)}  - \frac{(c-1)c e^{-c} \ln(1-e^{-c})}{2K \ln(2)} 
\\ & - \frac{c \ln(1 - e^{-c})}{K \ln(2)}  + \frac{(c-3)c}{2(e^c-1)K \ln(2)}
\\ & - \frac{(c-1)c}{2(e^c-1)K \ln(2)}
\\ & = \Theta \left( \frac{1}{K} \right)
\end{align}

This proves that the ratio between the performance of the uniform scheme and the lower bound for $p = c(1 - e^{-\frac{1}{K+1}})$ is upper bounded by a function that is $O(\ln(\ln(K)))$ for $0 \leq c \leq 1.$


==> concluding_remarks.tex <==
\section{Concluding Remarks}

%In this paper, we considered the problem of hiding the an individual's allele at a single biallelic site during the sequencing process.  

%Following the solution introduced in \cite{Maddah-Ali}, we studied how to best choose the proportion of each individual's DNA in a mixture.  


\iscomment{we should probably remove this section. it feels out of place out of so much discussion}

We derived a lower bound on the best possible mutual information achievable by a private DNA sequencing scheme, and showed that it is tight by comparing it with the scheme generated by a greedy algorithm. Directions  for follow-up work include considering multiple, possibly correlated, genetic loci simultaneously, and  characterizing the optimal tradeoffs between privacy and the ability to correctly recover the genotype $X$ from the data received from the lab.

==> introduction10_13_20.tex <==
% !TEX root = main.tex


\section{Introduction}


Advances in DNA sequencing technologies have led to the generation of human genetic data at an unprecedented rate \cite{astronomical}. 
This offers exciting prospects for biomedical research, and recent studies have leveraged the genetic data of hundreds of thousands of individuals to identify genetic markers associated with many traits and diseases \cite{cad,diabetes,alzheimer,cirulli_rare}.

% While the widespread availability of genetic testing for several diseases \cite{diseaserisk} and the popularization of direct-to-consumer genomics services \cite{23andme,ancestry} can provide 

Genetic testing for disease predisposition \cite{diseaserisk} and popular direct-to-consumer genomics services \cite{directtoconsumer,directtoconsumer2} can provide us with  important and actionable information about our health. 
However, these services require the submission of a blood or saliva sample, making an individual's entire DNA available to the testing center.
This raises significant privacy concerns surrounding genetic data \cite{erlich}, particularly regarding the potential use of this information by insurance companies \cite{23andmepharma}.


Given the potential privacy risks of DNA sequencing, an important question is whether it is possible to alter a physical DNA sample prior to submitting it to a laboratory, in order to ``hide'' some of its genetic information.
% for sequencing.
One possible way to alter a sample could be to 
% achieve this would be to 
\emph{mix} it with the DNA of other individuals.
% Since most labs utilize shotgun sequencing technologies \cite{illumina}, 
Upon sequencing, the lab would then observe 
% The sequencing data will then correspond to 
a mixture of 
the data from the different samples, 
% all the genetic variants,
% of all individuals in the mixture, 
which would hinder its ability to retrieve individual genetic variants.
% effectively ``hiding'' the genetic variants of each individual from the lab.

The general idea of mixing samples to attain genetic privacy
% , together with a framework to analyze its theoretical guarantees, 
was proposed in \cite{Maddah-Ali} (and later extended in \cite{Maddah-Ali2}).
Suppose Alice wants to have her DNA
sequenced and has at her disposal the
% Suppose a person A wishes to have their DNA sequenced and has at their disposal 
DNA samples of $K$ other people
% persons B and C, 
who \emph{already know} their DNA sequence.
Alice can then mix all $K+1$ DNA samples and send them to the sequencing lab.
From the lab's perspective, the DNA of the $K$ additional individuals plays the role of noise, impairing the lab's ability to recover Alice's DNA.
However, upon receiving the sequencing data back, the contribution of the ``noise individuals'' can be removed, and Alice can recover her DNA sequence information.
\iscomment{need to mention figure}

% Then, the 
% DNA of persons B and C, when added to the DNA of person A, plays the role of noise, impairing the lab's ability to retrieve
% by submitting a mixture of the three DNA samples, noise is effectively 


% In this paper, we consider this framework 
% from \cite{Maddah-Ali,Maddah-Ali2} 
Motivated by this idea, 
we study how to \emph{optimally mix} DNA samples in order to maximize the privacy achieved.
We focus on a single \emph{biallelic site} $s$ on the genome; i.e., a location on the human genome that admits two possible alleles\footnote{\rdcomment{this is a big part of justifying the model, so i prefer it get more discussion; perhaps even promote it out of a footnote. proposed change: Many mutations and disease indicators can be identified by a presence/absence of a single allele. For example, TODO. In future work, we hope to generalize these results to sequences of coupled biallelic sites.}This could model, for example, the presence of the mutation on the BRCA2 gene that increases the likelihood of breast cancer \cite{brca}}, and can thus be modeled as a single variable $X \in \{-1,+1\}$.
% The allele frequency in
In order to hide her value of $X$ from the sequencing lab, Alice mixes into her sample the samples of $K$ individuals with amounts $\alpha_1,...,\alpha_K$.
% Following \cite{Maddah-Ali}, we a
We model the lab's observation of site $s$ as
$Y = X + \sum_{i=1}^K \alpha_i Z_i$,
where $Z_i \in \{-1,1\}$ is the allele value of the $i$th noise individual.
This is motivated by the fact that, if the lab uses shotgun sequencing technologies \cite{illumina}, each reading of site $s$ is effectively a $\Ber\left(Y/(1+\sum \alpha_i)\right)$ random variable \iscomment{only if $X \in \{0,1\}$}.
Via repeated readings of $s$, $Y$ can thus be obtained with arbitrary accuracy, so we assume for simplicity that $Y$ is observed exactly.
We refer to the long version of this manuscript \cite{privateDNAlong} for a more detailed discussion on this model.

% Assuming that the lab uses a shotgun sequencing technology, which randomly samples pieces of DNA from the mixture and reads them, 
% we model its observation as 


% the lab will observe, in expectation,
% Then, when probing the genomic



Following \cite{Maddah-Ali}, we model $X,Z_1,...,Z_K$ as i.i.d.~random 
variables with $\Pr(X=1) = p \in [0,0.5]$.
We refer to $p$ as the minor allele frequency, a parameter that is known in practice for genetic loci of interest.
As in \cite{Maddah-Ali}, 
we utilize the mutual information as our privacy metric.
% and we seek to solve
Our goal is to solve 
\al{
\min_{\alpha_1,...,\alpha_K} I\left(X;X+\sum_{k=1}^K \alpha_k Z_k\right),
\label{eq:main}
}
i.e., choose the mixing coefficients $\alpha_1,...,\alpha_K \geq 0$ to minimize the mutual information between $X$ and the lab's observation.
% the privacy level is captured by the mutual informaiton between $X$ and 

\rdcomment{i would like more privacy interpretation here. for example, comment on the adversary's information recovery problem. in particular, as a reader, i imagine many questions. "are the alphas known by the adversary?" we don't need to go into to much detail, but here is where we would usually place some discussion on privacy and the adversary}

\rdcomment{re: worst case distribution. same note as in the intro: let's connect it to privacy here again}

This problem can be thought of as characterizing a worst-case noise distribution among those of the form $Z = \sum_k \alpha_k Z_k$, with $Z_k$ being i.i.d.~$\Ber(p)$.
Our main result is that the solution to (\ref{eq:main}) is well approximated as 
\al{
\min_{\alpha_1,...,\alpha_K} I\left(X;X + Z\right)
\approx I\left(X;X - 2G\right),
}
where $G \sim \Geom\left( (1-p)^K \right)$ and $G$ is independent of $X$.
This result is surprising given that it is not possible in general to choose $\alpha_1,...,\alpha_K$ so that $Z_\alpha \sim \Geom\left( (1-p)^K \right)$.

\rdcomment{when i read this part, the emotions i feel are skeptical, unsure, confused, and, as a result, mildly frustrated. it's not too big of a deal, but i think the "approx" part feels too vague to me at this point, so i prefer some foreshadowing. (in particular, you run the risk of a reader making up one set of expectations and being irrationally unhappy when these expectations are not met. my personal advice for writing these things is to always be calibrating and controlling the reader's expectations) proposed change: more details as to exactly what approx means, e.g.we say approx in the sense that the this mutual information serves as a lower bound and is very very close to an upper bound. (can we quantify how close it is to the upper bound?) maybe even say "a more formal statement of this is in Theorem 1" or something.}

To establish this result, we introduce a continuous (and convex) relaxation of (\ref{eq:main}), and formally show that $I\left(X;X - 2G\right)$ is a lower bound to the discrete optimization problem.
This lower bound is then empirically shown to be very close a greedy solution to (\ref{eq:main}), which chooses $\alpha_1,...,\alpha_K$ sequentially, to minimize the resulting mutual information.




% The simple nature of the random variables involved and the symmetry between the different variables $\alpha_i$ may suggest that the solution to the optimization problem in (\ref{eq:main}) is straightforward.
% However, as we will disc


% This models the fact that the prevalence of each allele in the population is typically known

% i.e., the known prevalence of the rare allele in the overall population \cite{minorallele}.

% Suppose a person wants to have their value of $X$ sequenced and has at their disposal 
% Suppose a person A wishes to have their DNA sequenced and has at their disposal 
% DNA samples of $K$ other people
% persons B and C, 
% who \emph{already know} their DNA sequence.
% Then, the DNA of persons B and C, when added to the DNA of person A, plays the role of noise, impairing the lab's ability to retrieve
% by submitting a mixture of the three DNA samples, noise is effectively 






% While the availability of public genetic databases (such as the UK Biobank \cite{ukbiobank} and gnomAD \cite{gnomad}) and the free exchange of information among research groups can accelerate the rate of biomedical findings, the indiscriminate sharing of genetic information raises significant concerns regarding the privacy of personal information \cite{erlich}. 


% The widespread adoption of DNA sequencing technologies is rapidly changing the landscape of modern biology and medicine.
% The consequences of this revolution are felt by society at large with the increasing availability of
% genetic testing for several diseases \cite{diseaserisk}, prenatal genetic screening \cite{prenatal}, and direct-to-consumer services such as 23andMe and Ancestry \cite{directtoconsumer,directtoconsumer2}.
% But despite all the excitement surrounding these applications, there are still several misconceptions about genetics \cite{hogarth2010myths} and 
% concerns about data privacy and unethical uses of personal genetic information \cite{ethics1,ethics2,ethics3,23andmepharma}.



% Studies have shown that surnames can be accurately inferred from personal genomes [8]. 
% Privacy can be compromised even when only aggregate statistics such as allele frequencies are made public [9], which led the National Institutes of Health (NIH) to move summary statistics data to access-controlled databases like dbGaP [10]. 









\begin{figure}\label{fig:overview}
	\centering
	\includegraphics[width=0.75\linewidth]{Overview}
	\caption{A high level diagram of the problem \rdcomment{my personal style is that the caption describes the figure in a fashion that it can be understood without reading the text in the body. i am not sure if IS agrees with this though. either way, i think this caption needs a little polishing.}}
	\label{fig:Overview}
\end{figure}

==> introduction10_19_20.tex <==
% !TEX root = main.tex


\section{Introduction}


Advances in DNA sequencing technologies have led to the generation of human genetic data at an unprecedented rate \cite{astronomical}. 
This offers exciting prospects for biomedical research, and recent studies have leveraged the genetic data of hundreds of thousands of individuals to identify genetic markers associated with many traits and diseases \cite{cad,diabetes,alzheimer,cirulli_rare}.

% While the widespread availability of genetic testing for several diseases \cite{diseaserisk} and the popularization of direct-to-consumer genomics services \cite{23andme,ancestry} can provide 

Genetic testing for disease predisposition \cite{diseaserisk} and popular direct-to-consumer genomics services \cite{directtoconsumer,directtoconsumer2} can provide us with  important and actionable information about our health. 
However, these services require the submission of a blood or saliva sample, making an individual's entire DNA available to the testing center.
This raises significant privacy concerns surrounding genetic data \cite{erlich}, particularly regarding the potential use of this information by insurance companies \cite{23andmepharma}.


Given the potential privacy risks of DNA sequencing, an important question is whether it is possible to alter a physical DNA sample prior to submitting it to a laboratory, in order to ``hide'' some of its genetic information.
% for sequencing.
One possible way to alter a sample could be to 
% achieve this would be to 
\emph{mix} it with the DNA of other individuals.
% Since most labs utilize shotgun sequencing technologies \cite{illumina}, 
Upon sequencing, the lab would then observe 
% The sequencing data will then correspond to 
a mixture of 
the data from the different samples, 
% all the genetic variants,
% of all individuals in the mixture, 
which would hinder its ability to retrieve individual genetic variants.
% effectively ``hiding'' the genetic variants of each individual from the lab.

The general idea of mixing samples to attain genetic privacy
% , together with a framework to analyze its theoretical guarantees, 
was proposed in \cite{Maddah-Ali} (and later extended in \cite{Maddah-Ali2}).
Suppose Alice wants to have her DNA
sequenced and has at her disposal the
% Suppose a person A wishes to have their DNA sequenced and has at their disposal 
DNA samples of $K$ other people
% persons B and C, 
who \emph{already know} their DNA sequence.
Alice can then mix all $K+1$ DNA samples and send them to the sequencing lab.
From the lab's perspective, the DNA of the $K$ additional individuals plays the role of noise, impairing the lab's ability to recover Alice's DNA.
However, upon receiving the sequencing data back, the contribution of the ``noise individuals'' can be removed, and Alice can recover her DNA sequence information.
This approach is illustrated in Figure~\ref{fig:Overview}.

% Then, the 
% DNA of persons B and C, when added to the DNA of person A, plays the role of noise, impairing the lab's ability to retrieve
% by submitting a mixture of the three DNA samples, noise is effectively 


% In this paper, we consider this framework 
% from \cite{Maddah-Ali,Maddah-Ali2} 
Motivated by this idea, 
we study how to \emph{optimally mix} DNA samples in order to maximize the privacy achieved.
We focus on a single \emph{biallelic site} $s$ on the genome; i.e., a location on the human genome that admits two possible alleles, and can thus be modeled as a single variable $X \in \{0,1\}$.
This could model, for example, the presence of the mutation on the BRCA2 gene that increases the likelihood of breast cancer \cite{brca} and many other disease genetic markers.
% \footnote{\rdcomment{this is a big part of justifying the model, so i prefer it get more discussion; perhaps even promote it out of a footnote. proposed change: Many mutations and disease indicators can be identified by a presence/absence of a single allele. For example, TODO. In future work, we hope to generalize these results to sequences of coupled biallelic sites.}This could model, for example, the presence of the mutation on the BRCA2 gene that increases the likelihood of breast cancer \cite{brca}}
% The allele frequency in
\iscomment{mention diploid in long}



\begin{figure}[b]
	\centering
	\includegraphics[width=0.77\linewidth]{data/alice_fig.pdf}
	\caption{
	In order to hide her genotype $X$ at a given locus $s$, Alice mixes her DNA sample with that of $K$ individuals in amounts $\alpha_1,...,\alpha_K$.
	Upon receiving the sequencing data from the lab, Alice can remove the contribution from the ``noise individuals'' (whose genotype at $s$ is known) to recover $X$.
% 	A high level diagram of the problem 
% 	\rdcomment{my personal style is that the caption describes the figure in a fashion that it can be understood without reading the text in the body. i am not sure if IS agrees with this though. either way, i think this caption needs a little polishing.}
	}
	\label{fig:Overview}
\end{figure}


In order to hide her genotype $X$ from the sequencing lab, Alice mixes into her sample the samples of $K$ individuals using proportions $\alpha_0,\alpha_1,...,\alpha_K$, where $\sum_{i=0}^K \alpha_i = 1$.
% Following \cite{Maddah-Ali}, we a
We model the lab's observation of site $s$ as
$Y = \alpha_0 X + \sum_{i=1}^K \alpha_i Z_i$,
where 
$Z_i \in \{0,1\}$ is the allele value of the $i$th noise individual.
This is motivated by the fact that, if the lab uses shotgun sequencing technologies \cite{illumina}, each reading of site $s$ is effectively a $\Ber\left(\alpha_0 X + \sum_{i=1}^K \alpha_i Z_i\right)$ random variable.
Via repeated readings of $s$, $Y$ can thus be obtained with arbitrary accuracy, so we assume for simplicity that $Y$ is observed exactly.
We refer to the long version of this manuscript \cite{privateDNAlong} for a more detailed discussion on this model.

% Assuming that the lab uses a shotgun sequencing technology, which randomly samples pieces of DNA from the mixture and reads them, 
% we model its observation as 


% the lab will observe, in expectation,
% Then, when probing the genomic



Following \cite{Maddah-Ali}, we model $X,Z_1,...,Z_K$ as i.i.d.~random 
variables with $\Pr(X=0) = p \in [0,0.5]$.
\kmcomment{I changed this to $\Pr(X=0) = p $ since we have been using $0$ as minor allele}
We refer to $p$ as the minor allele frequency, a parameter that is known in practice for genetic loci of interest.
As in \cite{Maddah-Ali}, 
we utilize the mutual information as our privacy metric.
% and we seek to solve
If we let $\alpha = (\alpha_0,...,\alpha_K)$ and $Z_\alpha = \sum_{k=1}^K \alpha_k Z_k$, our goal is thus to solve
% Our goal is to solve 
\al{
% \min_{\alpha \in \R_+^K} 
\min_{\alpha} 
I\left( X; \alpha_0X+Z_\alpha\right),
\label{eq:main}
}
i.e., choose the mixing coefficients $\alpha_0,...,\alpha_K$ to minimize the mutual information between $X$ and the lab's observation.  
% the privacy level is captured by the mutual information between $X$ and 


The problem in (\ref{eq:main}) is equivalent to maximizing the conditional entropy $H(X|Y)$; i.e., the residual uncertainty in $X$ after observing $Y = \alpha_0 X+Z_\alpha$, and can thus be understood as maximizing the privacy of $X$.
% \rdcomment{i would like more privacy interpretation here. for example, comment on the adversary's information recovery problem. in particular, as a reader, i imagine many questions. "are the alphas known by the adversary?" we don't need to go into to much detail, but here is where we would usually place some discussion on privacy and the adversary}
% \rdcomment{re: worst case distribution. same note as in the intro: let's connect it to privacy here again}
It can also be thought of as the problem of finding a worst-case noise $Z_\alpha$ among those of the form $\sum_k \alpha_k Z_k$, with $Z_k$ being i.i.d.~$\Ber(p)$.
Our main result is that the solution to (\ref{eq:main}) is 
lower-bounded as
% well approximated as 
\al{
\min_{\alpha} I\left(X;\alpha_0 X + Z_\alpha\right)
\geq I\left(X;X - G\right),
\label{eq:lower}
}
where $G \sim \Geom\left( (1-p)^K \right)$ and $G$ is independent of $X$.
The right-hand side of (\ref{eq:lower}) can be computed explicitly as a function of $p$ and $K$.
Moreover, we verify empirically that this lower bound is very close to an upper bound provided by a greedy algorithm that selects $\alpha_1,\alpha_2,...,\alpha_K$ sequentially to minimize the resulting mutual information, establishing $I\left(X;X - G\right)$ as a good approximation to the solution of (\ref{eq:main}).
% This result is surprising given that it is not possible in general to choose $\alpha_1,...,\alpha_K$ so that $Z_\alpha \sim \Geom\left( (1-p)^K \right)$.
% \rdcomment{when i read this part, the emotions i feel are skeptical, unsure, confused, and, as a result, mildly frustrated. it's not too big of a deal, but i think the "approx" part feels too vague to me at this point, so i prefer some foreshadowing. (in particular, you run the risk of a reader making up one set of expectations and being irrationally unhappy when these expectations are not met. my personal advice for writing these things is to always be calibrating and controlling the reader's expectations) proposed change: more details as to exactly what approx means, e.g.we say approx in the sense that the this mutual information serves as a lower bound and is very very close to an upper bound. (can we quantify how close it is to the upper bound?) maybe even say "a more formal statement of this is in Theorem 1" or something.}
We derive our lower bound via a convex relaxation of (\ref{eq:main}), and 
use the KKT conditions to show that its solution is given by
% formally show that 
$I\left(X;X - G\right)$.
\kmcomment{I guess we don't formally show that the solution to the infinite dimensional relaxation is $- G$}
% is a lower bound to the discrete optimization problem.
% This lower bound is then empirically shown to be very close a greedy solution to (\ref{eq:main}), which chooses $\alpha_1,...,\alpha_K$ sequentially, to minimize the resulting mutual information.




% The simple nature of the random variables involved and the symmetry between the different variables $\alpha_i$ may suggest that the solution to the optimization problem in (\ref{eq:main}) is straightforward.
% However, as we will disc


% This models the fact that the prevalence of each allele in the population is typically known

% i.e., the known prevalence of the rare allele in the overall population \cite{minorallele}.

% Suppose a person wants to have their value of $X$ sequenced and has at their disposal 
% Suppose a person A wishes to have their DNA sequenced and has at their disposal 
% DNA samples of $K$ other people
% persons B and C, 
% who \emph{already know} their DNA sequence.
% Then, the DNA of persons B and C, when added to the DNA of person A, plays the role of noise, impairing the lab's ability to retrieve
% by submitting a mixture of the three DNA samples, noise is effectively 






% While the availability of public genetic databases (such as the UK Biobank \cite{ukbiobank} and gnomAD \cite{gnomad}) and the free exchange of information among research groups can accelerate the rate of biomedical findings, the indiscriminate sharing of genetic information raises significant concerns regarding the privacy of personal information \cite{erlich}. 


% The widespread adoption of DNA sequencing technologies is rapidly changing the landscape of modern biology and medicine.
% The consequences of this revolution are felt by society at large with the increasing availability of
% genetic testing for several diseases \cite{diseaserisk}, prenatal genetic screening \cite{prenatal}, and direct-to-consumer services such as 23andMe and Ancestry \cite{directtoconsumer,directtoconsumer2}.
% But despite all the excitement surrounding these applications, there are still several misconceptions about genetics \cite{hogarth2010myths} and 
% concerns about data privacy and unethical uses of personal genetic information \cite{ethics1,ethics2,ethics3,23andmepharma}.



% Studies have shown that surnames can be accurately inferred from personal genomes [8]. 
% Privacy can be compromised even when only aggregate statistics such as allele frequencies are made public [9], which led the National Institutes of Health (NIH) to move summary statistics data to access-controlled databases like dbGaP [10]. 











==> main_proof10_18_20.tex <==


\section{Proof of Theorem~\ref{thm:main_lower_bound}}

% We now present the proof of Theorem \ref{thm:main_lower_bound}.  
\iscomment{No need for the proof environment here}

% \begin{IEEEproof}
%First, notice that choosing integral $\alpha_i \; : \;  i \in [K] \cup \{0\}$ in the optimization problem (\ref{eq:main}) is optimal due to Lemma \ref{lem:integer_sol_optimal}, which holds because scaling the $\alpha_i$'s does not change the mutual information.  
%Lemma \ref{lem:integer_sol_optimal} holds because if $\alpha_i = \frac{c_i}{b_i} \; \forall i$ in (\ref{eq:main}) where $c_i, b_i$ are integral, then the solution $\alpha_i = \frac{c_i}{b_i} \left(\Pi_j b_j\right) \; \forall i$ is integral and the mutual information is preserved. 
%We will thus consider (\ref{eq:main}) with the constraint that $\alpha_i \in \mathbb{N}$ for $i \in [K] \cup \{0\}.$

% \begin{lemma}
%     \label{lem:integer_sol_optimal}
%     If an optimal solution to (\ref{eq:main}) exists, then there exists an optimal solution to (\ref{eq:main}) with $\alpha_i \in \mathbb{N}$ for $i \in [K] \cup \{0\}.$
% \end{lemma}

%Let $ Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i.$ 
We obtain the lower bound on $I(X \, ; \, \alpha_0 X + Z_{\alpha})= H(p) - H(X \, | \, \alpha_0 X+Z_{\alpha})$ in Theorem~\ref{thm:main_lower_bound} by finding a lower bound on $-H(X \, | \, \alpha_0 X+Z_{\alpha}).$  The optimization problem we consider is therefore
\begin{align}
   \label{eq:integral_alpha_opt_prob}
    & \min_{\alpha_0,...,\alpha_K \in \mathbb{N}} -H\left(X \; \left| \; \alpha_{0} X+\sum_{k=1}^K \alpha_k Z_k \right. \right).
\end{align}
Observe that the pmf of the random variable $Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i$ has probability $(1-p)^{K}$ at its highest support value. 
More precisely, $\sum_{i=1}^k \alpha_K$ is the maximum value that $Z_\alpha$ can take, which occurs with probability $(1-p)^{K}$.
% Furthermore, we notice that adding a constant to $Z_\alpha$ does not 
% the following problem is clearly 
A relaxation to (\ref{eq:integral_alpha_opt_prob}) can be then obtained by ignoring all constraint on the pmf of $Z_\alpha$ except for the maximum pmf value.
Thus, for a fixed value of $\alpha_0$, a relaxation to (\ref{eq:integral_alpha_opt_prob}) is given by
\begin{align}
   \label{eq:relax_inf1}
    \min_{Q} \; &  -H\left(X \; | \; \alpha_0 X+Q\right)
    \\\text{subject to:} \; & 
    \nonumber 
    % \\ 
    Q \text{ is an integer-valued random variable} \nonumber
    \\ & \text{$Q$ is independent of $X$} \nonumber
    % \nonumber \\ & D  \text{ has maximum support value at 0} 
    \\ & \Pr(Q = 0) = (1-p)^K \nonumber
    \\ & \Pr(Q = i) = 0 \; \text{ for $i > 0$}.
    \nonumber
\end{align}
\iscomment{Should we use $Q$ instead of $Q$ to match pmf?}
Notice that the last constraint is equivalent to saying that $0$ is the maximum value of $Q$.
This can be assumed without loss of generality, since adding a constant to $Q$ does not change the value of $H(X\,|\,\alpha_0X+Q)$.
Furthermore, as we prove in Appendix~\ref{app:alpha0}, 
% Due to Lemma \ref{lem:alpha0_condition}, 
fixing $\alpha_0 = 1$ in (\ref{eq:relax_inf1}) above 
does not change the optimal value, and we assume throughout that $\alpha_0=1$.
    
% without changing the optimal value.  

Let $q_{(i)}$ be the pmf of $Q$; i.e., $q_{(i)} = \Pr(Q=i)$ for $i \leq 0$.
% In o
% Let $q_{(0)}$ be the probability at the maximum support value of $D$ and let $q_{(-i)}$ be the probability at the $i$th integer below the maximum support value of $D.$ 
In order to write (\ref{eq:relax_inf1}) explicitly in terms of $q$, we define 
% g_j(q) = P(X+D=j+1)*H(X|X+D=j+1). 
\begin{align}
    g_j(q) & \triangleq -H(X|X+Q=j+1)\Pr(X+Q=j+1) \nonumber \\
    & =  \Pr(Q+X=j+1)  \nonumber \\
    & \quad \times \bigg[ \frac{(1-p)q_{(j)}}{\Pr(Q+X=j+1)} \log\left(\frac{(1-p)q_{(j)}}{\Pr(Q+X=j+1)}\right) \nonumber \\       &  \quad + \frac{p q_{(j+1)}}{\Pr(Q+X=j+1)} \log\left(\frac{p q_{(j+1)}}{\Pr(Q+X=j+1)}\right) \bigg] \nonumber \\   
    % & =  \Pr(Q+X=j+1)  \nonumber \\
    % & \times \bigg(\frac{\Pr(Q=j)(1-p)}{\Pr(Q+X=j+1)} \log\left(\frac{\Pr(Q=j)(1-p)}{\Pr(Q+X=j+1)}\right) \nonumber \\       &  + \frac{\Pr(Q=j+1)p}{\Pr(Q+X=j+1)} \log\left(\frac{\Pr(Q=j+1)p}{\Pr(Q+X=j+1)}\right) \bigg) \nonumber \\   
    % & = q_{(j)}(1-p) \log\left(\frac{q_{(j)}(1-p)}{\Pr(Q+X=j+1)}\right) \nonumber \\       &  + q_{(j+1)}p \log\left(\frac{q_{(j+1)}p}{\Pr(Q+X=j+1)}\right) \nonumber \\   
    & = (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
    \nonumber 
    \\ & \quad + p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right).
\end{align}
Written in terms of $g_j(q)$ and with $\alpha_0 = 1$, (\ref{eq:relax_inf1}) is given by
\begin{align}
\label{eq:relax_inf2}
\min_{q_{(-i)} \geq 0 : \; i \in \mathbb{N}\cup\{0\} } \; & \sum_{j \in \{-n : \; n \in \mathbb{N}\}} g_j(q)
\\ \text{subject to:} \; & \quad q_{(0)} = (1-p)^K \nonumber \\ &  \quad    \sum_{j=0}^\infty q_{(-j)} = 1. \nonumber
\end{align}  
Note that the conditional entropy in the objective function is in a simplified form.   
\iscomment{What does this mean?}

\iscomment{I rewrote the following a bit:}

Observe that (\ref{eq:relax_inf2}) is a convex minimization problem with an infinitely many variables.  
For such problems, to the best of our knowledge, a solution to the KKT conditions is not in general guaranteed to yield an optimal solution.
For that reason, we do not seek to directly solve the KKT conditions.
Instead, we first consider a \emph{support-constrained} version of (\ref{eq:relax_inf2}, where the support of the pmf of $Q$ is restricted to $\{-n,...,0\}$, and then consider letting $n \to \infty$.
% 
% A solution to the KKT conditions with the added implicit constraint that $q_{(-i)}>0$ for $i \in \mathbb{N} \cup \{0\}$  is given by  $q_{(-i)} = (1-p)^K (1 - (1-p)^K)^i$ for $i \in \mathbb{N} \cup \{0\}$ 
% \iscomment{Is this obvious?}
% which corresponds to $D = -G$ in (\ref{eq:relax_inf1}) where $G$ is a geometric random variable with success probability equal to $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\}$.  
% We do not use this observation directly to establish Theorem \ref{theorem:main_recursion} because no reference on the relation between KKT conditions and optimality in the infinite dimensional case was found.  
% 
% Instead, we constrain $D$ to have distance no greater than $n \in \mathbb{N}$ between its maximum and minimum support values in (\ref{eq:relax_inf2}), derive a lower bound on the solution for each $n \in \mathbb{N},$ and use the resulting sequence of lower bounds to establish the result. 
The support-constrained version of (\ref{eq:relax_inf2}) is given by 
\begin{align}
\label{eq:relax_const}
\min_{q_{(i)} \geq 0 : \; i \in \{-n,...,0\} } \; & 
\sum_{j \in \{-m : \; m \in [n+1]\}} g_j(q) \\  \text{subject to:}  \; &  
q_{(0)} = (1-p)^K, \quad q_{(-n-1)} = 0 \nonumber \\
\quad & \; \sum_{j} q_{(j)} = 1. \nonumber
\end{align}  
\iscomment{say this is no longer a relaxation}

Changing the implicit constraint in (\ref{eq:relax_const}) from $q_{(i)} \geq 0$ to $q_{(i)} > 0$ and the explicit constraint $q_{(-n-1)} = 0$ to $q_{(-n-1)} = \epsilon$ where $\epsilon \in \mathbb{R}_{>0}$ gives us
\begin{align}
\label{eq:relax_const_posq}
& \min_{q_{(-i)} > 0 : \; i \in [n+1]\cup\{0\} }
\sum_{j \in \{-m : \; m \in [n+1]\}} g_j(q)
\\ &  \text{subject to:} \nonumber \\ & 
\quad q_{(0)} = (1-p)^K, \quad q_{(-n-1)} = \epsilon, \quad    \sum_{j} q_{(j)} = 1. \nonumber
\end{align}  

Let $p^*$ be the optimal value of \ref{eq:relax_const} and let $p_{\epsilon}^*$ be the optimal value of \ref{eq:relax_const_posq} for a given $\epsilon.$ Due to the continuity of the objective function in (\ref{eq:relax_const}), it is not hard to show that $ p^* \geq \inf_{\epsilon \in \mathbb{R}_{>0}} p_{\epsilon}^*.$  At a high level, this is due to the fact that for any solution to  (\ref{eq:relax_const}), it follows that (\ref{eq:relax_const_posq}) can get arbitrarily close to it as $\epsilon \to 0$ due to the continuity of the objective function.  



While we do not know the solution to (\ref{eq:relax_const}) or (\ref{eq:relax_const_posq}), we will perturb (\ref{eq:relax_const_posq}) to form a problem we can solve analytically, then use perturbation analysis to lower bound the optimal value of (\ref{eq:relax_const_posq}), and ultimately lower bound the optimal value of (\ref{eq:relax_const}).  The perturbed version of (\ref{eq:relax_const_posq}) is given by 
\begin{align}
\label{eq:relax_const_pert_posq}
& \min_{q_{(-i)} > 0 : \; i \in [n+1]\cup\{0\} }
\sum_{j \in \{-m : \; m \in [n+1]\}} g_j(q) \\	& 
\text{subject to:} \nonumber \\
& q_{(0)} = (1-p)^K, \quad q_{(-n-1)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
\nonumber \\ &     \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2} \nonumber
\end{align}  
\iscomment{change to $\beta$ notation. emphasize perturbation goes to $0$ as $n \to \infty$}
where we have changed the constraint on the probability at the minimum support value, and the constraint on the sum of all the probabilities.
We can solve this by solving the KKT conditions since the problem is convex, Slater's condition holds, and the objective function and constraint functions are differentiable on the domain $q_{(i)} > 0.$  

We proceed to find the solution to the KKT conditions for (\ref{eq:relax_const_pert_posq}).  Let $f_0(q)$ be the objective function of (\ref{eq:relax_const_pert_posq}).  The Lagrangian is given by 
\begin{align} 
&L(q, v, \lambda) = f_0(q) 
\nonumber \\ & + v_1 \left(\sum_i q_{(i)} - 1 + (1 - (1-p)^K)^{n+2} \right) 
\nonumber \\ & + v_2 \left(q_{(0)} - (1-p)^K \right) 
\nonumber \\ & + v_3 \left(q_{(-n-1)} - (1-p)^K (1 - (1-p)^K)^{n+1} \right). 
\end{align}
By Lemma \ref{lem:solve_KKT}, a solution to the KKT conditions is given by 
\begin{align}
\label{eq:KKT_conditions_sol}
& q_{(-i)} =  (1-p)^K (1 - (1-p)^K)^{i}  \text{ for } i \in [n+1] \cup \{0\} 
\nonumber \\ & v_1 = - p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right) 
\nonumber \\ & - (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right)
\nonumber \\ & v_2 = (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right) 
\nonumber \\ & v_3 = p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right),
\end{align}
which is then an optimal solution to (\ref{eq:relax_const_pert_posq}).  %The optimal value for (\ref{eq:relax_const_pert_posq}) is therefore given by 
%\begin{align} 
%& \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
%\nonumber \\ & - p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
%\nonumber \\ & = \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
%\nonumber \\ & - p \beta \alpha^i \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
%\end{align}
Applying the geometric sum formula and simplifying,  the optimal value for (\ref{eq:relax_const_pert_posq}) is   
\begin{align} 
& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
\end{align}
where $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K.$  

Using the perturbation analysis from Section 5.6.1 of \cite{boyd}, we see that the optimal value of (\ref{eq:relax_const_posq}) is lower bounded by
\begin{align}
\label{eq:relax_const_posq_bound}
& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
\nonumber \\ & - v_1^* \left( (1 - (1-p)^K)^{n+2} \right) 
\nonumber \\ & - v_3^* \left(- (1-p)^K (1 - (1-p)^K)^{n+1} +\epsilon \right) 
\end{align} 
where $v_1^*$ and $v_3^*$ are the optimal lagrange multipliers for (\ref{eq:relax_const_pert_posq})
we determined through the KKT conditions.

Taking the infimum of (\ref{eq:relax_const_posq_bound}) over $\epsilon \in \mathbb{R}_{>0}$ yields the following lower bound on (\ref{eq:relax_const}):

\begin{align}
\label{eq:relax_const_bound}
& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
\nonumber \\ & - v_1^* \left( (1 - (1-p)^K)^{n+2} \right) 
\nonumber \\ & - v_3^* \left(- (1-p)^K (1 - (1-p)^K)^{n+1} \right). 
\end{align} 

The sequence of optimal values returned by (\ref{eq:relax_const}) is monotonically decreasing in $n$ clearly.  Thus, taking the limit of the lower bound (\ref{eq:relax_const_bound}) as  $n \to \infty$ and simplifying yields the following lower bound on $-H(X \; | \; \alpha_0 X + Z_{\alpha})$ for any choice of $\alpha_i$'s: \begin{align} 
\label{eq:lower_bound_neg_cond_ent}
& -(p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right).
\end{align}

Finally, observe that
$-H(X \; ; \; X - G)$ is equal to (\ref{eq:lower_bound_neg_cond_ent})
where $G$ is a geometric random variable with
$\Pr(G = i) = (1-p)^K(1 - (1-p)^K)^i$ for $i \in  \mathbb{N} \cup \{0\}.$
% \end{IEEEproof}	
This concludes the proof of Theorem~\ref{thm:main_lower_bound}.



==> main_proof10_19_20.tex <==


\section{Proof of Theorem~\ref{thm:main_lower_bound}}

% We now present the proof of Theorem \ref{thm:main_lower_bound}.  
\iscomment{No need for the proof environment here}

% \begin{IEEEproof}
%First, notice that choosing integral $\alpha_i \; : \;  i \in [K] \cup \{0\}$ in the optimization problem (\ref{eq:main}) is optimal due to Lemma \ref{lem:integer_sol_optimal}, which holds because scaling the $\alpha_i$'s does not change the mutual information.  
%Lemma \ref{lem:integer_sol_optimal} holds because if $\alpha_i = \frac{c_i}{b_i} \; \forall i$ in (\ref{eq:main}) where $c_i, b_i$ are integral, then the solution $\alpha_i = \frac{c_i}{b_i} \left(\Pi_j b_j\right) \; \forall i$ is integral and the mutual information is preserved. 
%We will thus consider (\ref{eq:main}) with the constraint that $\alpha_i \in \mathbb{N}$ for $i \in [K] \cup \{0\}.$

% \begin{lemma}
%     \label{lem:integer_sol_optimal}
%     If an optimal solution to (\ref{eq:main}) exists, then there exists an optimal solution to (\ref{eq:main}) with $\alpha_i \in \mathbb{N}$ for $i \in [K] \cup \{0\}.$
% \end{lemma}

%Let $ Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i.$ 
We obtain the lower bound on $I(X \, ; \, \alpha_0 X + Z_{\alpha})= H(p) - H(X \, | \, \alpha_0 X+Z_{\alpha})$ in Theorem~\ref{thm:main_lower_bound} by finding a lower bound on $-H(X \, | \, \alpha_0 X+Z_{\alpha}).$  The optimization problem we consider is therefore
\begin{align}
   \label{eq:integral_alpha_opt_prob}
    & \min_{\alpha_0,...,\alpha_K \in \mathbb{N}} -H\left(X \; \left| \; \alpha_{0} X+\sum_{k=1}^K \alpha_k Z_k \right. \right).
\end{align}
Observe that the pmf of the random variable $Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i$ has probability $(1-p)^{K}$ at its highest support value. 
More precisely, $\sum_{i=1}^K \alpha_i$ is the maximum value that $Z_\alpha$ can take, which occurs with probability $(1-p)^{K}$.
% Furthermore, we notice that adding a constant to $Z_\alpha$ does not 
% the following problem is clearly 
A relaxation to (\ref{eq:integral_alpha_opt_prob}) can be then obtained by ignoring all constraints on the pmf of $Z_\alpha$ except the constraint on the maximum pmf value.
Thus, for a fixed value of $\alpha_0$, a relaxation to (\ref{eq:integral_alpha_opt_prob}) is given by
\begin{align}
   \label{eq:relax_inf1}
    \min_{Q} \; &  -H\left(X \; | \; \alpha_0 X+Q\right)
    \\\text{subject to:} \; & 
    \nonumber 
    % \\ 
    Q \text{ is an integer-valued random variable} \nonumber
    \\ & \text{$Q$ is independent of $X$} \nonumber
    % \nonumber \\ & D  \text{ has maximum support value at 0} 
    \\ & \Pr(Q = 0) = (1-p)^K \nonumber
    \\ & \Pr(Q = i) = 0 \; \text{ for $i > 0$}.
    \nonumber
\end{align}
\iscomment{Should we use $Q$ instead of $Q$ to match pmf?}
Notice that the last constraint is equivalent to saying that $0$ is the maximum value of $Q$.
This can be assumed without loss of generality, since adding a constant to $Q$ does not change the value of $H(X\,|\,\alpha_0X+Q)$.
Furthermore, as we prove in Appendix~\ref{app:alpha0}, 
% Due to Lemma \ref{lem:alpha0_condition}, 
fixing $\alpha_0 = 1$ in (\ref{eq:relax_inf1}) above 
does not change the optimal value, and we assume throughout that $\alpha_0=1$.
    
% without changing the optimal value.  

Let $q_{(i)}$ be the pmf of $Q$; i.e., $q_{(i)} = \Pr(Q=i)$ for $i \leq 0$.
% In o
% Let $q_{(0)}$ be the probability at the maximum support value of $D$ and let $q_{(-i)}$ be the probability at the $i$th integer below the maximum support value of $D.$ 
In order to write (\ref{eq:relax_inf1}) explicitly in terms of $q$, we define 
% g_j(q) = P(X+D=j+1)*H(X|X+D=j+1). 
\begin{align}
    g_j(q) & \triangleq -H(X|X+Q=j+1)\Pr(X+Q=j+1) \nonumber \\
    & =  \Pr(Q+X=j+1)  \nonumber \\
    & \quad \times \bigg[ \frac{(1-p)q_{(j)}}{\Pr(Q+X=j+1)} \log\left(\frac{(1-p)q_{(j)}}{\Pr(Q+X=j+1)}\right) \nonumber \\       &  \quad + \frac{p q_{(j+1)}}{\Pr(Q+X=j+1)} \log\left(\frac{p q_{(j+1)}}{\Pr(Q+X=j+1)}\right) \bigg] \nonumber \\   
    % & =  \Pr(Q+X=j+1)  \nonumber \\
    % & \times \bigg(\frac{\Pr(Q=j)(1-p)}{\Pr(Q+X=j+1)} \log\left(\frac{\Pr(Q=j)(1-p)}{\Pr(Q+X=j+1)}\right) \nonumber \\       &  + \frac{\Pr(Q=j+1)p}{\Pr(Q+X=j+1)} \log\left(\frac{\Pr(Q=j+1)p}{\Pr(Q+X=j+1)}\right) \bigg) \nonumber \\   
    % & = q_{(j)}(1-p) \log\left(\frac{q_{(j)}(1-p)}{\Pr(Q+X=j+1)}\right) \nonumber \\       &  + q_{(j+1)}p \log\left(\frac{q_{(j+1)}p}{\Pr(Q+X=j+1)}\right) \nonumber \\   
    & = (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
    \nonumber 
    \\ & \quad + p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right).
\end{align}
Written in terms of $g_j(q)$ and with $\alpha_0 = 1$, (\ref{eq:relax_inf1}) is given by
\begin{align}
\label{eq:relax_inf2}
\min_{q_{(-i)} \geq 0 : \; i \in \N_0 } \; & \sum_{j \in \{-n : \; n \in \mathbb{N}\}} g_j(q)
\\ \text{subject to:} \; & \quad q_{(0)} = (1-p)^K \nonumber \\ &  \quad    \sum_{j=0}^\infty q_{(-j)} = 1. \nonumber
\end{align}  
\kmcomment{I removed ``Note that the conditional entropy in the objective function is in a simplified form.''  It meant we used Bayes rule in the conditional entropy  }
\iscomment{What does this mean?}

\iscomment{I rewrote the following a bit:}

Observe that (\ref{eq:relax_inf2}) is a convex minimization problem with infinitely many variables.  
For such problems, to the best of our knowledge, a solution to the KKT conditions is not in general guaranteed to yield an optimal solution.
For that reason, we do not seek to directly solve the KKT conditions.
Instead, we first consider a \emph{support-constrained} version of (\ref{eq:relax_inf2}), where the support of the pmf of $Q$ is restricted to $\{-n,...,0\}$, and then consider letting $n \to \infty$.
% 
% A solution to the KKT conditions with the added implicit constraint that $q_{(-i)}>0$ for $i \in \N_0$  is given by  $q_{(-i)} = (1-p)^K (1 - (1-p)^K)^i$ for $i \in \N_0$ 
% \iscomment{Is this obvious?}
% which corresponds to $D = -G$ in (\ref{eq:relax_inf1}) where $G$ is a geometric random variable with success probability equal to $(1-p)^K$ and support equal to $\N_0$.  
% We do not use this observation directly to establish Theorem \ref{theorem:main_recursion} because no reference on the relation between KKT conditions and optimality in the infinite dimensional case was found.  
% 
% Instead, we constrain $D$ to have distance no greater than $n \in \mathbb{N}$ between its maximum and minimum support values in (\ref{eq:relax_inf2}), derive a lower bound on the solution for each $n \in \mathbb{N},$ and use the resulting sequence of lower bounds to establish the result. 
The support-constrained version of (\ref{eq:relax_inf2}) is given by 
\begin{align}
\label{eq:relax_const}
\min_{q_{(i)} \geq 0 : \; i \in \{-n-1,...,0\} } \; & 
\sum_{j \in \{-m : \; m \in [n+1]\}} g_j(q) \\  \text{subject to:}  \; &  
q_{(0)} = (1-p)^K, \quad q_{(-n-1)} = 0 \nonumber \\
\quad & \; \sum_{j=0}^\infty q_{(-j)} = 1. \nonumber
\end{align}  
Note that this is no longer a relaxation to the original problem.
\iscomment{say this is no longer a relaxation}


In order to ensure that the derivative of the objective function exists at all feasible $q_{(i)},$ and ultimately find a lower bound on the optimal value of (\ref{eq:relax_const}) through perturbation analysis, we we consider the problem below where we change the constraint in (\ref{eq:relax_const}) from $q_{(i)} \geq 0$ to $q_{(i)} > 0$ and the constraint $q_{(-n-1)} = 0$ to $q_{(-n-1)} = \epsilon$ where $\epsilon \in \mathbb{R}_{>0}:$
\begin{align}
\label{eq:relax_const_posq}
& \min_{q_{(i)} > 0 : \; i \in \{-n-1,...,0\} }
\sum_{j \in \{-m : \; m \in [n+1]\}} g_j(q)
\\ &  \text{subject to:} \nonumber \\ & 
\quad q_{(0)} = (1-p)^K, \quad q_{(-n-1)} = \epsilon, \quad    \sum_{j=0}^\infty q_{(-j)} = 1. \nonumber
\end{align}  

Let $v^*$ be the optimal value of (\ref{eq:relax_const}) and let $v_{\epsilon}^*$ be the optimal value of (\ref{eq:relax_const_posq}) for a given $\epsilon.$ Due to the continuity of the objective function in (\ref{eq:relax_const}), we have $ v^* \geq \inf_{\epsilon \in \mathbb{R}_{>0}} v_{\epsilon}^*.$  More precisely, for any solution to  (\ref{eq:relax_const}), it follows that (\ref{eq:relax_const_posq}) can get arbitrarily close to the corresponding value as $\epsilon \to 0$ due to the continuity of the objective function.  



While we do not know the solution to (\ref{eq:relax_const}) or (\ref{eq:relax_const_posq}), we will perturb (\ref{eq:relax_const_posq}) to form a problem we can solve analytically, then use perturbation analysis to lower bound the optimal value of (\ref{eq:relax_const_posq}), and ultimately lower bound the optimal value of (\ref{eq:relax_const}).  Let $\beta \triangleq (1-p)^K.$  The perturbed version of (\ref{eq:relax_const_posq}) is given by 
\begin{align}
\label{eq:relax_const_pert_posq}
& \min_{q_{(i)} > 0 : \; i \in \{-n-1,...,0\} }
\sum_{j \in \{-m : \; m \in [n+1]\}} g_j(q) \\	& 
\text{subject to:} \nonumber \\
& q_{(0)} = \beta , \quad q_{(-n-1)} = \beta  (1 - \beta )^{n+1}, 
\nonumber \\ &    \sum_{j=0}^\infty q_{(-j)} = 1 - (1 - \beta )^{n+2} \nonumber
\end{align}  
\iscomment{change to $\beta$ notation. emphasize perturbation goes to $0$ as $n \to \infty$} 
where we have changed the constraint on the probability at the minimum support value, and the constraint on the sum of all the probabilities.  Observe that as $n$ increases, we have that $\beta  (1 - \beta )^{n+1}\to 0$ and $1 - (1 - \beta )^{n+2} \to 1.$  In other words, the constraints in (\ref{eq:relax_const_pert_posq}) approach the constraints in (\ref{eq:relax_const}).
We can solve (\ref{eq:relax_const_pert_posq}) by solving the KKT conditions since the problem is convex, Slater's condition holds, and the objective function and constraint functions are differentiable on the domain $q_{(i)} > 0.$  

We proceed to find the solution to the KKT conditions for (\ref{eq:relax_const_pert_posq}).  Let $f_0(q)$ be the objective function of (\ref{eq:relax_const_pert_posq}).  The Lagrangian is given by 
\begin{align} 
&L(q, v, \lambda) = f_0(q) 
\nonumber \\ & + v_1 \left(\sum_i q_{(i)} - 1 + (1 - \beta)^{n+2} \right) 
\nonumber \\ & + v_2 \left(q_{(0)} - \beta \right) 
\nonumber \\ & + v_3 \left(q_{(-n-1)} - \beta (1 - \beta)^{n+1} \right). 
\end{align}
By Lemma \ref{lem:solve_KKT}, a solution to the KKT conditions is given by 
\begin{align}
\label{eq:KKT_conditions_sol}
& q_{(-i)} =  \beta (1 - \beta)^{i}  \text{ for } i \in [n+1] \cup \{0\} 
\nonumber \\ & v_1 = - p \log \left( \frac{p}{(1-p)(1 - \beta) + p} \right) 
\nonumber \\ & - (1-p)\log \left( \frac{(1-p)(1 - \beta)}{(1-p)(1 - \beta) + p} \right)
\nonumber \\ & v_2 = (1-p)\log \left( \frac{(1-p)(1 - \beta)}{(1-p)(1 - \beta) + p} \right) 
\nonumber \\ & v_3 = p \log \left( \frac{p}{(1-p)(1 - \beta) + p} \right),
\end{align}
which is then an optimal solution to (\ref{eq:relax_const_pert_posq}).  %The optimal value for (\ref{eq:relax_const_pert_posq}) is therefore given by 
%\begin{align} 
%& \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
%\nonumber \\ & - p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
%\nonumber \\ & = \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
%\nonumber \\ & - p \beta \alpha^i \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
%\end{align}
Applying the geometric sum formula and simplifying,  the optimal value for (\ref{eq:relax_const_pert_posq}) is   
\begin{align} 
& -(1-p) \beta (1-\beta) \frac{1 - (1-\beta)^{n+1}}{1 - (1-\beta)} \log \left( \frac{(1-p) (1-\beta) + p }{(1-p) (1-\beta)} \right) 
\nonumber \\ & - p \beta \frac{1 - (1-\beta)^{n+1}}{1 - (1-\beta)} \log \left( \frac{(1-p)  (1-\beta) + p }{ p } \right).
\end{align}

Using the perturbation analysis from Section 5.6.1 of \cite{boyd}, we see that the optimal value of (\ref{eq:relax_const_posq}) is lower bounded by
\begin{align}
\label{eq:relax_const_posq_bound}
& -(1-p) \beta (1-\beta) \frac{1 - (1-\beta)^{n+1}}{1 - (1-\beta)} \log \left( \frac{(1-p) (1-\beta) + p }{(1-p) (1-\beta)} \right) 
\nonumber \\ & - p \beta \frac{1 - (1-\beta)^{n+1}}{1 - (1-\beta)} \log \left( \frac{(1-p)  (1-\beta) + p }{ p } \right)
\nonumber \\ & - v_1^* \left( (1 - \beta)^{n+2} \right) 
\nonumber \\ & - v_3^* \left(- \beta (1 - \beta)^{n+1} +\epsilon \right) 
\end{align} 
where $v_1^*$ and $v_3^*$ are the optimal lagrange multipliers for (\ref{eq:relax_const_pert_posq})
we determined through the KKT conditions.

Taking the infimum of (\ref{eq:relax_const_posq_bound}) over $\epsilon \in \mathbb{R}_{>0}$ yields the following lower bound on (\ref{eq:relax_const}):

\begin{align}
\label{eq:relax_const_bound}
& -(1-p) \beta (1-\beta) \frac{1 - (1-\beta)^{n+1}}{1 - (1-\beta)} \log \left( \frac{(1-p) (1-\beta) + p }{(1-p) (1-\beta)} \right) 
\nonumber \\ & - p \beta \frac{1 - (1-\beta)^{n+1}}{1 - (1-\beta)} \log \left( \frac{(1-p)  (1-\beta) + p }{ p } \right)
\nonumber \\ & - v_1^* \left( (1 - \beta)^{n+2} \right) 
\nonumber \\ & - v_3^* \left(- \beta (1 - \beta)^{n+1} \right). 
\end{align} 

The sequence of optimal values returned by (\ref{eq:relax_const}) is monotonically decreasing in $n$ clearly.  Thus, taking the limit of the lower bound (\ref{eq:relax_const_bound}) as  $n \to \infty$ and simplifying yields the following lower bound on $-H(X \; | \; \alpha_0 X + Z_{\alpha})$ for any choice of $\alpha_i$'s: \begin{align} 
\label{eq:lower_bound_neg_cond_ent}
& -(p-1) \left( (1-p)^K - 1\right) \log \left( \frac{1 - (1-p)^{K+1} }{(p-1) \left( (1-p)^K -1 \right)}\right) 
\nonumber \\ & - p \log \left( \frac{1 - (1-p)^{K+1} }{p} \right).
\end{align}

Finally, observe that
$-H(X \; ; \; X - G)$ is equal to (\ref{eq:lower_bound_neg_cond_ent})
where $G$ is a geometric random variable with
$\Pr(G = i) = (1-p)^K(1 - (1-p)^K)^i$ for $i \in  \N_0.$
% \end{IEEEproof}	
This concludes the proof of Theorem~\ref{thm:main_lower_bound}.



==> main_result10_13_20.tex <==
\section{Main Result}


%\begin{figure}
%\centering
%\includegraphics[width=0.9\linewidth]{performance_plot_K6_minor_allele}
%\caption{}
%\label{fig:performance_plot_K6_minor_allele}
%\end{figure}

Our main result is stated below.

\begin{theorem} \label{thm:main_lower_bound}
	For any $K\in \mathbb{N},$ $p \in [0, 0.5],$  we have that 
	\begin{align} 
	& \min_{\alpha_i \in \mathbb{N}, \; i \in [K]\cup\{0\}} I(X \; ; \; \alpha_0 X + \sum_{i=1}^{K} \alpha_i Z_i) 
% 	\nonumber \\ & 
	\geq 
	I(X \; ; \; X - 2G)
	\end{align}
	where $G$ is a geometric random variable with success probability equal to $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\}.$
\end{theorem}
The formula for $I(X \; ; \; X - 2G)$ is given by 
\begin{align}
& I(X \; ; \; X - 2G)
\nonumber \\ & = H(p) 
\nonumber \\ & - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
\end{align}
Observe that the formula is quickly computable for any value of $K$ and $p,$ making it attractive from a computational standpoint.  To assess how tight the lower bound is, we empirically compare it to an upper bound that is computed with a greedy algorithm in Figure \ref{fig:greedy_versus_bound_K15}.  For a given $p$ and $K,$ the greedy algorithm chooses $\alpha_1 = 1,$ and sequentially chooses \begin{align} \alpha_{j} = \argmin_{\alpha \in \mathbb{N} \; : \; 1 \leq \alpha \leq 1 + \sum_{i = 1}^{j-1}  \alpha_i} I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)
\end{align}
for $2 \leq j \leq K.$  As seen in Figure \ref{fig:greedy_versus_bound_K15}, $I(X \; ; \; X - 2G)$ serves as a very tight lower bound when compared with the upper bound.  We therefore view $I(X \; ; \; X - 2G)$ as an approximation to the original problem.

While the greedy algorithm requires $\Omega(2^K)$ time in the worst case, similar plots to Figure \ref{fig:greedy_versus_bound_K15} can be obtained for larger values of $K$ using a more computationally efficient variation of the greedy algorithm that is discussed in the longer version of this paper.

In order to prove the lower bound on the minimization of $I(X \; ; \; \alpha_0 X + \sum_{i=1}^K \alpha_i Z_i)$ in Theorem \ref{thm:main_lower_bound}, we form a convex relaxation of the minimization problem, perturb the relaxation to form a problem that is analytically solvable using KKT conditions, and use perturbation analysis to find a lower bound on the relaxation.  This is then a lower bound on the original problem.  The full proof is in the Section V.

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .06]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{upper bound (greedy)}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\label{fig:greedy_versus_bound_K15}
\end{figure}

%\begin{tikzpicture}
%\begin{axis} 
%[title ={Comparison of Bounds: $K = 15$},
%ylabel = mutual information, 
%xlabel = minor allele frequency (p),
%ymax = .001,
%legend pos=north west]

%\addplot [
%line width=1pt,
%color=red!80!black
%] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{upper bound}

%\addplot [
%line width=1pt,
%color=blue!80!black
%] table[x index=0,y index=1] %{data/plt2_bound.dat};
%\addlegendentry{lower bound}

%\end{axis}    
%\end{tikzpicture}
%\caption{}
%\label{fig:greedy_versus_bound_K15}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p1}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p1}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p001}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p001}
%\end{figure}


%The lower bound is formally proved in the appendix, but we outline the argument here, as it sheds light on the problem, and makes interesting use of convex optimization theory

\section{Efficiently Computable Schemes}

\rdcomment{this may sound stupid, but i think it warrants a sentence here. `Theorem 1 gives us a lower bound on the mutual information between $X$ and ..., which would be the mixing ratio that provides the highest level of privacy. However, it does not provide any mixing scheme for approaching this lower bound.'}

While much faster than brute force search, the greedy algorithm used to obtain the upper bound requires $\Omega(2^K)$ time in the worst case.  At a high level, this is due to the fact that at the $j$th  step in the algorithm, computation of $I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)$ requires use of each support value in the PMF of $\alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i,$ and there are $\Omega(2^j)$ support values in the worst case.  This motivates the design of efficiently computable schemes, which can then be evaluated using the lower bound in Theorem \ref{thm:main_lower_bound}.

Perhaps the most natural approach is given by the uniform scheme, which we define to set $\alpha_i = 1$ for all $i \in [K]\cup\{0\}.$  This is the scheme used by the authors of \cite{Maddah-Ali} to obtain their results.  The scheme is explicitly defined given $K,$ so no algorithm is needed to compute it.  The performance of the scheme for a given $p$ and $K$ can be computed in $O(K)$ time using the formula in Lemma \ref{lem:uniform_schem_formula} which is given in the appendix.

The uniform scheme is important because it is optimal as $p \to 0$ as proved in Lemma \ref{lem:optimality_of_uniform}
and exemplified by the optimal curve in Figure \ref{fig:optimal_scheme_K5_minor_allele}.

\begin{lemma}
\label{lem:optimality_of_uniform}
For any $K \in \mathbb{N},$ there exists some $p^* > 0$ such that the uniform scheme is optimal for $p < p^*.$
\end{lemma}

\rdcomment{i changed epsilon to $p^*$ here. epsilon is typically taken to mean a very small constant, which makes this result feel weak, i.e. this result is only true when p is arbitrarily small.}

At $p= 0.5,$ in Figure \ref{fig:optimal_scheme_K5_minor_allele}, the optimal solution is given by the binary scheme, which we define to set $\alpha_0 = 1$ and $\alpha_i = 2^{i-1}$ for all $i \in [K].$  Similar to the uniform scheme, the binary scheme is explicitly defined given $K.$  Also, similar to the uniform scheme, there exists a formula for computing its performance given $p$ and $K$ in $O(K)$ time.  This formula is given in Lemma \ref{lem:binary_scheme_performance} in the appendix.  It is interesting that such a formula exists because the PMF of $\sum_{i=1}^K 2^{i-1} Z_i$ has $2^K$ support values. 

Most importantly, the optimality of the binary scheme at $p = 0.5$ for $K=5$ shown in Figure \ref{fig:optimal_scheme_K5_minor_allele} generalizes to all $K$ as proved in Lemma \ref{lem:optimality_of_binary}.

\begin{lemma} \label{lem:optimality_of_binary}
	For any $K \in \mathbb{N},$ the binary scheme is optimal for $p = 0.5.$
\end{lemma}

Because the uniform scheme is optimal for $p \to 0$ and the binary scheme is optimal for $p = 0.5,$  it is natural to try and combine these schemes to interpolate the performance for $p$ in the range $0<p<0.5.$  Combining only the uniform scheme and the binary scheme does not produce a scheme that approaches the lower bound.  However, the general shape of the lower bound can be captured in polynomial time by combining the uniform scheme, the linear scheme, and the binary scheme where the linear scheme is defined as $\alpha_i = i$ for $i \in [K].$  We define the $(K,L,U)$-binary-linear-uniform scheme to set $\alpha_0 = 1$ and 
\begin{align} &\alpha_i = 1 \quad i \in \{1, ..., U\} \nonumber \\  &\alpha_{U+i} = i \quad i \in \{1, ..., L\} \nonumber \\
&\alpha_{U+L+i} = 2^{i-1} \quad i \in \{1, ..., K-U-L\}
\end{align}

\rdcomment{should it be binary-linear-uniform above?}

For a given $K$ and $p,$ we define the $K$-binary-linear-uniform scheme as the $(K,L^*,U^*)$-binary-linear-uniform scheme where
\begin{align} & (L^*, U^*) = \argmin_{(L,U) \in ([K]\cup\{0\})^2 \; : \; L + U \leq K} \\ &  I\left(X \; ; \; X + \sum_{i=1}^{U} Z_i + \sum_{j=1}^{L} j Z_{U+j} +  \sum_{k=1}^{K-U-L} 2^{k -1} Z_{U+L+k}\right) \nonumber.
\end{align}
The $K$-binary-linear-uniform scheme is computed in $O(K^4)$ time using a generalization of the recursion used to prove Lemma \ref{lem:binary_scheme_performance}.  

We compare the performance of the uniform scheme, the binary scheme, the $K$-binary-linear-uniform scheme, and the scheme generated by the greedy algorithm in Figure \ref{fig:efficiently_computable_schemes}.  We have observed that the greedy scheme generated by the greedy algorithm is much tighter than the   $K$-binary-linear-uniform scheme after the initial hump in the lower bound as $K$ increases.



\begin{figure}[h]
\label{fig:efficiently_computable_schemes}
\centering
\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .6,
legend pos = north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}


\end{axis}    
\end{tikzpicture}

\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .01]
%,
%legend pos=north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
%\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
%\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
%\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
%\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
%\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\end{figure}



%Greedy takes exponential time in $K$ to compute.

%Simpler schemes: uniform, binary, interpolation between uniform and binary.


%Maybe state theorems about uniform and binary. Or maybe just mention them and refer to the longer version

\section{Proof of Main Result}

We now present the proof of Theorem \ref{thm:main_lower_bound}, which makes interesting use of convex optimization theory.  

\rdcomment{this may be similar to the IS comments, but this proof is a bit hard to read for me. i understand the first few paragraphs in words, but it is not trivial to me to see exactly how this formally changes the problem. i would suggest stating the problem, and then how the support-constraint changes the optimization, and so on. to be honest, if you're tight on space, i still think it would be more beneficial to dedicate more space to this `reduction' and then even leave some of the more mechanical parts of derivatives/KKT condition analysis out.

also, we arrived at this result through figures and drawings; can we add some of this into the proof? i think it would strengthen the appeal of this paper to hint at why the idea is actually intuitive and cute. as written, it feels more a set of mechanical manipulations of KKT conditions, and it loses the sort of elegance i typically associate with info theory papers. (this is not a comment on the result, it's just a comment on the presentation and how it makes me feel.) i really liked the drawings of the convolution of discrete measures, and how we're really chosing a measure that gets shifted to the left by 1 and rescaled by 1-p and shifted to the right by 1 and rescaled by p. can this be put in this section at all?}
\begin{IEEEproof}
	Let $ Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i.$ We obtain the lower bound on $I(X \; ; \; \alpha_0 X + Z_{\alpha})= H(p) - H(X \; | \; \alpha_0 X+Z_{\alpha})$ in Theorem \ref{thm:main_lower_bound} by finding a lower bound on $-H(X \; | \; \alpha_0 X+Z_{\alpha}).$  In order to lower bound $-H(X \; | \; \alpha_0 X+Z_{\alpha}),$ we begin by considering the original optimization problem with the added constraint that the distance between the minimum support value and the maximum support value in the PMF of $Z_{\alpha}$ is less than $2n+2$ where $n \in \mathbb{N}, \; n > 0.$  We will obtain a lower bound for this support constrained optimization problem, and use it to obtain a lower bound on the original optimization problem.  
	\iscomment{unclear why this can be done}
	
	To lower bound the support constrained optimization problem, we work with a relaxation of the support constrained  optimization problem.  Instead of requiring that the PMF for the noise random variable $D$ be generated by adding the sum of scaled random variables with support $\{-1, 1\},$ we relax the problem to only require that the probability at the highest support value of $D$'s PMF is equal to $(1-p)^K$ and the distance between each pair of support values in $D$'s PMF is a multiple of two (this holds for any valid PMF of $Z_{\alpha}$).  
	Due to Lemma \ref{lem:alpha0_condition}, given $\alpha_0,$ any solution can be transformed into solution whose PMF had support values in $\{2t \alpha_0 : \; t \in \mathbb{Z}\}$ without increasing the mutual information.   Therefore, for a fixed $\alpha_0,$ it suffices to only consider PMFs that have support values in $\{2t \alpha_0 : \; t \in \mathbb{Z}\}$ in the optimization.  If $\alpha_0 = a \in \mathbb{N}$ any solution random variable $D$ with  support values in $\{2t a : \; t \in \mathbb{Z}\}$ can be transformed into a solution with the same mutual information, $\alpha_0 = 1,$ and support values in $\{2t : \; t \in \mathbb{Z}\}.$ This is accomplished by dividing $D$ by $a.$     Therefore, we analyze the relaxation with $\alpha_0 = 1.$
	
	We then obtain a lower bound on this relaxation of the support constrained optimization problem .  Finally, we take the limit of the lower bound as $n$ goes to infinity in order to obtain a lower bound on the original minimization problem.
	
	The support-constrained relaxation of the original problem with $\alpha_0 = 1$ is given below. The objective function is a simplified form of $-H(X \; | \; X+D)$ where $D$ is the noise distribution we are optimizing over that is constrained to have probability of $(1-p)^K$ at the maximum support value, and each pair of support values separated by a multiple of two. Here, $q_{(0)}$ is the probability at the maximum support value of $D$ and $q_{(-i)}$ is the probability at the $i$th integer below the maximum support value of $D.$  Observe that the problem is a convex minimization problem.
	%Due to the fact that $X, Z_j \in \{-1, 1\},$ we have that all support values are separated by multiples of two in any valid PMF of $Z_{\alpha}.$  Therefore, $q_{(i)}=0$ for odd values of $i$ in the relaxation.  Observe that the problem is a convex minimization problem.
	\iscomment{not clear how this was obtained:}
	\begin{align}
	& \min_{q_{(-2n-2)}, \; ..., \;  q_{(0)}} \sum_{j \in \{-2n-2, \; ...,\;  -2\}} 
	\nonumber \\ & (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+2)}} \right) 
	\nonumber \\ & + p q_{(j+2)} \log \left(\frac{p q_{(j+2)}}{(1-p)q_{(j)} + p q_{(j+2)}} \right)    \\
	\nonumber \\ &  \text{subject to:} \quad  q_{(j)} \geq 0 \; \; \forall j,  \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad q_{(-2n-2)} = 0, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1. \nonumber
	\end{align}  
	
	\iscomment{do we need the full formula for the conditional entropy above? makes it harder to parse}
	While we cannot solve this problem analytically, we will perturb it to form an optimization problem that we can solve analytically.  We will then use perturbation analysis to obtain a lower bound on the problem above.
	
	
	The perturbed problem is given below where we have changed the constraint on the probability at the minimum support value, and the constraint on the sum of all the probabilities.
	
	\begin{align}
	& \min_{q_{(-2n-2)}, \; ..., \;  q_{(0)}} \sum_{j \in \{-2n-2, \; ...,\;  -2\}} 
	\nonumber \\ &  (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+2)}} \right) 
	\nonumber \\ & +  p q_{(j+2)} \log \left(\frac{p q_{(j+2)}}{(1-p)q_{(j)} + p q_{(j+2)}} \right)    \\
	\nonumber \\	&  \text{subject to:} \quad  q_{(j)} \geq 0 \; \; \forall j,  \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad q_{(-2n-2)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2} \nonumber
	\end{align}  
	
	
	Let $f_0(q)$ be the objective function above.  The Lagrangian is given by 
	
	\begin{align} 
	&L(q, v, \lambda) = f_0(q) 
	\nonumber \\ & + v_1 \left(\sum_i q_{(i)} - 1 + (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & + v_2 \left(q_{(0)} - (1-p)^K \right) 
	\nonumber \\ & + v_3 \left(q_{(-2n-2)} - (1-p)^K (1 - (1-p)^K)^{n+1} \right) 
	\nonumber \\ & - \sum_i \lambda_i q_{(i)}. 
	\end{align}
	The derivative of $f_0(q)$ with respect to $q_{(j)}$ is given by 
	\begin{align}
	& p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-2)} + p q_{(j)}} \right) \nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+2)} + (1-p) q_{(j)}} \right).
	\end{align}  
	for $j \in \{-2n, \; ..., \;  -2\}$ and the KKT conditions are therefore given by 
	\begin{align}
	&  q_{(j)} \geq 0 \; \; \forall j,  \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & q_{(-2n-2)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ &     \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2}
	\nonumber \\ & \lambda_j \geq 0 \quad \lambda_j q_{(j)} = 0 \quad \forall j 
	\nonumber \\ & (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+2)} + (1-p) q_{(j)}} \right) - \lambda_j + v_1 + v_3 = 0 \quad 
	\nonumber \\ &  \text{for } j = - 2n -2
	\nonumber \\ & 	p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-2)} + p q_{(j)}} \right) 
	\nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+2)} + (1-p) q_{(j)}} \right) - \lambda_j + v_1 = 0 
	\nonumber \\ &  \forall j \in \{-2n, \; ..., \;  -2\}
	\nonumber \\ & p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-2)} + p q_{(j)}} \right) - \lambda_j + v_1 + v_2 = 0 
	\nonumber \\ & \text{for } j = 0
	\end{align}
	
	\rdcomment{stupid question: can you tell me a little more why (12) is this derivative? at a glance, it seems to be that there's a ton of term cancellations... (it's like the terms inside the log don't depend on $q_j$ with the way the derivative is written, so all those terms cancel?) i fear that a unfastidious reviewer may just claim this is a fundamental error and give a poor review without analyzing it deeply. (this happens sometimes to me.)}
	
	The last three conditions can be rewritten as 
	\begin{align} 
	& (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+2)}}{q_{(j)}} + (1-p) } \right) - \lambda_j + v_1 + v_3 = 0  
	\nonumber \\ &  \text{for } j = - 2n - 2
	\nonumber \\ & p \log \left(\frac{p }{(1-p)\frac{q_{(j-2)}}{q_{(j)}} + p } \right) + (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+2)}}{q_{(j)}} + (1-p) } \right) 
	\nonumber \\ & - \lambda_j + v_1  = 0 \quad \forall j \in \{-2n, \; ..., \;  -2\}
	\nonumber \\ & p \log \left(\frac{p }{(1-p) \frac{q_{(j-2)}}{q_{(j)}} + p } \right) - \lambda_j + v_1 + v_2  = 0 \quad \text{for } j = 0
	\end{align}
	which shows that if the ratio $\frac{q_{(j-2)}}{q_{(j)}}$ between consecutive variables is the same for all $j$ and $\lambda_j = 0 $ for all $j,$ then $v_1,$ $v_2$ can  be chosen so that of these derivatives equal $0$ for all $j.$  Picking \[\frac{q_{(j-2)}}{q_{(j)}} = (1 - (1-p)^K),\] a solution to these equations is then
	\begin{align}
	& q_{(-2i)} =  (1-p)^K (1 - (1-p)^K)^{i}  
	\nonumber \\ & \quad \quad \text{for } i \in \{0, \; 1, \; ..., \; n+1 \} 
	\nonumber \\ & \lambda_i = 0 \quad \forall i
	\nonumber \\ & v_1 = - p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & - (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right)
	\nonumber \\ & v_2 = (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & v_3 = p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right)
	\end{align}
	
	Because this is a convex optimization problem, this solution is optimal since it satisfies the KKT conditions.
	
	The optimal value for the optimization problem is therefore given by 
	\begin{align} 
	& \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
	\\ & - p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	\\ & = \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\\ & - p \beta \alpha^i \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\end{align}
	where $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K.$  
	Applying the geometric sum formula and simplifying, we obtain 
	\begin{align} 
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right).
	\end{align}
	
	
	
	%The optimal value for the optimization problem is therefore given by 
	%\begin{align} 
	%& -(1-p) \beta \alpha \frac{1 - \alpha^{2n+2}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	%\nonumber \\ & - p \beta \frac{1 - \alpha^{2n+2}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right).
	%\end{align}
	%after some simplification.
	
	Using the perturbation analysis from Section 5.6.1 of \cite{boyd}, we see that the optimal value of the support constrained relaxation of the original problem is lower bounded by
	\begin{align}
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\nonumber \\ & - v_1^* \left( (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & - v_3^* \left(- (1-p)^K (1 - (1-p)^K)^{n+1}  \right) 
	\end{align} 
	where $v_1^*$ and $v_3^*$ are the optimal lagrange multipliers for the perturbed problem which we determined above through the KKT conditions.
	
	The sequence of optimal values returned by the support constrained relaxation of the original problem is monotonically decreasing in $n$ clearly.  Thus, taking the limit of the bound as  $n \to \infty$ and simplifying yields the following lower bound on $-H(X \; | \; \alpha_0 X + Z_{\alpha})$ for any choice of $\alpha_i$'s: 	\begin{align} 
	& -(p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right).
	\end{align}
	
	Thus, a lower bound on mutual information is
	\begin{align} 
	& H(p) - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
	\end{align}
	for any choice of $\alpha_i$'s.
	
	Finally, observe that
	\begin{align}
	& H(X \; ; \; X - 2G) 
	\nonumber \\ & =\sum_{i = 0}^{\infty} (1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
	\nonumber \\ & + p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	\nonumber \\ & = (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right)  
	\nonumber \\ & + p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
	\end{align}
	where $G$ is a geometric random variable with success probability $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\},$  and $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K$ as before.
\end{IEEEproof}

\begin{lemma}
    \label{lem:alpha0_condition}
	Let $X$ be a random variable that equals $1$ with probability $(1-p)$ and equals $-1$ with probability $p.$  Let $\alpha_0 \in \mathbb{N}.$ 
	Let $Z$ be any random variable such that its PMF has integral support and maximum support value at $t = 0.$  Let 
	\begin{align}
	& \hat{Z} = Z - (Z \mod{2\alpha_0})   
	\end{align} 
	%\sum_{i = 1}^{2\alpha_0-1} i \text{\bf1} \{Z \mod{2\alpha_0}= i\}. 
	%$\Pr(\hat{Z} = t) = \sum_{i=0}^{2\alpha_0-1} \Pr(Z = t+i)$ 
	We then have that 
	\begin{align}
	& I(X ; \alpha_0 X + 	Z)  \geq I(X ; \alpha_0 X + \hat{Z}).   
	\end{align}	
\end{lemma}

\begin{IEEEproof}
	Let  $S = Z \mod{2\alpha_0}.$  We then have that 
	\begin{align} 
		& I(X ; \; \alpha_0 X + 	Z)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z} +  S)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z}, \; S)
		\nonumber \\ & = I(X ; \; S) + I(X ; \; \alpha_0 X + \hat{Z} \; | \; S)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z} \; | \; S)
		\nonumber \\ & = H(X \; | \; S)  - H(X \; | \; \alpha_0 X + \hat{Z}, \; S) 
		\nonumber \\ & = H(X)  - H(X \; | \; \alpha_0 X + \hat{Z}, \; S)
		\nonumber \\ & \geq H(X)  - H(X \; | \; \alpha_0 X + \hat{Z})
		\nonumber \\ & = I(X \; ; \; \alpha_0 X + \hat{Z})
	\end{align} 
	where the third line follows because given $\alpha_0 X + \hat{Z} + S,$ we have that 
	\begin{align}
	    S = ((\alpha_0 X + \hat{Z} + S) - \alpha_0) \mod 2 \alpha_0 
	\end{align}
	and
    \begin{align}
	    \alpha_0 X + \hat{Z} = (\alpha_0 X + \hat{Z} + S) - S.
	\end{align}
	
	\end{IEEEproof}


==> main_result10_14_20.tex <==
\section{Main Result}


%\begin{figure}
%\centering
%\includegraphics[width=0.9\linewidth]{performance_plot_K6_minor_allele}
%\caption{}
%\label{fig:performance_plot_K6_minor_allele}
%\end{figure}

Our main result is stated below.

\begin{theorem} \label{thm:main_lower_bound}
	For any $K\in \mathbb{N},$ $p \in [0, 0.5],$  we have that 
	\begin{align} 
	& \min_{\alpha_i \in \mathbb{N}, \; i \in [K]\cup\{0\}} I(X \; ; \; \alpha_0 X + \sum_{i=1}^{K} \alpha_i Z_i) 
% 	\nonumber \\ & 
	\geq 
	I(X \; ; \; X - G)
	\end{align}
	where $G$ is a geometric random variable with success probability equal to $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\}.$
\end{theorem}
The formula for $I(X \; ; \; X - G)$ is given by 
\begin{align}
& I(X \; ; \; X - G)
\nonumber \\ & = H(p) 
\nonumber \\ & - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
\end{align}
Observe that the formula is quickly computable for any value of $K$ and $p,$ making it attractive from a computational standpoint.  To assess how tight the lower bound is, we empirically compare it to an upper bound that is computed with a greedy algorithm in Figure \ref{fig:greedy_versus_bound_K15}.  For a given $p$ and $K,$ the greedy algorithm chooses $\alpha_0 = 1, \; \alpha_1 = 1,$ and sequentially chooses \begin{align} \alpha_{j} = \argmin_{\alpha \in \mathbb{N} \; : \; 1 \leq \alpha \leq 1 + \sum_{i = 1}^{j-1}  \alpha_i} I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)
\end{align}
for $2 \leq j \leq K.$  As seen in Figure \ref{fig:greedy_versus_bound_K15}, $I(X \; ; \; X - G)$ serves as a very tight lower bound when compared with the upper bound.  We therefore view $I(X \; ; \; X - G)$ as an approximation to the original problem.

While the greedy algorithm requires $\Omega(2^K)$ time in the worst case, similar plots to Figure \ref{fig:greedy_versus_bound_K15} can be obtained for larger values of $K$ using a more computationally efficient variation of the greedy algorithm that is discussed in the longer version of this paper.

In order to prove the lower bound on the minimization of $I(X \; ; \; \alpha_0 X + \sum_{i=1}^K \alpha_i Z_i)$ in Theorem \ref{thm:main_lower_bound}, we form a convex relaxation of the minimization problem, perturb the relaxation to form a problem that is analytically solvable using KKT conditions, and use perturbation analysis to find a lower bound on the relaxation.  This is then a lower bound on the original problem.  The full proof is in the Section V.

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .06]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{upper bound (greedy)}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\label{fig:greedy_versus_bound_K15}
\end{figure}

%\begin{tikzpicture}
%\begin{axis} 
%[title ={Comparison of Bounds: $K = 15$},
%ylabel = mutual information, 
%xlabel = minor allele frequency (p),
%ymax = .001,
%legend pos=north west]

%\addplot [
%line width=1pt,
%color=red!80!black
%] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{upper bound}

%\addplot [
%line width=1pt,
%color=blue!80!black
%] table[x index=0,y index=1] %{data/plt2_bound.dat};
%\addlegendentry{lower bound}

%\end{axis}    
%\end{tikzpicture}
%\caption{}
%\label{fig:greedy_versus_bound_K15}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p1}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p1}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p001}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p001}
%\end{figure}


%The lower bound is formally proved in the appendix, but we outline the argument here, as it sheds light on the problem, and makes interesting use of convex optimization theory

\section{Efficiently Computable Schemes}

\rdcomment{this may sound stupid, but i think it warrants a sentence here. `Theorem 1 gives us a lower bound on the mutual information between $X$ and ..., which would be the mixing ratio that provides the highest level of privacy. However, it does not provide any mixing scheme for approaching this lower bound.'}

While much faster than brute force search, the greedy algorithm used to obtain the upper bound requires $\Omega(2^K)$ time in the worst case.  At a high level, this is due to the fact that at the $j$th  step in the algorithm, computation of $I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)$ requires use of each support value in the PMF of $\alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i,$ and there are $\Omega(2^j)$ support values in the worst case.  This motivates the design of efficiently computable schemes, which can then be evaluated using the lower bound in Theorem \ref{thm:main_lower_bound}.

Perhaps the most natural approach is given by the uniform scheme, which we define to set $\alpha_i = 1$ for all $i \in [K]\cup\{0\}.$  This is the scheme used by the authors of \cite{Maddah-Ali} to obtain their results.  The scheme is explicitly defined given $K,$ so no algorithm is needed to compute it.  The performance of the scheme for a given $p$ and $K$ can be computed in $O(K)$ time using the formula in Lemma \ref{lem:uniform_schem_formula} which is given in the appendix.

The uniform scheme is important because it is optimal as $p \to 0$ as proved in Lemma \ref{lem:optimality_of_uniform}
and exemplified by the optimal curve in Figure \ref{fig:optimal_scheme_K5_minor_allele}.

\begin{lemma}
\label{lem:optimality_of_uniform}
For any $K \in \mathbb{N},$ there exists some $p^* > 0$ such that the uniform scheme is optimal for $p < p^*.$
\end{lemma}

\rdcomment{i changed epsilon to $p^*$ here. epsilon is typically taken to mean a very small constant, which makes this result feel weak, i.e. this result is only true when p is arbitrarily small.}

At $p= 0.5,$ in Figure \ref{fig:optimal_scheme_K5_minor_allele}, the optimal solution is given by the binary scheme, which we define to set $\alpha_0 = 1$ and $\alpha_i = 2^{i-1}$ for all $i \in [K].$  Similar to the uniform scheme, the binary scheme is explicitly defined given $K.$  Also, similar to the uniform scheme, there exists a formula for computing its performance given $p$ and $K$ in $O(K)$ time.  This formula is given in Lemma \ref{lem:binary_scheme_performance} in the appendix.  It is interesting that such a formula exists because the PMF of $\sum_{i=1}^K 2^{i-1} Z_i$ has $2^K$ support values. 

Most importantly, the optimality of the binary scheme at $p = 0.5$ for $K=5$ shown in Figure \ref{fig:optimal_scheme_K5_minor_allele} generalizes to all $K$ as proved in Lemma \ref{lem:optimality_of_binary}.

\begin{lemma} \label{lem:optimality_of_binary}
	For any $K \in \mathbb{N},$ the binary scheme is optimal for $p = 0.5.$
\end{lemma}

Because the uniform scheme is optimal for $p \to 0$ and the binary scheme is optimal for $p = 0.5,$  it is natural to try and combine these schemes to interpolate the performance for $p$ in the range $0<p<0.5.$  Combining only the uniform scheme and the binary scheme does not produce a scheme that approaches the lower bound.  However, the general shape of the lower bound can be captured in polynomial time by combining the uniform scheme, the linear scheme, and the binary scheme where the linear scheme is defined as $\alpha_i = i$ for $i \in [K].$  We define the $(K,L,U)$-binary-linear-uniform scheme to set $\alpha_0 = 1$ and 
\begin{align} &\alpha_i = 1 \quad i \in \{1, ..., U\} \nonumber \\  &\alpha_{U+i} = i \quad i \in \{1, ..., L\} \nonumber \\
&\alpha_{U+L+i} = 2^{i-1} \quad i \in \{1, ..., K-U-L\}
\end{align}

\rdcomment{should it be binary-linear-uniform above?}

For a given $K$ and $p,$ we define the $K$-binary-linear-uniform scheme as the $(K,L^*,U^*)$-binary-linear-uniform scheme where
\begin{align} & (L^*, U^*) = \argmin_{(L,U) \in ([K]\cup\{0\})^2 \; : \; L + U \leq K} \\ &  I\left(X \; ; \; X + \sum_{i=1}^{U} Z_i + \sum_{j=1}^{L} j Z_{U+j} +  \sum_{k=1}^{K-U-L} 2^{k -1} Z_{U+L+k}\right) \nonumber.
\end{align}
The $K$-binary-linear-uniform scheme is computed in $O(K^4)$ time using a generalization of the recursion used to prove Lemma \ref{lem:binary_scheme_performance}.  

We compare the performance of the uniform scheme, the binary scheme, the $K$-binary-linear-uniform scheme, and the scheme generated by the greedy algorithm in Figure \ref{fig:efficiently_computable_schemes}.  We have observed that the greedy scheme generated by the greedy algorithm is much tighter than the   $K$-binary-linear-uniform scheme after the initial hump in the lower bound as $K$ increases.



\begin{figure}[h]
\label{fig:efficiently_computable_schemes}
\centering
\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .6,
legend pos = north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}


\end{axis}    
\end{tikzpicture}

\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .01]
%,
%legend pos=north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
%\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
%\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
%\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
%\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
%\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\end{figure}



%Greedy takes exponential time in $K$ to compute.

%Simpler schemes: uniform, binary, interpolation between uniform and binary.


%Maybe state theorems about uniform and binary. Or maybe just mention them and refer to the longer version

\section{Proof of Main Result}

We now present the proof of Theorem \ref{thm:main_lower_bound}, which makes interesting use of convex optimization theory.  

\rdcomment{this may be similar to the IS comments, but this proof is a bit hard to read for me. i understand the first few paragraphs in words, but it is not trivial to me to see exactly how this formally changes the problem. i would suggest stating the problem, and then how the support-constraint changes the optimization, and so on. to be honest, if you're tight on space, i still think it would be more beneficial to dedicate more space to this `reduction' and then even leave some of the more mechanical parts of derivatives/KKT condition analysis out.

also, we arrived at this result through figures and drawings; can we add some of this into the proof? i think it would strengthen the appeal of this paper to hint at why the idea is actually intuitive and cute. as written, it feels more a set of mechanical manipulations of KKT conditions, and it loses the sort of elegance i typically associate with info theory papers. (this is not a comment on the result, it's just a comment on the presentation and how it makes me feel.) i really liked the drawings of the convolution of discrete measures, and how we're really chosing a measure that gets shifted to the left by 1 and rescaled by 1-p and shifted to the right by 1 and rescaled by p. can this be put in this section at all?}
\begin{IEEEproof}
	Let $ Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i.$ We obtain the lower bound on $I(X \; ; \; \alpha_0 X + Z_{\alpha})= H(p) - H(X \; | \; \alpha_0 X+Z_{\alpha})$ in Theorem \ref{thm:main_lower_bound} by finding a lower bound on $-H(X \; | \; \alpha_0 X+Z_{\alpha}).$  In order to lower bound $-H(X \; | \; \alpha_0 X+Z_{\alpha}),$ we begin by considering the original optimization problem with the added constraint that the distance between the minimum support value and the maximum support value in the PMF of $Z_{\alpha}$ is less than $n+1$ where $n \in \mathbb{N}, \; n > 0.$  We will obtain a lower bound for this support constrained optimization problem, and use it to obtain a lower bound on the original optimization problem.  
	\iscomment{unclear why this can be done}
	
	To lower bound the support constrained optimization problem, we work with a relaxation of the support constrained  optimization problem.  Instead of requiring that the PMF for the noise random variable $D$ be generated by adding the sum of scaled $\text{Ber}(1-p)$ random variables, we relax the problem to only require that the probability at the highest support value of $D$'s PMF is equal to $(1-p)^K$ (this holds for any valid PMF of $Z_{\alpha}$).  
	Due to Lemma \ref{lem:alpha0_condition}, given $\alpha_0,$ any solution can be transformed into a solution whose PMF had support values in $\{t \alpha_0 : \; t \in \mathbb{Z}\}$ without increasing the mutual information.   Therefore, for a fixed $\alpha_0,$ it suffices to only consider PMFs that have support values in $\{t \alpha_0 : \; t \in \mathbb{Z}\}$ in the optimization.  If $\alpha_0 = a \in \mathbb{N}$ any solution random variable $D$ with  support values in $\{t a : \; t \in \mathbb{Z}\}$ can be transformed into a solution with the same mutual information, $\alpha_0 = 1,$ and support values in $\{t : \; t \in \mathbb{Z}\}.$ This is accomplished by dividing $D$ by $a.$     Therefore, we analyze the relaxation with $\alpha_0 = 1.$
	
	We then obtain a lower bound on this relaxation of the support constrained optimization problem .  Finally, we take the limit of the lower bound as $n$ goes to infinity in order to obtain a lower bound on the original minimization problem.
	
	The support-constrained relaxation of the original problem with $\alpha_0 = 1$ is given below. The objective function is a simplified form of $-H(X \; | \; X+D)$ where $D$ is the noise distribution we are optimizing over that is constrained to have probability of $(1-p)^K$ at the maximum support value. Here, $q_{(0)}$ is the probability at the maximum support value of $D$ and $q_{(-i)}$ is the probability at the $i$th integer below the maximum support value of $D.$  Observe that the problem is a convex minimization problem.
	\iscomment{not clear how this was obtained:}
	\begin{align}
	& \min_{q_{(-n-1)}, \; ..., \;  q_{(0)}} \sum_{j \in \{-n-1, \; ...,\;  -1\}} 
	\nonumber \\ & (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & + p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right)    \\
	\nonumber \\ &  \text{subject to:} \quad  q_{(j)} \geq 0 \; \; \forall j,  \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad q_{(-n-1)} = 0, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1. \nonumber
	\end{align}  
	
	\iscomment{do we need the full formula for the conditional entropy above? makes it harder to parse}
	While we cannot solve this problem analytically, we will perturb it to form an optimization problem that we can solve analytically.  We will then use perturbation analysis to obtain a lower bound on the problem above.
	
	
	The perturbed problem is given below where we have changed the constraint on the probability at the minimum support value, and the constraint on the sum of all the probabilities.
	
	\begin{align}
	& \min_{q_{(-n-1)}, \; ..., \;  q_{(0)}} \sum_{j \in \{-n-1, \; ...,\;  -1\}} 
	\nonumber \\ &  (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & +  p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right)    \\
	\nonumber \\	&  \text{subject to:} \quad  q_{(j)} \geq 0 \; \; \forall j,  \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad q_{(-n-1)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2} \nonumber
	\end{align}  
	
	
	Let $f_0(q)$ be the objective function above.  The Lagrangian is given by 
	
	\begin{align} 
	&L(q, v, \lambda) = f_0(q) 
	\nonumber \\ & + v_1 \left(\sum_i q_{(i)} - 1 + (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & + v_2 \left(q_{(0)} - (1-p)^K \right) 
	\nonumber \\ & + v_3 \left(q_{(-n-1)} - (1-p)^K (1 - (1-p)^K)^{n+1} \right) 
	\nonumber \\ & - \sum_i \lambda_i q_{(i)}. 
	\end{align}
	The derivative of $f_0(q)$ with respect to $q_{(j)}$ is given by 
	\begin{align}
	& p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) \nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right).
	\end{align}  
	for $j \in \{-n, \; ..., \;  -1\}$ and the KKT conditions are therefore given by 
	\begin{align}
	&  q_{(j)} \geq 0 \; \; \forall j,  \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & q_{(-n-1)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ &     \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2}
	\nonumber \\ & \lambda_j \geq 0 \quad \lambda_j q_{(j)} = 0 \quad \forall j 
	\nonumber \\ & (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right) - \lambda_j + v_1 + v_3 = 0 \quad 
	\nonumber \\ &  \text{for } j = - n -1
	\nonumber \\ & 	p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) 
	\nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right) - \lambda_j + v_1 = 0 
	\nonumber \\ &  \forall j \in \{-n, \; ..., \;  -1\}
	\nonumber \\ & p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) - \lambda_j + v_1 + v_2 = 0 
	\nonumber \\ & \text{for } j = 0
	\end{align}
	
	\rdcomment{stupid question: can you tell me a little more why (12) is this derivative? at a glance, it seems to be that there's a ton of term cancellations... (it's like the terms inside the log don't depend on $q_j$ with the way the derivative is written, so all those terms cancel?) i fear that a unfastidious reviewer may just claim this is a fundamental error and give a poor review without analyzing it deeply. (this happens sometimes to me.)}
	
	The last three conditions can be rewritten as 
	\begin{align} 
	& (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+1)}}{q_{(j)}} + (1-p) } \right) - \lambda_j + v_1 + v_3 = 0  
	\nonumber \\ &  \text{for } j = - n - 1
	\nonumber \\ & p \log \left(\frac{p }{(1-p)\frac{q_{(j-1)}}{q_{(j)}} + p } \right) + (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+1)}}{q_{(j)}} + (1-p) } \right) 
	\nonumber \\ & - \lambda_j + v_1  = 0 \quad \forall j \in \{-n, \; ..., \;  -1\}
	\nonumber \\ & p \log \left(\frac{p }{(1-p) \frac{q_{(j-1)}}{q_{(j)}} + p } \right) - \lambda_j + v_1 + v_2  = 0 \quad \text{for } j = 0
	\end{align}
	which shows that if the ratio $\frac{q_{(j-1)}}{q_{(j)}}$ between consecutive variables is the same for all $j$ and $\lambda_j = 0 $ for all $j,$ then $v_1,$ $v_2$ can  be chosen so that of these derivatives equal $0$ for all $j.$  Picking \[\frac{q_{(j-1)}}{q_{(j)}} = (1 - (1-p)^K),\] a solution to these equations is then
	\begin{align}
	& q_{(-i)} =  (1-p)^K (1 - (1-p)^K)^{i}  
	\nonumber \\ & \quad \quad \text{for } i \in \{0, \; 1, \; ..., \; n+1 \} 
	\nonumber \\ & \lambda_i = 0 \quad \forall i
	\nonumber \\ & v_1 = - p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & - (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right)
	\nonumber \\ & v_2 = (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & v_3 = p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right)
	\end{align}
	
	Because this is a convex optimization problem, this solution is optimal since it satisfies the KKT conditions.
	
	The optimal value for the optimization problem is therefore given by 
	\begin{align} 
	& \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
	\\ & - p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	\\ & = \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\\ & - p \beta \alpha^i \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\end{align}
	where $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K.$  
	Applying the geometric sum formula and simplifying, we obtain 
	\begin{align} 
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right).
	\end{align}
	
	
	
	%The optimal value for the optimization problem is therefore given by 
	%\begin{align} 
	%& -(1-p) \beta \alpha \frac{1 - \alpha^{2n+2}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	%\nonumber \\ & - p \beta \frac{1 - \alpha^{2n+2}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right).
	%\end{align}
	%after some simplification.
	
	Using the perturbation analysis from Section 5.6.1 of \cite{boyd}, we see that the optimal value of the support constrained relaxation of the original problem is lower bounded by
	\begin{align}
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\nonumber \\ & - v_1^* \left( (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & - v_3^* \left(- (1-p)^K (1 - (1-p)^K)^{n+1}  \right) 
	\end{align} 
	where $v_1^*$ and $v_3^*$ are the optimal lagrange multipliers for the perturbed problem which we determined above through the KKT conditions.
	
	The sequence of optimal values returned by the support constrained relaxation of the original problem is monotonically decreasing in $n$ clearly.  Thus, taking the limit of the bound as  $n \to \infty$ and simplifying yields the following lower bound on $-H(X \; | \; \alpha_0 X + Z_{\alpha})$ for any choice of $\alpha_i$'s: 	\begin{align} 
	& -(p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right).
	\end{align}
	
	Thus, a lower bound on mutual information is
	\begin{align} 
	& H(p) - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
	\end{align}
	for any choice of $\alpha_i$'s.
	
	Finally, observe that
	\begin{align}
	& H(X \; ; \; X - G) 
	\nonumber \\ & =\sum_{i = 0}^{\infty} (1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
	\nonumber \\ & + p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	\nonumber \\ & = (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right)  
	\nonumber \\ & + p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
	\end{align}
	where $G$ is a geometric random variable with success probability $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\},$  and $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K$ as before.
\end{IEEEproof}

\begin{lemma}
    \label{lem:alpha0_condition}
	Let $X$ be a $\text{Ber}(1-p)$ random variable.  Let $\alpha_0 \in \mathbb{N}.$ 
	Let $Z$ be any random variable such that its PMF has integral support and maximum support value at $t = 0.$  Let 
	\begin{align}
	& \hat{Z} = Z - (Z \mod{\alpha_0})   
	\end{align} 
	%\sum_{i = 1}^{2\alpha_0-1} i \text{\bf1} \{Z \mod{2\alpha_0}= i\}. 
	%$\Pr(\hat{Z} = t) = \sum_{i=0}^{2\alpha_0-1} \Pr(Z = t+i)$ 
	We then have that 
	\begin{align}
	& I(X ; \alpha_0 X + 	Z)  \geq I(X ; \alpha_0 X + \hat{Z}).   
	\end{align}	
\end{lemma}

\begin{IEEEproof}
	Let  $S = Z \mod{\alpha_0}.$  We then have that 
	\begin{align} 
		& I(X ; \; \alpha_0 X + 	Z)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z} +  S)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z}, \; S)
		\nonumber \\ & = I(X ; \; S) + I(X ; \; \alpha_0 X + \hat{Z} \; | \; S)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z} \; | \; S)
		\nonumber \\ & = H(X \; | \; S)  - H(X \; | \; \alpha_0 X + \hat{Z}, \; S) 
		\nonumber \\ & = H(X)  - H(X \; | \; \alpha_0 X + \hat{Z}, \; S)
		\nonumber \\ & \geq H(X)  - H(X \; | \; \alpha_0 X + \hat{Z})
		\nonumber \\ & = I(X \; ; \; \alpha_0 X + \hat{Z})
	\end{align} 
	where the third line follows because given $\alpha_0 X + \hat{Z} + S,$ we have that 
	\begin{align}
	    S = ((\alpha_0 X + \hat{Z} + S) - \alpha_0) \mod  \alpha_0 
	\end{align}
	and
    \begin{align}
	    \alpha_0 X + \hat{Z} = (\alpha_0 X + \hat{Z} + S) - S.
	\end{align}
	
	\end{IEEEproof}


==> main_result10_15_20.tex <==
\section{Main Result}


%\begin{figure}
%\centering
%\includegraphics[width=0.9\linewidth]{performance_plot_K6_minor_allele}
%\caption{}
%\label{fig:performance_plot_K6_minor_allele}
%\end{figure}

Our main result is stated below.

\begin{theorem} \label{thm:main_lower_bound}
	For any $K\in \mathbb{N},$ $p \in [0, 0.5],$  we have that 
	\begin{align} 
	%& \min_{\alpha_i \in \mathbb{N}, \; i \in [K]\cup\{0\}}
	& \min_{\alpha_1, ..., \alpha_K \in \mathbb{R}_{\geq 0}}
	I(X \; ; \; X + \sum_{i=1}^{K} \alpha_i Z_i) 
	\geq 
	I(X \; ; \; X - G)
	\end{align}
	where $G$ is a geometric random variable with success probability equal to $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\}.$
\end{theorem}
The formula for $I(X \; ; \; X - G)$ is given by 
\begin{align}
& I(X \; ; \; X - G)
\nonumber \\ & = H(p) 
\nonumber \\ & - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
\end{align}
Observe that the formula is quickly computable for any value of $K$ and $p,$ making it attractive from a computational standpoint.  To assess how tight the lower bound is, we empirically compare it to an upper bound that is computed with a greedy algorithm in Figure \ref{fig:greedy_versus_bound_K15}.  For a given $p$ and $K,$ the greedy algorithm chooses $\alpha_0 = 1, \; \alpha_1 = 1,$ and sequentially chooses \begin{align} \alpha_{j} = \argmin_{\alpha \in \mathbb{N} \; : \; 1 \leq \alpha \leq 1 + \sum_{i = 1}^{j-1}  \alpha_i} I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)
\end{align}
for $2 \leq j \leq K.$  As seen in Figure \ref{fig:greedy_versus_bound_K15}, $I(X \; ; \; X - G)$ serves as a very tight lower bound when compared with the upper bound.  We therefore view $I(X \; ; \; X - G)$ as an approximation to the original problem.

While the greedy algorithm requires $\Omega(2^K)$ time in the worst case, similar plots to Figure \ref{fig:greedy_versus_bound_K15} can be obtained for larger values of $K$ using a more computationally efficient variation of the greedy algorithm that is discussed in the longer version of this paper.

In order to prove the lower bound on the minimization of $I(X \; ; \; X + \sum_{i=1}^K \alpha_i Z_i)$ in Theorem \ref{thm:main_lower_bound}, we form a convex relaxation of the minimization problem, perturb the relaxation to form a problem that is analytically solvable using KKT conditions, and use perturbation analysis to find a lower bound on the relaxation.  This is then a lower bound on the original problem.  The full proof is in the Section V.

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .06]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{upper bound (greedy)}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\label{fig:greedy_versus_bound_K15}
\end{figure}

%\begin{tikzpicture}
%\begin{axis} 
%[title ={Comparison of Bounds: $K = 15$},
%ylabel = mutual information, 
%xlabel = minor allele frequency (p),
%ymax = .001,
%legend pos=north west]

%\addplot [
%line width=1pt,
%color=red!80!black
%] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{upper bound}

%\addplot [
%line width=1pt,
%color=blue!80!black
%] table[x index=0,y index=1] %{data/plt2_bound.dat};
%\addlegendentry{lower bound}

%\end{axis}    
%\end{tikzpicture}
%\caption{}
%\label{fig:greedy_versus_bound_K15}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p1}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p1}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p001}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p001}
%\end{figure}


%The lower bound is formally proved in the appendix, but we outline the argument here, as it sheds light on the problem, and makes interesting use of convex optimization theory

\section{Efficiently Computable Schemes}

\rdcomment{this may sound stupid, but i think it warrants a sentence here. `Theorem 1 gives us a lower bound on the mutual information between $X$ and ..., which would be the mixing ratio that provides the highest level of privacy. However, it does not provide any mixing scheme for approaching this lower bound.'}

While much faster than brute force search, the greedy algorithm used to obtain the upper bound requires $\Omega(2^K)$ time in the worst case.  At a high level, this is due to the fact that at the $j$th  step in the algorithm, computation of $I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)$ requires use of each support value in the PMF of $\alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i,$ and there are $\Omega(2^j)$ support values in the worst case.  This motivates the design of efficiently computable schemes, which can then be evaluated using the lower bound in Theorem \ref{thm:main_lower_bound}.

Perhaps the most natural approach is given by the uniform scheme, which we define to set $\alpha_i = 1$ for all $i \in [K]\cup\{0\}.$  This is the scheme used by the authors of \cite{Maddah-Ali} to obtain their results.  The scheme is explicitly defined given $K,$ so no algorithm is needed to compute it.  The performance of the scheme for a given $p$ and $K$ can be computed in $O(K)$ time using the formula in Lemma \ref{lem:uniform_schem_formula} which is given in the appendix.

The uniform scheme is important because it is optimal as $p \to 0$ as proved in Lemma \ref{lem:optimality_of_uniform}
and exemplified by the optimal curve in Figure \ref{fig:optimal_scheme_K5_minor_allele}.

\begin{lemma}
\label{lem:optimality_of_uniform}
For any $K \in \mathbb{N},$ there exists some $p^* > 0$ such that the uniform scheme is optimal for $p < p^*.$
\end{lemma}

\rdcomment{i changed epsilon to $p^*$ here. epsilon is typically taken to mean a very small constant, which makes this result feel weak, i.e. this result is only true when p is arbitrarily small.}

At $p= 0.5,$ in Figure \ref{fig:optimal_scheme_K5_minor_allele}, the optimal solution is given by the binary scheme, which we define to set $\alpha_0 = 1$ and $\alpha_i = 2^{i-1}$ for all $i \in [K].$  Similar to the uniform scheme, the binary scheme is explicitly defined given $K.$  Also, similar to the uniform scheme, there exists a formula for computing its performance given $p$ and $K$ in $O(K)$ time.  This formula is given in Lemma \ref{lem:binary_scheme_performance} in the appendix.  It is interesting that such a formula exists because the PMF of $\sum_{i=1}^K 2^{i-1} Z_i$ has $2^K$ support values. 

Most importantly, the optimality of the binary scheme at $p = 0.5$ for $K=5$ shown in Figure \ref{fig:optimal_scheme_K5_minor_allele} generalizes to all $K$ as proved in Lemma \ref{lem:optimality_of_binary}.

\begin{lemma} \label{lem:optimality_of_binary}
	For any $K \in \mathbb{N},$ the binary scheme is optimal for $p = 0.5.$
\end{lemma}

Because the uniform scheme is optimal for $p \to 0$ and the binary scheme is optimal for $p = 0.5,$  it is natural to try and combine these schemes to interpolate the performance for $p$ in the range $0<p<0.5.$  Combining only the uniform scheme and the binary scheme does not produce a scheme that approaches the lower bound.  However, the general shape of the lower bound can be captured in polynomial time by combining the uniform scheme, the linear scheme, and the binary scheme where the linear scheme is defined as $\alpha_i = i$ for $i \in [K].$  We define the $(K,L,U)$-binary-linear-uniform scheme to set $\alpha_0 = 1$ and 
\begin{align} &\alpha_i = 1 \quad i \in \{1, ..., U\} \nonumber \\  &\alpha_{U+i} = i \quad i \in \{1, ..., L\} \nonumber \\
&\alpha_{U+L+i} = 2^{i-1} \quad i \in \{1, ..., K-U-L\}
\end{align}

\rdcomment{should it be binary-linear-uniform above?}

For a given $K$ and $p,$ we define the $K$-binary-linear-uniform scheme as the $(K,L^*,U^*)$-binary-linear-uniform scheme where
\begin{align} & (L^*, U^*) = \argmin_{(L,U) \in ([K]\cup\{0\})^2 \; : \; L + U \leq K} \\ &  I\left(X \; ; \; X + \sum_{i=1}^{U} Z_i + \sum_{j=1}^{L} j Z_{U+j} +  \sum_{k=1}^{K-U-L} 2^{k -1} Z_{U+L+k}\right) \nonumber.
\end{align}
The $K$-binary-linear-uniform scheme is computed in $O(K^4)$ time using a generalization of the recursion used to prove Lemma \ref{lem:binary_scheme_performance}.  

We compare the performance of the uniform scheme, the binary scheme, the $K$-binary-linear-uniform scheme, and the scheme generated by the greedy algorithm in Figure \ref{fig:efficiently_computable_schemes}.  We have observed that the greedy scheme generated by the greedy algorithm is much tighter than the   $K$-binary-linear-uniform scheme after the initial hump in the lower bound as $K$ increases.



\begin{figure}[h]
\label{fig:efficiently_computable_schemes}
\centering
\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .6,
legend pos = north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}


\end{axis}    
\end{tikzpicture}

\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .01]
%,
%legend pos=north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
%\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
%\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
%\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
%\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
%\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\end{figure}



%Greedy takes exponential time in $K$ to compute.

%Simpler schemes: uniform, binary, interpolation between uniform and binary.


%Maybe state theorems about uniform and binary. Or maybe just mention them and refer to the longer version

\rdcomment{this may be similar to the IS comments, but this proof is a bit hard to read for me. i understand the first few paragraphs in words, but it is not trivial to me to see exactly how this formally changes the problem. i would suggest stating the problem, and then how the support-constraint changes the optimization, and so on. to be honest, if you're tight on space, i still think it would be more beneficial to dedicate more space to this `reduction' and then even leave some of the more mechanical parts of derivatives/KKT condition analysis out.

also, we arrived at this result through figures and drawings; can we add some of this into the proof? i think it would strengthen the appeal of this paper to hint at why the idea is actually intuitive and cute. as written, it feels more a set of mechanical manipulations of KKT conditions, and it loses the sort of elegance i typically associate with info theory papers. (this is not a comment on the result, it's just a comment on the presentation and how it makes me feel.) i really liked the drawings of the convolution of discrete measures, and how we're really chosing a measure that gets shifted to the left by 1 and rescaled by 1-p and shifted to the right by 1 and rescaled by p. can this be put in this section at all?}

\rdcomment{stupid question: can you tell me a little more why (12) is this derivative? at a glance, it seems to be that there's a ton of term cancellations... (it's like the terms inside the log don't depend on $q_j$ with the way the derivative is written, so all those terms cancel?) i fear that a unfastidious reviewer may just claim this is a fundamental error and give a poor review without analyzing it deeply. (this happens sometimes to me.)}

\section{Proof of Main Result}

We now present the proof of Theorem \ref{thm:main_lower_bound}, which makes interesting use of convex optimization theory.  

\begin{IEEEproof}
    First, notice that choosing integral $\alpha_i \; : \;  i \in [K] \cup \{0\}$ in the optimization problem (\ref{eq:main}) is optimal due to Lemma \ref{lem:integer_sol_optimal}, which clearly holds.  We will thus consider (\ref{eq:main}) with the constraint that $\alpha_i \in \mathbb{N}$ for $i \in [K] \cup \{0\}.$
    
    \begin{lemma}
        \label{lem:integer_sol_optimal}
        If an optimal solution to (\ref{eq:main}) exists, then there exists an optimal solution to Equation \ref{eq:main} with $\alpha_i \in \mathbb{N}$ for $i \in [K] \cup \{0\}.$
    \end{lemma}
    
    Let $ Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i.$ We obtain the lower bound on $I(X \; ; \; \alpha_0 X + Z_{\alpha})= H(p) - H(X \; | \; \alpha_0 X+Z_{\alpha})$ in Theorem \ref{thm:main_lower_bound} by finding a lower bound on $-H(X \; | \; \alpha_0 X+Z_{\alpha}).$  The optimization problem we consider is therefore
    \begin{align}
        \label{eq:integral_alpha_opt_prob}
        & \min_{\alpha_1,...,\alpha_K \in \mathbb{N}} -H\left(X \; | \; \alpha_{0} X+\sum_{k=1}^K \alpha_k Z_k\right).
    \end{align}
    
    Observe that the PMF for any random variable $Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i$ has probability $(1-p)^{K+1}$ at the highest support value.  Thus, the following problem is clearly a relaxation to (\ref{eq:integral_alpha_opt_prob})

    \begin{align}
        \label{eq:relax_inf1}
        & \min_{D} -H\left(X \; | \; \alpha_0 X+D\right)
        \\ & \text{subject to:} 
        \nonumber \\ & D \text{ is a random variable with integral support,}
        \nonumber \\ & D  \text{ has maximum support value at 0,} 
        \nonumber \\ & \Pr(D = 0) = (1-p)^K.
        \nonumber
    \end{align}
    Due to Lemma \ref{lem:alpha0_condition}, we can fix $\alpha_0 = 1$ in (\ref{eq:relax_inf1}) above without changing the optimal value.  
    Written more explicitly, (\ref{eq:relax_inf1}) with $\alpha_0 = 1$ fixed is given by
    \begin{align}
    \label{eq:relax_inf2}
	& \min_{q_{(-i)} \geq 0 : \; i \in \mathbb{N}\cup\{0\} } \sum_{j \in \{-n : \; n \in \mathbb{N}\}} 
	\nonumber \\ & (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & + p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right)    \\
	\nonumber \\ &  \text{subject to:} \quad \nonumber \\ & \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad    \sum_{j \in \{-n : \; n \in \mathbb{N}\cup\{0\}\}} q_{(j)} = 1 \nonumber
	\end{align}  
    where $q_{(0)}$ is the probability at the maximum support value of $D$ and $q_{(-i)}$ is the probability at the $i$th integer below the maximum support value of $D.$  Note that the conditional entropy in the objective function is in a simplified form.   
    
    Observe that the problem is an infinite dimensional convex minimization problem.  A solution to the KKT conditions with the added implicit constraint that $q_{(-i)}>0$ for $i \in \mathbb{N} \cup \{0\}$  is given by  $q_{(-i)} = (1-p)^K (1 - (1-p)^K)^i$ for $i \in \mathbb{N} \cup \{0\}$ which corresponds to $D = -G$ in (\ref{eq:relax_inf1}) where $G$ is a geometric random variable with success probability equal to $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\}.$  We do not use this observation directly to establish the result because no reference on KKT conditions in the infinite dimensional case was found.  
    
    Instead, we form a new optimization problem where we constrain $D$ to have distance $n$ between its maximum and minimum support values, derive a lower bound on the solution for $n \in \mathbb{N}$, and use this sequence of lower bounds to establish the result. The support constrained version of (\ref{eq:relax_inf2}) is given by 
    \begin{align}
    \label{eq:relax_const}
    & \min_{q_{(-i)} \geq 0 : \; i \in [n+1]\cup\{0\} }
    \sum_{j \in \{-m : \; m \in [n+1]\}} 
	\nonumber \\ & (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & + p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right)    \\
	\nonumber \\ &  \text{subject to:} \nonumber \\ & 
    \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad q_{(-n-1)} = 0, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1. \nonumber
	\end{align}  
    While we do not know the solution to (\ref{eq:relax_const}), we will perturb it to form a problem we can solve analytically, then use perturbation analysis to lower bound the optimal value of (\ref{eq:relax_const}).
    
    The perturbed version of (\ref{eq:relax_const}) is given by 
	\begin{align}
	\label{eq:relax_const_pert}
    & \min_{q_{(-i)} \geq 0 : \; i \in [n+1]\cup\{0\} }
    \sum_{j \in \{-m : \; m \in [n+1]\}} 
	\nonumber \\ &  (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & +  p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right)    \\
	\nonumber \\	&  \text{subject to:} \nonumber \\
	& \quad q_{(0)} = (1-p)^K,
	\nonumber \\ & \quad q_{(-n-1)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2} \nonumber
	\end{align}  
    where we have changed the constraint on the probability at the minimum support value, and the constraint on the sum of all the probabilities.
    
    Changing the implicit constraint in (\ref{eq:relax_const_pert}) from $q_{(i)} \geq 0$ to $q_{(i)} > 0$ gives us
	\begin{align}
	\label{eq:relax_const_pert_posq}
    & \min_{q_{(-i)} > 0 : \; i \in [n+1]\cup\{0\} }
    \sum_{j \in \{-m : \; m \in [n+1]\}} 
	\nonumber \\ &  (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & +  p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right)    \\
	\nonumber \\	&  \text{subject to:} \nonumber \\
	& \quad q_{(0)} = (1-p)^K,
	\nonumber \\ & \quad q_{(-n-1)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2} \nonumber
	\end{align}  
    which we can solve through KKT conditions since the problem is convex, Slater's condition holds, and the objective function and constraint functions are differentiable on their domains.  Due to the continuity of the objective function in (\ref{eq:relax_const_pert}), it is not hard to show that an optimal solution to (\ref{eq:relax_const_pert_posq}) is also an optimal solution to (\ref{eq:relax_const_pert}).  At a high level, this is due to the fact that if there was a solution to  (\ref{eq:relax_const_pert}) with $q_{(i)} = 0$ for some $i$ and this solution was better than the optimal solution to   (\ref{eq:relax_const_pert_posq}), then this would create a contradiction because (\ref{eq:relax_const_pert_posq}) could get arbitrarily close to the better solution by the continuity of the objective function.  
    
    We proceed to find the solution to the KKT conditions for (\ref{eq:relax_const_pert_posq}), which is then a solution to (\ref{eq:relax_const_pert}).  Let $f_0(q)$ be the objective function of (\ref{eq:relax_const_pert_posq}).  The Lagrangian is given by 
	
	\begin{align} 
	&L(q, v, \lambda) = f_0(q) 
	\nonumber \\ & + v_1 \left(\sum_i q_{(i)} - 1 + (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & + v_2 \left(q_{(0)} - (1-p)^K \right) 
	\nonumber \\ & + v_3 \left(q_{(-n-1)} - (1-p)^K (1 - (1-p)^K)^{n+1} \right). 
	\end{align}
	The derivative of $f_0(q)$ with respect to $q_{(j)}$ is given by 
	\begin{align}
	& p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) \nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right)
	\end{align}  
	for $j \in \{-n, \; ..., \;  -1\}$ and the KKT conditions are given by 
	\begin{align}
	& q_{(0)} = (1-p)^K,
	\nonumber \\ & q_{(-n-1)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ &     \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2}
	\nonumber \\ & (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right) + v_1 + v_3 = 0 \quad 
	\nonumber \\ &  \text{for } j = - n -1
	\nonumber \\ & 	p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) 
	\nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right)+ v_1 = 0 
	\nonumber \\ &  \forall j \in \{-n, \; ..., \;  -1\}
	\nonumber \\ & p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) + v_1 + v_2 = 0 
	\nonumber \\ & \text{for } j = 0.
	\end{align}
	

	
	The last three conditions can be rewritten as 
	\begin{align} 
	& (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+1)}}{q_{(j)}} + (1-p) } \right) + v_1 + v_3 = 0  
	\nonumber \\ &  \text{for } j = - n - 1
	\nonumber \\ & p \log \left(\frac{p }{(1-p)\frac{q_{(j-1)}}{q_{(j)}} + p } \right) \nonumber \\ & + (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+1)}}{q_{(j)}} + (1-p) } \right)   + v_1  = 0 
	\nonumber \\ & \forall j \in \{-n, \; ..., \;  -1\}
	\nonumber \\ & p \log \left(\frac{p }{(1-p) \frac{q_{(j-1)}}{q_{(j)}} + p } \right)  + v_1 + v_2  = 0 \quad \text{for } j = 0
	\end{align}
	which shows that if the ratio $\frac{q_{(j-1)}}{q_{(j)}}$ between consecutive variables is the same for all $j,$  then $v_1,$ $v_2$ can  be chosen so that of these derivatives equal $0$ for all $j.$  Picking \[\frac{q_{(j-1)}}{q_{(j)}} = (1 - (1-p)^K),\] a solution to these equations is then
	\begin{align}
	& q_{(-i)} =  (1-p)^K (1 - (1-p)^K)^{i}  
	\nonumber \\ & \text{for } i \in \{0, \; 1, \; ..., \; n+1 \} 
	\nonumber \\ & v_1 = - p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & - (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right)
	\nonumber \\ & v_2 = (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & v_3 = p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right)
	\end{align}
	
    This is the solution to both (\ref{eq:relax_const_pert_posq}) and (\ref{eq:relax_const_pert}) as discussed earlier.  The optimal value for (\ref{eq:relax_const_pert_posq}) and (\ref{eq:relax_const_pert}) is therefore given by 
	\begin{align} 
	& \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
	\nonumber \\ & - p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	\nonumber \\ & = \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \alpha^i \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\end{align}
	where $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K.$  
	Applying the geometric sum formula and simplifying,  the optimal value for (\ref{eq:relax_const_pert_posq}) and (\ref{eq:relax_const_pert}) is   
	\begin{align} 
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right).
	\end{align}
	
	Using the perturbation analysis from Section 5.6.1 of \cite{boyd}, we see that the optimal value of (\ref{eq:relax_const}) is lower bounded by
	\begin{align}
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\nonumber \\ & - v_1^* \left( (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & - v_3^* \left(- (1-p)^K (1 - (1-p)^K)^{n+1}  \right) 
	\end{align} 
	where $v_1^*$ and $v_3^*$ are the optimal lagrange multipliers for (\ref{eq:relax_const_pert_posq}) and (\ref{eq:relax_const_pert})
	we determined through the KKT conditions.
	
	The sequence of optimal values returned by (\ref{eq:relax_const}) is monotonically decreasing in $n$ clearly.  Thus, taking the limit of the lower bound as  $n \to \infty$ and simplifying yields the following lower bound on $-H(X \; | \; \alpha_0 X + Z_{\alpha})$ for any choice of $\alpha_i$'s: 	\begin{align} 
	& -(p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right).
	\end{align}
	
	Thus, a lower bound on mutual information is
	\begin{align} 
	& H(p) - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
	\end{align}
	for any choice of $\alpha_i$'s.
	
	Finally, observe that
	\begin{align}
	& H(X \; ; \; X - G) 
	\nonumber \\ & =\sum_{i = 0}^{\infty} (1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
	\nonumber \\ & + p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	\nonumber \\ & = (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right)  
	\nonumber \\ & + p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
	\end{align}
	where $G$ is a geometric random variable with success probability $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\},$  and $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K$ as before.
	
	%Due to Lemma \ref{lem:alpha0_condition}, given $\alpha_0,$ any solution can be transformed into a solution whose PMF had support values in $\{t \alpha_0 : \; t \in \mathbb{Z}\}$ without increasing the mutual information.   Therefore, for a fixed $\alpha_0,$ it suffices to only consider PMFs that have support values in $\{t \alpha_0 : \; t \in \mathbb{Z}\}$ in the optimization.  If $\alpha_0 = a \in \mathbb{N}$ any solution random variable $D$ with  support values in $\{t a : \; t \in \mathbb{Z}\}$ can be transformed into a solution with the same mutual information, $\alpha_0 = 1,$ and support values in $\{t : \; t \in \mathbb{Z}\}.$ This is accomplished by dividing $D$ by $a.$     Therefore, we analyze the relaxation with $\alpha_0 = 1.$
	
\end{IEEEproof}

\begin{lemma}
    \label{lem:alpha0_condition}
    Fixing $\alpha_0 = 1$ in (\ref{eq:relax_const}) can not increase the optimal value.
\end{lemma}

\begin{IEEEproof}
    Let $\alpha_0 \in \mathbb{N}.$ 
	Let $Z$ be any random variable such that its PMF has integral support and maximum support value at $t = 0.$  Let 
	\begin{align}
	& \hat{Z} = Z - S
	\end{align} 
	where $S = Z \mod{\alpha_0}.$ 
	We then have that 
	\begin{align}
	& I(X ; \alpha_0 X + 	Z)  \geq I(X ; \alpha_0 X + \hat{Z}).   
	\end{align}
	because  
	\begin{align} 
		& I(X ; \; \alpha_0 X + 	Z)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z} +  S)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z}, \; S)
		\nonumber \\ & = I(X ; \; S) + I(X ; \; \alpha_0 X + \hat{Z} \; | \; S)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z} \; | \; S)
		\nonumber \\ & = H(X \; | \; S)  - H(X \; | \; \alpha_0 X + \hat{Z}, \; S) 
		\nonumber \\ & = H(X)  - H(X \; | \; \alpha_0 X + \hat{Z}, \; S)
		\nonumber \\ & \geq H(X)  - H(X \; | \; \alpha_0 X + \hat{Z})
		\nonumber \\ & = I(X \; ; \; \alpha_0 X + \hat{Z})
	\end{align} 
	where the third line follows because given $\alpha_0 X + \hat{Z} + S,$ we have that 
	\begin{align}
	    S = ((\alpha_0 X + \hat{Z} + S) - \alpha_0) \mod  \alpha_0 
	\end{align}
	and
    \begin{align}
	    \alpha_0 X + \hat{Z} = (\alpha_0 X + \hat{Z} + S) - S.
	\end{align}
	Thus, any solution to (\ref{eq:relax_inf1}) with  $\alpha_0 = a$ can be transformed into a solution whose PMF had support values in $\{t a : \; t \in \mathbb{Z}\}$ without increasing the mutual information.   Therefore, for a fixed $\alpha_0,$ it suffices to only consider PMFs that have support values in $\{t \alpha_0 : \; t \in \mathbb{Z}\}$ in the optimization.  If $\alpha_0 = a \in \mathbb{N}$ any solution random variable $D$ with  support values in $\{t a : \; t \in \mathbb{Z}\}$ can be transformed into a solution with the same mutual information, $\alpha_0 = 1,$ and support values in $\{t : \; t \in \mathbb{Z}\}.$ This is accomplished by dividing $D$ by $a.$  Therefore it suffices to fix $\alpha_0=1$ in the optimization. 
	\end{IEEEproof}


==> main_result10_15_20_v2.tex <==
\section{Main Result}


%\begin{figure}
%\centering
%\includegraphics[width=0.9\linewidth]{performance_plot_K6_minor_allele}
%\caption{}
%\label{fig:performance_plot_K6_minor_allele}
%\end{figure}

Our main result is stated below.

\begin{theorem} \label{thm:main_lower_bound}
	For any $K\in \mathbb{N},$ $p \in [0, 0.5],$  we have that 
	\begin{align} 
	%& \min_{\alpha_i \in \mathbb{N}, \; i \in [K]\cup\{0\}}
	& \min_{\alpha_0, ..., \alpha_K \in \mathbb{Q}_{\geq 0}}
	I(X \; ; \; \alpha_0 X + \sum_{i=1}^{K} \alpha_i Z_i) 
	\geq 
	I(X \; ; \; X - G)
	\end{align}
	where $G$ is a geometric random variable with success probability equal to $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\}.$
\end{theorem}
The formula for $I(X \; ; \; X - G)$ is given by 
\begin{align}
& I(X \; ; \; X - G)
\nonumber \\ & = H(p) 
\nonumber \\ & - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
\end{align}
Observe that the formula is quickly computable for any value of $K$ and $p,$ making it attractive from a computational standpoint.  To assess how tight the lower bound is, we empirically compare it to an upper bound that is computed with a greedy algorithm in Figure \ref{fig:greedy_versus_bound_K15}.  For a given $p$ and $K,$ the greedy algorithm chooses $\alpha_0 = 1, \; \alpha_1 = 1,$ and sequentially chooses \begin{align} \alpha_{j} = \argmin_{\alpha \in \mathbb{N} \; : \; 1 \leq \alpha \leq 1 + \sum_{i = 1}^{j-1}  \alpha_i} I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)
\end{align}
for $2 \leq j \leq K.$  As seen in Figure \ref{fig:greedy_versus_bound_K15}, $I(X \; ; \; X - G)$ serves as a very tight lower bound when compared with the upper bound.  We therefore view $I(X \; ; \; X - G)$ as an approximation to the original problem.

While the greedy algorithm requires $\Omega(2^K)$ time in the worst case, similar plots to Figure \ref{fig:greedy_versus_bound_K15} can be obtained for larger values of $K$ using a more computationally efficient variation of the greedy algorithm that is discussed in the longer version of this paper.

In order to prove the lower bound on the minimization of $I(X \; ; \; X + \sum_{i=1}^K \alpha_i Z_i)$ in Theorem \ref{thm:main_lower_bound}, we form a convex relaxation of the minimization problem, perturb the relaxation to form a problem that is analytically solvable using KKT conditions, and use perturbation analysis to find a lower bound on the relaxation.  This is then a lower bound on the original problem.  The full proof is in the Section V.

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .06]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{upper bound (greedy)}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\label{fig:greedy_versus_bound_K15}
\end{figure}

%\begin{tikzpicture}
%\begin{axis} 
%[title ={Comparison of Bounds: $K = 15$},
%ylabel = mutual information, 
%xlabel = minor allele frequency (p),
%ymax = .001,
%legend pos=north west]

%\addplot [
%line width=1pt,
%color=red!80!black
%] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{upper bound}

%\addplot [
%line width=1pt,
%color=blue!80!black
%] table[x index=0,y index=1] %{data/plt2_bound.dat};
%\addlegendentry{lower bound}

%\end{axis}    
%\end{tikzpicture}
%\caption{}
%\label{fig:greedy_versus_bound_K15}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p1}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p1}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p001}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p001}
%\end{figure}


%The lower bound is formally proved in the appendix, but we outline the argument here, as it sheds light on the problem, and makes interesting use of convex optimization theory

\section{Efficiently Computable Schemes}

\rdcomment{this may sound stupid, but i think it warrants a sentence here. `Theorem 1 gives us a lower bound on the mutual information between $X$ and ..., which would be the mixing ratio that provides the highest level of privacy. However, it does not provide any mixing scheme for approaching this lower bound.'}

While much faster than brute force search, the greedy algorithm used to obtain the upper bound requires $\Omega(2^K)$ time in the worst case.  At a high level, this is due to the fact that at the $j$th  step in the algorithm, computation of $I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)$ requires use of each support value in the PMF of $\alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i,$ and there are $\Omega(2^j)$ support values in the worst case.  This motivates the design of efficiently computable schemes, which can then be evaluated using the lower bound in Theorem \ref{thm:main_lower_bound}.

Perhaps the most natural approach is given by the uniform scheme, which we define to set $\alpha_i = 1$ for all $i \in [K]\cup\{0\}.$  This is the scheme used by the authors of \cite{Maddah-Ali} to obtain their results.  The scheme is explicitly defined given $K,$ so no algorithm is needed to compute it.  The performance of the scheme for a given $p$ and $K$ can be computed in $O(K)$ time using the formula in Lemma \ref{lem:uniform_schem_formula} which is given in the appendix.

The uniform scheme is important because it is optimal as $p \to 0$ as proved in Lemma \ref{lem:optimality_of_uniform}
and exemplified by the optimal curve in Figure \ref{fig:optimal_scheme_K5_minor_allele}.

\begin{lemma}
\label{lem:optimality_of_uniform}
For any $K \in \mathbb{N},$ there exists some $p^* > 0$ such that the uniform scheme is optimal for $p < p^*.$
\end{lemma}

\rdcomment{i changed epsilon to $p^*$ here. epsilon is typically taken to mean a very small constant, which makes this result feel weak, i.e. this result is only true when p is arbitrarily small.}

At $p= 0.5,$ in Figure \ref{fig:optimal_scheme_K5_minor_allele}, the optimal solution is given by the binary scheme, which we define to set $\alpha_0 = 1$ and $\alpha_i = 2^{i-1}$ for all $i \in [K].$  Similar to the uniform scheme, the binary scheme is explicitly defined given $K.$  Also, similar to the uniform scheme, there exists a formula for computing its performance given $p$ and $K$ in $O(K)$ time.  This formula is given in Lemma \ref{lem:binary_scheme_performance} in the appendix.  It is interesting that such a formula exists because the PMF of $\sum_{i=1}^K 2^{i-1} Z_i$ has $2^K$ support values. 

Most importantly, the optimality of the binary scheme at $p = 0.5$ for $K=5$ shown in Figure \ref{fig:optimal_scheme_K5_minor_allele} generalizes to all $K$ as proved in Lemma \ref{lem:optimality_of_binary}.

\begin{lemma} \label{lem:optimality_of_binary}
	For any $K \in \mathbb{N},$ the binary scheme is optimal for $p = 0.5.$
\end{lemma}

Because the uniform scheme is optimal for $p \to 0$ and the binary scheme is optimal for $p = 0.5,$  it is natural to try and combine these schemes to interpolate the performance for $p$ in the range $0<p<0.5.$  Combining only the uniform scheme and the binary scheme does not produce a scheme that approaches the lower bound.  However, the general shape of the lower bound can be captured in polynomial time by combining the uniform scheme, the linear scheme, and the binary scheme where the linear scheme is defined as $\alpha_i = i$ for $i \in [K].$  We define the $(K,L,U)$-binary-linear-uniform scheme to set $\alpha_0 = 1$ and 
\begin{align} &\alpha_i = 1 \quad i \in \{1, ..., U\} \nonumber \\  &\alpha_{U+i} = i \quad i \in \{1, ..., L\} \nonumber \\
&\alpha_{U+L+i} = 2^{i-1} \quad i \in \{1, ..., K-U-L\}
\end{align}

\rdcomment{should it be binary-linear-uniform above?}

For a given $K$ and $p,$ we define the $K$-binary-linear-uniform scheme as the $(K,L^*,U^*)$-binary-linear-uniform scheme where
\begin{align} & (L^*, U^*) = \argmin_{(L,U) \in ([K]\cup\{0\})^2 \; : \; L + U \leq K} \\ &  I\left(X \; ; \; X + \sum_{i=1}^{U} Z_i + \sum_{j=1}^{L} j Z_{U+j} +  \sum_{k=1}^{K-U-L} 2^{k -1} Z_{U+L+k}\right) \nonumber.
\end{align}
The $K$-binary-linear-uniform scheme is computed in $O(K^4)$ time using a generalization of the recursion used to prove Lemma \ref{lem:binary_scheme_performance}.  

We compare the performance of the uniform scheme, the binary scheme, the $K$-binary-linear-uniform scheme, and the scheme generated by the greedy algorithm in Figure \ref{fig:efficiently_computable_schemes}.  We have observed that the greedy scheme generated by the greedy algorithm is much tighter than the   $K$-binary-linear-uniform scheme after the initial hump in the lower bound as $K$ increases.



\begin{figure}[h]
\label{fig:efficiently_computable_schemes}
\centering
\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .6,
legend pos = north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}


\end{axis}    
\end{tikzpicture}

\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .01]
%,
%legend pos=north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
%\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
%\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
%\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
%\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
%\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\end{figure}



%Greedy takes exponential time in $K$ to compute.

%Simpler schemes: uniform, binary, interpolation between uniform and binary.


%Maybe state theorems about uniform and binary. Or maybe just mention them and refer to the longer version

\rdcomment{this may be similar to the IS comments, but this proof is a bit hard to read for me. i understand the first few paragraphs in words, but it is not trivial to me to see exactly how this formally changes the problem. i would suggest stating the problem, and then how the support-constraint changes the optimization, and so on. to be honest, if you're tight on space, i still think it would be more beneficial to dedicate more space to this `reduction' and then even leave some of the more mechanical parts of derivatives/KKT condition analysis out.

also, we arrived at this result through figures and drawings; can we add some of this into the proof? i think it would strengthen the appeal of this paper to hint at why the idea is actually intuitive and cute. as written, it feels more a set of mechanical manipulations of KKT conditions, and it loses the sort of elegance i typically associate with info theory papers. (this is not a comment on the result, it's just a comment on the presentation and how it makes me feel.) i really liked the drawings of the convolution of discrete measures, and how we're really chosing a measure that gets shifted to the left by 1 and rescaled by 1-p and shifted to the right by 1 and rescaled by p. can this be put in this section at all?}

\rdcomment{stupid question: can you tell me a little more why (12) is this derivative? at a glance, it seems to be that there's a ton of term cancellations... (it's like the terms inside the log don't depend on $q_j$ with the way the derivative is written, so all those terms cancel?) i fear that a unfastidious reviewer may just claim this is a fundamental error and give a poor review without analyzing it deeply. (this happens sometimes to me.)}

\section{Proof of Main Result}

We now present the proof of Theorem \ref{thm:main_lower_bound}.  

\begin{IEEEproof}
    First, notice that choosing integral $\alpha_i \; : \;  i \in [K] \cup \{0\}$ in the optimization problem (\ref{eq:main}) is optimal due to Lemma \ref{lem:integer_sol_optimal}.  Lemma \ref{lem:integer_sol_optimal} holds because if $\alpha_i = \frac{c_i}{b_i} \; \forall i$ in (\ref{eq:main}) where $c_i, b_i$ are integral, then the solution $\alpha_i = \frac{c_i}{b_i} \left(\Pi_j b_j\right) \; \forall i$ is integral and the mutual information is preserved. We will thus consider (\ref{eq:main}) with the constraint that $\alpha_i \in \mathbb{N}$ for $i \in [K] \cup \{0\}.$
    
    \begin{lemma}
        \label{lem:integer_sol_optimal}
        If an optimal solution to (\ref{eq:main}) exists, then there exists an optimal solution to Equation \ref{eq:main} with $\alpha_i \in \mathbb{N}$ for $i \in [K] \cup \{0\}.$
    \end{lemma}
    
    Let $ Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i.$ We obtain the lower bound on $I(X \; ; \; \alpha_0 X + Z_{\alpha})= H(p) - H(X \; | \; \alpha_0 X+Z_{\alpha})$ in Theorem \ref{thm:main_lower_bound} by finding a lower bound on $-H(X \; | \; \alpha_0 X+Z_{\alpha}).$  The optimization problem we consider is therefore
    \begin{align}
       \label{eq:integral_alpha_opt_prob}
        & \min_{\alpha_0,...,\alpha_K \in \mathbb{N}} -H\left(X \; | \; \alpha_{0} X+\sum_{k=1}^K \alpha_k Z_k\right).
    \end{align}
    Observe that the PMF for any random variable $Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i$ has probability $(1-p)^{K+1}$ at the highest support value.  Thus, the following problem is clearly a relaxation to (\ref{eq:integral_alpha_opt_prob})
    \begin{align}
       \label{eq:relax_inf1}
        & \min_{D} -H\left(X \; | \; \alpha_0 X+D\right)
        \\ & \text{subject to:} 
        \nonumber \\ & D \text{ is a random variable with integral support,}
        \nonumber \\ & D  \text{ has maximum support value at 0,} 
        \nonumber \\ & \Pr(D = 0) = (1-p)^K.
        \nonumber
    \end{align}
    Due to Lemma \ref{lem:alpha0_condition}, we can fix $\alpha_0 = 1$ in (\ref{eq:relax_inf1}) above without changing the optimal value.  
    Written more explicitly  with $\alpha_0 = 1$ fixed, (\ref{eq:relax_inf1}) is given by
    \begin{align}
    \label{eq:relax_inf2}
	& \min_{q_{(-i)} \geq 0 : \; i \in \mathbb{N}\cup\{0\} } \sum_{j \in \{-n : \; n \in \mathbb{N}\}} 
	\nonumber \\ & (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & + p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right)    \\ &  \text{subject to:} \quad \nonumber \\ & \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad    \sum_{j \in \{-n : \; n \in \mathbb{N}\cup\{0\}\}} q_{(j)} = 1 \nonumber
	\end{align}  
    where $q_{(0)}$ is the probability at the maximum support value of $D$ and $q_{(-i)}$ is the probability at the $i$th integer below the maximum support value of $D.$  Note that the conditional entropy in the objective function is in a simplified form.   
    
    Observe that (\ref{eq:relax_inf2}) is an infinite dimensional convex minimization problem.  A solution to the KKT conditions with the added implicit constraint that $q_{(-i)}>0$ for $i \in \mathbb{N} \cup \{0\}$  is given by  $q_{(-i)} = (1-p)^K (1 - (1-p)^K)^i$ for $i \in \mathbb{N} \cup \{0\}$ which corresponds to $D = -G$ in (\ref{eq:relax_inf1}) where $G$ is a geometric random variable with success probability equal to $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\}.$  We do not use this observation directly to establish Theorem \ref{theorem:main_recursion} because no reference on the relation between KKT conditions and optimality in the infinite dimensional case was found.  
    
    Instead, we form a new optimization problem where we constrain $D$ to have distance $n$ between its maximum and minimum support values, derive a lower bound on the solution for $n \in \mathbb{N}$, and use this sequence of lower bounds to establish the result. The support constrained version of (\ref{eq:relax_inf2}) is given by 
    \begin{align}
    \label{eq:relax_const}
    & \min_{q_{(-i)} \geq 0 : \; i \in [n+1]\cup\{0\} }
    \sum_{j \in \{-m : \; m \in [n+1]\}} 
	\nonumber \\ & (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & + p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right)    \\ &  \text{subject to:} \nonumber \\ & 
    \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad q_{(-n-1)} = 0, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1. \nonumber
	\end{align}  

    Changing the implicit constraint in (\ref{eq:relax_const}) from $q_{(i)} \geq 0$ to $q_{(i)} > 0$ and the explicit constraint $q_{(-n-1)} = 0$ to $q_{(-n-1)} = \epsilon$ where $\epsilon \in \mathbb{R}_{>0}$ gives us
    \begin{align}
    \label{eq:relax_const_posq}
    & \min_{q_{(-i)} > 0 : \; i \in [n+1]\cup\{0\} }
    \sum_{j \in \{-m : \; m \in [n+1]\}} 
	\nonumber \\ & (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & + p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right)   \\ &  \text{subject to:} \nonumber \\ & 
    \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad q_{(-n-1)} = \epsilon,
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1. \nonumber
	\end{align}  

    Let $p^*$ be the optimal value of \ref{eq:relax_const} and let $p_{\epsilon}^*$ be the optimal value of \ref{eq:relax_const_posq} for a given $\epsilon.$ Due to the continuity of the objective function in (\ref{eq:relax_const}), it is not hard to show that $ p^* \geq \inf_{\epsilon \in \mathbb{R}_{>0}} p_{\epsilon}^*.$  At a high level, this is due to the fact that for any solution to  (\ref{eq:relax_const}), it follows that (\ref{eq:relax_const_posq}) can get arbitrarily close to it as $\epsilon \to 0$ due to the continuity of the objective function.  



    While we do not know the solution to (\ref{eq:relax_const}) or (\ref{eq:relax_const_posq}), we will perturb (\ref{eq:relax_const_posq}) to form a problem we can solve analytically, then use perturbation analysis to lower bound the optimal value of (\ref{eq:relax_const_posq}), and ultimately lower bound the optimal value of (\ref{eq:relax_const}).  The perturbed version of (\ref{eq:relax_const_posq}) is given by 
	\begin{align}
	\label{eq:relax_const_pert_posq}
    & \min_{q_{(-i)} > 0 : \; i \in [n+1]\cup\{0\} }
    \sum_{j \in \{-m : \; m \in [n+1]\}} 
	\nonumber \\ &  (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & +  p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) \\	& 
	\text{subject to:} \nonumber \\
	& \quad q_{(0)} = (1-p)^K,
	\nonumber \\ & \quad q_{(-n-1)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2} \nonumber
	\end{align}  
    where we have changed the constraint on the probability at the minimum support value, and the constraint on the sum of all the probabilities.
    We can solve this by solving the KKT conditions since the problem is convex, Slater's condition holds, and the objective function and constraint functions are differentiable on the domain $q_{(i)} > 0.$  
    
    We proceed to find the solution to the KKT conditions for (\ref{eq:relax_const_pert_posq}).  Let $f_0(q)$ be the objective function of (\ref{eq:relax_const_pert_posq}).  The Lagrangian is given by 
	\begin{align} 
	&L(q, v, \lambda) = f_0(q) 
	\nonumber \\ & + v_1 \left(\sum_i q_{(i)} - 1 + (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & + v_2 \left(q_{(0)} - (1-p)^K \right) 
	\nonumber \\ & + v_3 \left(q_{(-n-1)} - (1-p)^K (1 - (1-p)^K)^{n+1} \right). 
	\end{align}
	The derivative of $f_0(q)$ with respect to $q_{(j)}$ is given by 
	\begin{align}
	& p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) \nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right)
	\end{align}  
	for $j \in \{-n, \; ..., \;  -1\}$ and the KKT conditions are given by 
	\begin{align}
	& q_{(0)} = (1-p)^K,
	\nonumber \\ & q_{(-n-1)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ &     \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2}
	\nonumber \\ & (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right) + v_1 + v_3 = 0 \quad 
	\nonumber \\ &  \text{for } j = - n -1
	\nonumber \\ & 	p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) 
	\nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right)+ v_1 = 0 
	\nonumber \\ &  \forall j \in \{-n, \; ..., \;  -1\}
	\nonumber \\ & p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) + v_1 + v_2 = 0 
	\nonumber \\ & \text{for } j = 0.
	\end{align}
	

	
	The last three conditions can be rewritten as 
	\begin{align} 
	& (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+1)}}{q_{(j)}} + (1-p) } \right) + v_1 + v_3 = 0  
	\nonumber \\ &  \text{for } j = - n - 1
	\nonumber \\ & p \log \left(\frac{p }{(1-p)\frac{q_{(j-1)}}{q_{(j)}} + p } \right) \nonumber \\ & + (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+1)}}{q_{(j)}} + (1-p) } \right)   + v_1  = 0 
	\nonumber \\ & \forall j \in \{-n, \; ..., \;  -1\}
	\nonumber \\ & p \log \left(\frac{p }{(1-p) \frac{q_{(j-1)}}{q_{(j)}} + p } \right)  + v_1 + v_2  = 0 \quad \text{for } j = 0
	\end{align}
	which shows that if the ratio $\frac{q_{(j-1)}}{q_{(j)}}$ between consecutive variables is the same for all $j,$  then $v_1,$ $v_2$ can  be chosen so that of these derivatives equal $0$ for all $j.$  Picking \[\frac{q_{(j-1)}}{q_{(j)}} = (1 - (1-p)^K),\] a solution to these equations is then
	\begin{align}
	& q_{(-i)} =  (1-p)^K (1 - (1-p)^K)^{i}  
	\nonumber \\ & \text{for } i \in \{0, \; 1, \; ..., \; n+1 \} 
	\nonumber \\ & v_1 = - p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & - (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right)
	\nonumber \\ & v_2 = (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & v_3 = p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right)
	\end{align}
	
    This is the solution to (\ref{eq:relax_const_pert_posq}) as discussed earlier.  The optimal value for (\ref{eq:relax_const_pert_posq}) is therefore given by 
	\begin{align} 
	& \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
	\nonumber \\ & - p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	\nonumber \\ & = \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \alpha^i \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\end{align}
	where $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K.$  
	Applying the geometric sum formula and simplifying,  the optimal value for (\ref{eq:relax_const_pert_posq}) is   
	\begin{align} 
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right).
	\end{align}
	
	Using the perturbation analysis from Section 5.6.1 of \cite{boyd}, we see that the optimal value of (\ref{eq:relax_const_posq}) is lower bounded by
	\begin{align}
	\label{eq:relax_const_posq_bound}
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\nonumber \\ & - v_1^* \left( (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & - v_3^* \left(- (1-p)^K (1 - (1-p)^K)^{n+1} +\epsilon \right) 
	\end{align} 
	where $v_1^*$ and $v_3^*$ are the optimal lagrange multipliers for (\ref{eq:relax_const_pert_posq})
	we determined through the KKT conditions.
	
	Taking the infimum of \ref{eq:relax_const_posq_bound} then over $\epsilon \in \mathbb{R}_{>0}$ yields the following lower bound on (\ref{eq:relax_const_posq}):
	
	\begin{align}
	\label{eq:relax_const_bound}
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\nonumber \\ & - v_1^* \left( (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & - v_3^* \left(- (1-p)^K (1 - (1-p)^K)^{n+1} \right). 
	\end{align} 
	
	The sequence of optimal values returned by (\ref{eq:relax_const}) is monotonically decreasing in $n$ clearly.  Thus, taking the limit of the lower bound (\ref{eq:relax_const_bound}) as  $n \to \infty$ and simplifying yields the following lower bound on $-H(X \; | \; \alpha_0 X + Z_{\alpha})$ for any choice of $\alpha_i$'s: 	\begin{align} 
	& -(p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right).
	\end{align}
	
	Thus, a lower bound on mutual information is
	\begin{align} 
	& H(p) - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
	\end{align}
	for any choice of $\alpha_i$'s.
	
	Finally, observe that
	\begin{align}
	& H(X \; ; \; X - G) 
	\nonumber \\ & =\sum_{i = 0}^{\infty} (1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
	\nonumber \\ & + p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	\nonumber \\ & = (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right)  
	\nonumber \\ & + p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
	\end{align}
	where $G$ is a geometric random variable with success probability $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\},$  and $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K$ as before.
	
	%Due to Lemma \ref{lem:alpha0_condition}, given $\alpha_0,$ any solution can be transformed into a solution whose PMF had support values in $\{t \alpha_0 : \; t \in \mathbb{Z}\}$ without increasing the mutual information.   Therefore, for a fixed $\alpha_0,$ it suffices to only consider PMFs that have support values in $\{t \alpha_0 : \; t \in \mathbb{Z}\}$ in the optimization.  If $\alpha_0 = a \in \mathbb{N}$ any solution random variable $D$ with  support values in $\{t a : \; t \in \mathbb{Z}\}$ can be transformed into a solution with the same mutual information, $\alpha_0 = 1,$ and support values in $\{t : \; t \in \mathbb{Z}\}.$ This is accomplished by dividing $D$ by $a.$     Therefore, we analyze the relaxation with $\alpha_0 = 1.$
	
\end{IEEEproof}

\begin{lemma}
    \label{lem:alpha0_condition}
    Fixing $\alpha_0 = 1$ in (\ref{eq:relax_const}) can not increase the optimal value.
\end{lemma}

\begin{IEEEproof}
    Let $\alpha_0 \in \mathbb{N}.$ 
	Let $Z$ be any random variable such that its PMF has integral support and maximum support value at $t = 0.$  Let 
	\begin{align}
	& \hat{Z} = Z - S
	\end{align} 
	where $S = Z \mod{\alpha_0}.$ 
	We then have that 
	\begin{align}
	& I(X ; \alpha_0 X + 	Z)  \geq I(X ; \alpha_0 X + \hat{Z}).   
	\end{align}
	because  
	\begin{align} 
		& I(X ; \; \alpha_0 X + 	Z)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z} +  S)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z}, \; S)
		\nonumber \\ & = I(X ; \; S) + I(X ; \; \alpha_0 X + \hat{Z} \; | \; S)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z} \; | \; S)
		\nonumber \\ & = H(X \; | \; S)  - H(X \; | \; \alpha_0 X + \hat{Z}, \; S) 
		\nonumber \\ & = H(X)  - H(X \; | \; \alpha_0 X + \hat{Z}, \; S)
		\nonumber \\ & \geq H(X)  - H(X \; | \; \alpha_0 X + \hat{Z})
		\nonumber \\ & = I(X \; ; \; \alpha_0 X + \hat{Z})
	\end{align} 
	where the third line follows because given $\alpha_0 X + \hat{Z} + S,$ we have that 
	\begin{align}
	    S = ((\alpha_0 X + \hat{Z} + S) - \alpha_0) \mod  \alpha_0 
	\end{align}
	and
    \begin{align}
	    \alpha_0 X + \hat{Z} = (\alpha_0 X + \hat{Z} + S) - S.
	\end{align}
	Thus, any solution to (\ref{eq:relax_inf1}) with  $\alpha_0 = a$ can be transformed into a solution whose PMF had support values in $\{t a : \; t \in \mathbb{Z}\}$ without increasing the mutual information.   Therefore, for a fixed $\alpha_0,$ it suffices to only consider PMFs that have support values in $\{t \alpha_0 : \; t \in \mathbb{Z}\}$ in the optimization.  If $\alpha_0 = a \in \mathbb{N}$ any solution random variable $D$ with  support values in $\{t a : \; t \in \mathbb{Z}\}$ can be transformed into a solution with the same mutual information, $\alpha_0 = 1,$ and support values in $\{t : \; t \in \mathbb{Z}\}.$ This is accomplished by dividing $D$ by $a.$  Therefore it suffices to fix $\alpha_0=1$ in the optimization. 
	\end{IEEEproof}


==> main_result10_17_20.tex <==
\section{Main Results}


%\begin{figure}
%\centering
%\includegraphics[width=0.9\linewidth]{performance_plot_K6_minor_allele}
%\caption{}
%\label{fig:performance_plot_K6_minor_allele}
%\end{figure}

In order to tackle the discrete optimization problem in (\ref{eq:main2}), we seek to bound its optimal solution.
Our main result is the following lower bound.


% Our main result is a lower bound to (\ref{eq:main2})

\begin{theorem} \label{thm:main_lower_bound}
	For any $K\in \mathbb{N}$ and $p \in [0, 0.5],$  we have 
	\begin{align} 
	%& \min_{\alpha_i \in \mathbb{N}, \; i \in [K]\cup\{0\}}
	& \min_{\alpha}
	I(X \; ; \; X +Z_\alpha) 
	\geq 
	I(X \; ; \; X - G),
	\end{align}
	where $G$ is a geometric random variable with success probability equal to $(1-p)^K$.
	and support equal to $\mathbb{N} \cup \{0\}.$
	\iscomment{instead, let's describe the pmf of $G$ to be concrete}
\end{theorem}

Intuitively, Theorem~\ref{thm:main_lower_bound} says that the noise distribution of $-G$ is worse than the worst-case noise $Z_\alpha$ for all possible $\alpha$s.
This lower bound can in fact be explicitly computed as
% The formula for $I(X \; ; \; X - G)$ is given by 
\begin{align}
& I(X \; ; \; X - G)
% \nonumber \\ & 
= H(p) 
\nonumber \\ & - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
\end{align}
\iscomment{simpler:}
\begin{align}
& I(X \; ; \; X - G)
% \nonumber \\ & 
= H(p) 
\nonumber \\ & - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{1-(1-p)^{K+1} }{(p-1) \left( (1-p)^K -1 \right)}\right) 
\nonumber \\ & - p \log \left( \frac{1-(1-p)^{K+1}}{p} \right)
\end{align}
% \iscomment{
% Can we extract a KL divergence between $p$ and $(1-p)^$
% }
Observe that the formula is quickly computable for any value of $K$ and $p,$ making it attractive from a computational standpoint.  To assess how tight the lower bound is, we empirically compare it to an upper bound that is computed with a greedy algorithm in Figure \ref{fig:greedy_versus_bound_K15}.  For a given $p$ and $K,$ the greedy algorithm chooses $\alpha_0 = 1, \; \alpha_1 = 1,$ and sequentially chooses \begin{align} \alpha_{j} = \argmin_{\alpha \in \mathbb{N} \; : \; 1 \leq \alpha \leq 1 + \sum_{i = 1}^{j-1}  \alpha_i} I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)
\end{align}
for $2 \leq j \leq K.$  As seen in Figure \ref{fig:greedy_versus_bound_K15}, $I(X \; ; \; X - G)$ serves as a very tight lower bound when compared with the upper bound.  We therefore view $I(X \; ; \; X - G)$ as an approximation to the original problem.  This is surprising, because for a given $K,$ it is not possible in general to choose $\alpha_i$'s to make the PMF of $\sum_{i = 1}^{j-1} \alpha_i Z_i$ look like a shifted version of the PMF for  $-G.$

While the greedy algorithm requires $\Omega(2^K)$ time in the worst case, similar plots to Figure \ref{fig:greedy_versus_bound_K15} can be obtained for larger values of $K$ using a more computationally efficient variation of the greedy algorithm that is discussed in the longer version of this paper.

In order to prove the lower bound on the minimization of $I(X \; ; \; X + \sum_{i=1}^K \alpha_i Z_i)$ in Theorem \ref{thm:main_lower_bound}, we form a convex relaxation of the minimization problem, perturb the relaxation to form a problem that is analytically solvable using KKT conditions, and use perturbation analysis to find a lower bound on the relaxation.  This is then a lower bound on the original problem.  The full proof is in the Section V.

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .06]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{upper bound (greedy)}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\label{fig:greedy_versus_bound_K15}
\end{figure}

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Ratio: Upper Bound to Lower Bound},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
legend pos = north west]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt4_greedy_opt_ratio_K15.dat};
\addlegendentry{K = 15}

\addplot [
line width=1pt,
color=blue!80!black
] table[x index=0,y index=1] {data/plt4_greedy_opt_ratio_K10.dat};
\addlegendentry{K = 10}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt4_greedy_opt_ratio_K5.dat};
\addlegendentry{K = 5}

\end{axis}    
\end{tikzpicture}
\caption{}
\label{fig:greedy_versus_bound_ratio}
\end{figure}

%\begin{tikzpicture}
%\begin{axis} 
%[title ={Comparison of Bounds: $K = 15$},
%ylabel = mutual information, 
%xlabel = minor allele frequency (p),
%ymax = .001,
%legend pos=north west]

%\addplot [
%line width=1pt,
%color=red!80!black
%] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{upper bound}

%\addplot [
%line width=1pt,
%color=blue!80!black
%] table[x index=0,y index=1] %{data/plt2_bound.dat};
%\addlegendentry{lower bound}

%\end{axis}    
%\end{tikzpicture}
%\caption{}
%\label{fig:greedy_versus_bound_K15}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p1}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p1}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p001}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p001}
%\end{figure}


%The lower bound is formally proved in the appendix, but we outline the argument here, as it sheds light on the problem, and makes interesting use of convex optimization theory

\section{Efficiently Computable Schemes}

\rdcomment{this may sound stupid, but i think it warrants a sentence here. `Theorem 1 gives us a lower bound on the mutual information between $X$ and ..., which would be the mixing ratio that provides the highest level of privacy. However, it does not provide any mixing scheme for approaching this lower bound.'}

While much faster than brute force search, the greedy algorithm used to obtain the upper bound requires $\Omega(2^K)$ time in the worst case.  At a high level, this is due to the fact that at the $j$th  step in the algorithm, computation of $I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)$ requires use of each support value in the PMF of $\alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i,$ and there are $\Omega(2^j)$ support values in the worst case.  This motivates the design of efficiently computable schemes, which can then be evaluated using the lower bound in Theorem \ref{thm:main_lower_bound}.

Perhaps the most natural approach is given by the uniform scheme, which we define to set $\alpha_i = 1$ for all $i \in [K]\cup\{0\}.$  This is the scheme used by the authors of \cite{Maddah-Ali} to obtain their results.  The scheme is explicitly defined given $K,$ so no algorithm is needed to compute it.  The performance of the scheme for a given $p$ and $K$ can be computed in $O(K)$ time using the formula in Lemma \ref{lem:uniform_schem_formula} which is given in the appendix.

The uniform scheme is important because it is optimal as $p \to 0$ as proved in Lemma \ref{lem:optimality_of_uniform}
and exemplified by the optimal curve in Figure \ref{fig:optimal_scheme_K5_minor_allele}.

\begin{lemma}
\label{lem:optimality_of_uniform}
For any $K \in \mathbb{N},$ there exists some $p^* > 0$ such that the uniform scheme is optimal for $p < p^*.$
\end{lemma}

\rdcomment{i changed epsilon to $p^*$ here. epsilon is typically taken to mean a very small constant, which makes this result feel weak, i.e. this result is only true when p is arbitrarily small.}

At $p= 0.5,$ in Figure \ref{fig:optimal_scheme_K5_minor_allele}, the optimal solution is given by the binary scheme, which we define to set $\alpha_0 = 1$ and $\alpha_i = 2^{i-1}$ for all $i \in [K].$  Similar to the uniform scheme, the binary scheme is explicitly defined given $K.$  Also, similar to the uniform scheme, there exists a formula for computing its performance given $p$ and $K$ in $O(K)$ time.  This formula is given in Lemma \ref{lem:binary_scheme_performance} in the appendix.  It is interesting that such a formula exists because the PMF of $\sum_{i=1}^K 2^{i-1} Z_i$ has $2^K$ support values. 

Most importantly, the optimality of the binary scheme at $p = 0.5$ for $K=5$ shown in Figure \ref{fig:optimal_scheme_K5_minor_allele} generalizes to all $K$ as proved in Lemma \ref{lem:optimality_of_binary}.

\begin{lemma} \label{lem:optimality_of_binary}
	For any $K \in \mathbb{N},$ the binary scheme is optimal for $p = 0.5.$
\end{lemma}

Because the uniform scheme is optimal for $p \to 0$ and the binary scheme is optimal for $p = 0.5,$  it is natural to try and combine these schemes to interpolate the performance for $p$ in the range $0<p<0.5.$  Combining only the uniform scheme and the binary scheme does not produce a scheme that approaches the lower bound.  However, the general shape of the lower bound can be captured in polynomial time by combining the uniform scheme, the linear scheme, and the binary scheme where the linear scheme is defined as $\alpha_0 = 1$ and $\alpha_i = i$ for $i \in [K].$  We define the $(K,L,U)$-binary-linear-uniform scheme to set $\alpha_0 = 1$ and 
\begin{align} &\alpha_i = 1 \quad i \in \{1, ..., U\} \nonumber \\  &\alpha_{U+i} = i \quad i \in \{1, ..., L\} \nonumber \\
&\alpha_{U+L+i} = 2^{i-1} \quad i \in \{1, ..., K-U-L\}
\end{align}

\rdcomment{should it be binary-linear-uniform above?}

For a given $K$ and $p,$ we define the $K$-binary-linear-uniform scheme as the $(K,L^*,U^*)$-binary-linear-uniform scheme where
\begin{align} & (L^*, U^*) = \argmin_{(L,U) \in ([K]\cup\{0\})^2 \; : \; L + U \leq K} \\ &  I\left(X \; ; \; X + \sum_{i=1}^{U} Z_i + \sum_{j=1}^{L} j Z_{U+j} +  \sum_{k=1}^{K-U-L} 2^{k -1} Z_{U+L+k}\right) \nonumber.
\end{align}
The $K$-binary-linear-uniform scheme is computed in $O(K^4)$ time using a generalization of the recursion used to prove Lemma \ref{lem:binary_scheme_performance}.  

We compare the performance of the uniform scheme, the binary scheme, the $K$-binary-linear-uniform scheme, and the scheme generated by the greedy algorithm in Figure \ref{fig:efficiently_computable_schemes}.  We have observed that the scheme generated by the greedy algorithm is much tighter than the   $K$-binary-linear-uniform scheme after the initial hump in the lower bound as $K$ increases.



\begin{figure}[h]
\label{fig:efficiently_computable_schemes}
\centering
\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .6,
legend pos = north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}


\end{axis}    
\end{tikzpicture}

\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .01]
%,
%legend pos=north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
%\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
%\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
%\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
%\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
%\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\end{figure}



%Greedy takes exponential time in $K$ to compute.

%Simpler schemes: uniform, binary, interpolation between uniform and binary.


%Maybe state theorems about uniform and binary. Or maybe just mention them and refer to the longer version


\section{Proof of Main Result}

We now present the proof of Theorem \ref{thm:main_lower_bound}.  

\begin{IEEEproof}
    First, notice that choosing integral $\alpha_i \; : \;  i \in [K] \cup \{0\}$ in the optimization problem (\ref{eq:main}) is optimal due to Lemma \ref{lem:integer_sol_optimal}.  Lemma \ref{lem:integer_sol_optimal} holds because if $\alpha_i = \frac{c_i}{b_i} \; \forall i$ in (\ref{eq:main}) where $c_i, b_i$ are integral, then the solution $\alpha_i = \frac{c_i}{b_i} \left(\Pi_j b_j\right) \; \forall i$ is integral and the mutual information is preserved. We will thus consider (\ref{eq:main}) with the constraint that $\alpha_i \in \mathbb{N}$ for $i \in [K] \cup \{0\}.$
    
    \begin{lemma}
        \label{lem:integer_sol_optimal}
        If an optimal solution to (\ref{eq:main}) exists, then there exists an optimal solution to (\ref{eq:main}) with $\alpha_i \in \mathbb{N}$ for $i \in [K] \cup \{0\}.$
    \end{lemma}
    
    Let $ Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i.$ We obtain the lower bound on $I(X \; ; \; \alpha_0 X + Z_{\alpha})= H(p) - H(X \; | \; \alpha_0 X+Z_{\alpha})$ in Theorem \ref{thm:main_lower_bound} by finding a lower bound on $-H(X \; | \; \alpha_0 X+Z_{\alpha}).$  The optimization problem we consider is therefore
    \begin{align}
       \label{eq:integral_alpha_opt_prob}
        & \min_{\alpha_0,...,\alpha_K \in \mathbb{N}} -H\left(X \; | \; \alpha_{0} X+\sum_{k=1}^K \alpha_k Z_k\right).
    \end{align}
    Observe that the PMF for any random variable $Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i$ has probability $(1-p)^{K}$ at the highest support value.  Thus, the following problem is clearly a relaxation to (\ref{eq:integral_alpha_opt_prob}):
    \begin{align}
       \label{eq:relax_inf1}
        & \min_{D} -H\left(X \; | \; \alpha_0 X+D\right)
        \\ & \text{subject to:} 
        \nonumber \\ & D \text{ is a random variable with integral support,}
        \nonumber \\ & D  \text{ has maximum support value at 0,} 
        \nonumber \\ & \Pr(D = 0) = (1-p)^K.
        \nonumber
    \end{align}
    Due to Lemma \ref{lem:alpha0_condition}, we can fix $\alpha_0 = 1$ in (\ref{eq:relax_inf1}) above without changing the optimal value.  Written more explicitly  with $\alpha_0 = 1$ fixed, (\ref{eq:relax_inf1}) is given by
    \begin{align}
    \label{eq:relax_inf2}
	& \min_{q_{(-i)} \geq 0 : \; i \in \mathbb{N}\cup\{0\} } \sum_{j \in \{-n : \; n \in \mathbb{N}\}} 
	\nonumber \\ & (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & + p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right)    \\ &  \text{subject to:} \quad \nonumber \\ & \quad q_{(0)} = (1-p)^K, \quad    \sum_{j} q_{(j)} = 1 \nonumber
	\end{align}  
    where $q_{(0)}$ is the probability at the maximum support value of $D$ and $q_{(-i)}$ is the probability at the $i$th integer below the maximum support value of $D.$  Note that the conditional entropy in the objective function is in a simplified form.   
    
    Observe that (\ref{eq:relax_inf2}) is an infinite dimensional convex minimization problem.  A solution to the KKT conditions with the added implicit constraint that $q_{(-i)}>0$ for $i \in \mathbb{N} \cup \{0\}$  is given by  $q_{(-i)} = (1-p)^K (1 - (1-p)^K)^i$ for $i \in \mathbb{N} \cup \{0\}$ which corresponds to $D = -G$ in (\ref{eq:relax_inf1}) where $G$ is a geometric random variable with success probability equal to $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\}.$  We do not use this observation directly to establish Theorem \ref{theorem:main_recursion} because no reference on the relation between KKT conditions and optimality in the infinite dimensional case was found.  
    
    Instead, we constrain $D$ to have distance no greater than $n \in \mathbb{N}$ between its maximum and minimum support values in (\ref{eq:relax_inf2}), derive a lower bound on the solution for each $n \in \mathbb{N},$ and use the resulting sequence of lower bounds to establish the result. The support constrained version of (\ref{eq:relax_inf2}) is given by 
    \begin{align}
    \label{eq:relax_const}
    & \min_{q_{(-i)} \geq 0 : \; i \in [n+1]\cup\{0\} }
    \sum_{j \in \{-m : \; m \in [n+1]\}} 
	\nonumber \\ & (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & + p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right)    \\ &  \text{subject to:} \nonumber \\ & 
    \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad q_{(-n-1)} = 0, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1. \nonumber
	\end{align}  

    Changing the implicit constraint in (\ref{eq:relax_const}) from $q_{(i)} \geq 0$ to $q_{(i)} > 0$ and the explicit constraint $q_{(-n-1)} = 0$ to $q_{(-n-1)} = \epsilon$ where $\epsilon \in \mathbb{R}_{>0}$ gives us
    \begin{align}
    \label{eq:relax_const_posq}
    & \min_{q_{(-i)} > 0 : \; i \in [n+1]\cup\{0\} }
    \sum_{j \in \{-m : \; m \in [n+1]\}} 
	\nonumber \\ & (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & + p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right)   \\ &  \text{subject to:} \nonumber \\ & 
    \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad q_{(-n-1)} = \epsilon,
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1. \nonumber
	\end{align}  

    Let $p^*$ be the optimal value of \ref{eq:relax_const} and let $p_{\epsilon}^*$ be the optimal value of \ref{eq:relax_const_posq} for a given $\epsilon.$ Due to the continuity of the objective function in (\ref{eq:relax_const}), it is not hard to show that $ p^* \geq \inf_{\epsilon \in \mathbb{R}_{>0}} p_{\epsilon}^*.$  At a high level, this is due to the fact that for any solution to  (\ref{eq:relax_const}), it follows that (\ref{eq:relax_const_posq}) can get arbitrarily close to it as $\epsilon \to 0$ due to the continuity of the objective function.  



    While we do not know the solution to (\ref{eq:relax_const}) or (\ref{eq:relax_const_posq}), we will perturb (\ref{eq:relax_const_posq}) to form a problem we can solve analytically, then use perturbation analysis to lower bound the optimal value of (\ref{eq:relax_const_posq}), and ultimately lower bound the optimal value of (\ref{eq:relax_const}).  The perturbed version of (\ref{eq:relax_const_posq}) is given by 
	\begin{align}
	\label{eq:relax_const_pert_posq}
    & \min_{q_{(-i)} > 0 : \; i \in [n+1]\cup\{0\} }
    \sum_{j \in \{-m : \; m \in [n+1]\}} 
	\nonumber \\ &  (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	\nonumber \\ & +  p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) \\	& 
	\text{subject to:} \nonumber \\
	& \quad q_{(0)} = (1-p)^K,
	\nonumber \\ & \quad q_{(-n-1)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2} \nonumber
	\end{align}  
    where we have changed the constraint on the probability at the minimum support value, and the constraint on the sum of all the probabilities.
    We can solve this by solving the KKT conditions since the problem is convex, Slater's condition holds, and the objective function and constraint functions are differentiable on the domain $q_{(i)} > 0.$  
    
    We proceed to find the solution to the KKT conditions for (\ref{eq:relax_const_pert_posq}).  Let $f_0(q)$ be the objective function of (\ref{eq:relax_const_pert_posq}).  The Lagrangian is given by 
	\begin{align} 
	&L(q, v, \lambda) = f_0(q) 
	\nonumber \\ & + v_1 \left(\sum_i q_{(i)} - 1 + (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & + v_2 \left(q_{(0)} - (1-p)^K \right) 
	\nonumber \\ & + v_3 \left(q_{(-n-1)} - (1-p)^K (1 - (1-p)^K)^{n+1} \right). 
	\end{align}
	By Lemma \ref{lem:solve_KKT}, a solution to the KKT conditions is given by 
	\begin{align}
	\label{eq:KKT_conditions_sol}
	& q_{(-i)} =  (1-p)^K (1 - (1-p)^K)^{i}  \text{ for } i \in [n+1] \cup \{0\} 
	\nonumber \\ & v_1 = - p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & - (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right)
	\nonumber \\ & v_2 = (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & v_3 = p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right),
	\end{align}
    which is then an optimal solution to (\ref{eq:relax_const_pert_posq}).  %The optimal value for (\ref{eq:relax_const_pert_posq}) is therefore given by 
	%\begin{align} 
	%& \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
	%\nonumber \\ & - p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	%\nonumber \\ & = \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	%\nonumber \\ & - p \beta \alpha^i \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	%\end{align}
	Applying the geometric sum formula and simplifying,  the optimal value for (\ref{eq:relax_const_pert_posq}) is   
	\begin{align} 
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\end{align}
	where $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K.$  
	
	Using the perturbation analysis from Section 5.6.1 of \cite{boyd}, we see that the optimal value of (\ref{eq:relax_const_posq}) is lower bounded by
	\begin{align}
	\label{eq:relax_const_posq_bound}
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\nonumber \\ & - v_1^* \left( (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & - v_3^* \left(- (1-p)^K (1 - (1-p)^K)^{n+1} +\epsilon \right) 
	\end{align} 
	where $v_1^*$ and $v_3^*$ are the optimal lagrange multipliers for (\ref{eq:relax_const_pert_posq})
	we determined through the KKT conditions.
	
	Taking the infimum of (\ref{eq:relax_const_posq_bound}) over $\epsilon \in \mathbb{R}_{>0}$ yields the following lower bound on (\ref{eq:relax_const}):
	
	\begin{align}
	\label{eq:relax_const_bound}
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\nonumber \\ & - v_1^* \left( (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & - v_3^* \left(- (1-p)^K (1 - (1-p)^K)^{n+1} \right). 
	\end{align} 
	
	The sequence of optimal values returned by (\ref{eq:relax_const}) is monotonically decreasing in $n$ clearly.  Thus, taking the limit of the lower bound (\ref{eq:relax_const_bound}) as  $n \to \infty$ and simplifying yields the following lower bound on $-H(X \; | \; \alpha_0 X + Z_{\alpha})$ for any choice of $\alpha_i$'s: 	\begin{align} 
	& -(p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right).
	\end{align}
	
	%Thus, a lower bound on mutual information is
	%\begin{align} 
	%& H(p) - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right)
	%\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
	%\end{align}
	%for any choice of $\alpha_i$'s.
	
	Finally, observe that
	\begin{align}
	& -H(X \; ; \; X - G) 
%	\nonumber \\ & =\sum_{i = 0}^{\infty} (1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
%	\nonumber \\ & + p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	\nonumber \\ & = -(p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right)
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
	\end{align}
	where $G$ is a geometric random variable with success probability $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\},$  and $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K$ as before.
\end{IEEEproof}	

\begin{lemma}
    \label{lem:alpha0_condition}
    Fixing $\alpha_0 = 1$ in (\ref{eq:relax_const}) can not increase the optimal value.
\end{lemma}

\begin{IEEEproof}
    Let $\alpha_0 \in \mathbb{N}.$ 
	Let $Z$ be any random variable such that its PMF has integral support and maximum support value at $t = 0.$  Let 
	\begin{align}
	& \hat{Z} = Z - S
	\end{align} 
	where $S = Z \mod{\alpha_0}.$ 
	We then have that 
	\begin{align}
	& I(X ; \alpha_0 X + 	Z)  \geq I(X ; \alpha_0 X + \hat{Z}).   
	\end{align} 
	because
	\begin{align} 
		& I(X ; \; \alpha_0 X + 	Z)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z} +  S)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z}, \; S)
		\nonumber \\ & = I(X ; \; S) + I(X ; \; \alpha_0 X + \hat{Z} \; | \; S)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z} \; | \; S)
		\nonumber \\ & = H(X \; | \; S)  - H(X \; | \; \alpha_0 X + \hat{Z}, \; S) 
		\nonumber \\ & = H(X)  - H(X \; | \; \alpha_0 X + \hat{Z}, \; S)
		\nonumber \\ & \geq H(X)  - H(X \; | \; \alpha_0 X + \hat{Z})
		\nonumber \\ & = I(X \; ; \; \alpha_0 X + \hat{Z})
	\end{align} 
	where the third line follows because given $\alpha_0 X + \hat{Z} + S,$ we have that 
	\begin{align}
	    S = ((\alpha_0 X + \hat{Z} + S) - \alpha_0) \mod  \alpha_0 
	\end{align}
	and
    \begin{align}
	    \alpha_0 X + \hat{Z} = (\alpha_0 X + \hat{Z} + S) - S.
	\end{align}
	Thus, any solution to (\ref{eq:relax_inf1}) with  $\alpha_0 = a$ can be transformed into a solution whose PMF had support values in $\{t a : \; t \in \mathbb{Z}\}$ without increasing the mutual information.   Therefore, for a fixed $\alpha_0,$ it suffices to only consider PMFs that have support values in $\{t \alpha_0 : \; t \in \mathbb{Z}\}$ in the optimization.  If $\alpha_0 = a ,$ any solution random variable $D$ with  support values in $\{t a : \; t \in \mathbb{Z}\}$ can be transformed into a solution with the same mutual information, $\alpha_0 = 1,$ and support values in $\{t : \; t \in \mathbb{Z}\}.$ This is accomplished by dividing $D$ by $a.$  Therefore it suffices to fix $\alpha_0=1$ in the optimization. 
\end{IEEEproof}
	
	\begin{lemma}
	\label{lem:solve_KKT}
	    A solution to problem (\ref{eq:relax_const_pert_posq}) is given by (\ref{eq:KKT_conditions_sol})
	\end{lemma}
	\begin{IEEEproof}
	Let $f_0(q)$ be the objective function of (\ref{eq:relax_const_pert_posq}).  The Lagrangian is given by 
	\begin{align} 
	&L(q, v, \lambda) = f_0(q) 
	\nonumber \\ & + v_1 \left(\sum_i q_{(i)} - 1 + (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & + v_2 \left(q_{(0)} - (1-p)^K \right) 
	\nonumber \\ & + v_3 \left(q_{(-n-1)} - (1-p)^K (1 - (1-p)^K)^{n+1} \right). 
	\end{align}
	
	The derivative of $f_0(q)$ with respect to $q_{(j)}$ is given by 
	\begin{align}
	& p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) \nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right)
	\end{align}  
	for $j \in \{-n, \; ..., \;  -1\}$ and the KKT conditions are given by 
	\begin{align}
	& q_{(0)} = (1-p)^K,
	\nonumber \\ & q_{(-n-1)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ &     \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2}
	\nonumber \\ & (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right) + v_1 + v_3 = 0 \quad 
	\nonumber \\ &  \text{for } j = - n -1
	\nonumber \\ & 	p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) 
	\nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right)+ v_1 = 0 
	\nonumber \\ &  \forall j \in \{-n, \; ..., \;  -1\}
	\nonumber \\ & p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) + v_1 + v_2 = 0 
	\nonumber \\ & \text{for } j = 0.
	\end{align}
	

	
	The last three conditions can be rewritten as 
	\begin{align} 
	& (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+1)}}{q_{(j)}} + (1-p) } \right) + v_1 + v_3 = 0  
	\nonumber \\ &  \text{for } j = - n - 1
	\nonumber \\ & p \log \left(\frac{p }{(1-p)\frac{q_{(j-1)}}{q_{(j)}} + p } \right) \nonumber \\ & + (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+1)}}{q_{(j)}} + (1-p) } \right)   + v_1  = 0 
	\nonumber \\ & \forall j \in \{-n, \; ..., \;  -1\}
	\nonumber \\ & p \log \left(\frac{p }{(1-p) \frac{q_{(j-1)}}{q_{(j)}} + p } \right)  + v_1 + v_2  = 0 \quad \text{for } j = 0
	\end{align}
	which shows that if the ratio $\frac{q_{(j-1)}}{q_{(j)}}$ between consecutive variables is the same for all $j,$  then $v_1,$ $v_2$ can  be chosen so that of these derivatives equal $0$ for all $j.$  Picking \[\frac{q_{(j-1)}}{q_{(j)}} = (1 - (1-p)^K),\] a solution to these equations is then
	\begin{align}
	& q_{(-i)} =  (1-p)^K (1 - (1-p)^K)^{i}  
	\nonumber \\ & \text{for } i \in \{0, \; 1, \; ..., \; n+1 \} 
	\nonumber \\ & v_1 = - p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & - (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right)
	\nonumber \\ & v_2 = (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & v_3 = p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right).
	\end{align}
	\end{IEEEproof}
	
	\rdcomment{this may be similar to the IS comments, but this proof is a bit hard to read for me. i understand the first few paragraphs in words, but it is not trivial to me to see exactly how this formally changes the problem. i would suggest stating the problem, and then how the support-constraint changes the optimization, and so on. to be honest, if you're tight on space, i still think it would be more beneficial to dedicate more space to this `reduction' and then even leave some of the more mechanical parts of derivatives/KKT condition analysis out.

also, we arrived at this result through figures and drawings; can we add some of this into the proof? i think it would strengthen the appeal of this paper to hint at why the idea is actually intuitive and cute. as written, it feels more a set of mechanical manipulations of KKT conditions, and it loses the sort of elegance i typically associate with info theory papers. (this is not a comment on the result, it's just a comment on the presentation and how it makes me feel.) i really liked the drawings of the convolution of discrete measures, and how we're really chosing a measure that gets shifted to the left by 1 and rescaled by 1-p and shifted to the right by 1 and rescaled by p. can this be put in this section at all?}

\rdcomment{stupid question: can you tell me a little more why (12) is this derivative? at a glance, it seems to be that there's a ton of term cancellations... (it's like the terms inside the log don't depend on $q_j$ with the way the derivative is written, so all those terms cancel?) i fear that a unfastidious reviewer may just claim this is a fundamental error and give a poor review without analyzing it deeply. (this happens sometimes to me.)}



==> main_result10_18_20.tex <==
\section{Main Results}


%\begin{figure}
%\centering
%\includegraphics[width=0.9\linewidth]{performance_plot_K6_minor_allele}
%\caption{}
%\label{fig:performance_plot_K6_minor_allele}
%\end{figure}

In order to tackle the discrete optimization problem in (\ref{eq:main2}), we seek to bound its optimal solution.
Our main result is the following lower bound.


% Our main result is a lower bound to (\ref{eq:main2})

\begin{theorem} \label{thm:main_lower_bound}
	For any $K\in \mathbb{N}$ and $p \in [0, 0.5],$  we have 
	\begin{align} 
	%& \min_{\alpha_i \in \mathbb{N}, \; i \in [K]\cup\{0\}}
	& \min_{\alpha \in \N^K}
	I(X \; ; \; \alpha_0 X +Z_\alpha) 
	\geq 
	I(X \; ; \; X - G),
	\end{align}
	where $G$ is a geometric random variable with
	$\Pr(G = i) = (1-p)^K(1 - (1-p)^K)^i$ for $i = 0,1,2,...$.
% 	success probability equal to $(1-p)^K$.
% 	and support equal to $\mathbb{N} \cup \{0\}.$
\end{theorem}

Intuitively, Theorem~\ref{thm:main_lower_bound} says that the noise distribution of $-G$ is worse than the worst-case noise $Z_\alpha$.
% for all $\alpha \in \N^K$.
This lower bound can in fact be explicitly computed as
% The formula for $I(X \; ; \; X - G)$ is given by 
\begin{align}
& I(X \; ; \; X - G)
% \nonumber \\ & 
= H(p) 
\nonumber \\ & - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{1-(1-p)^{K+1} }{(p-1) \left( (1-p)^K -1 \right)}\right) 
\nonumber \\ & - p \log \left( \frac{1-(1-p)^{K+1}}{p} \right)
\label{eq:closedform}
\end{align}
%\begin{align}
%& I(X \; ; \; X - G)
% \nonumber \\ & 
%= H(p) 
%\nonumber \\ & - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{1-(1-p)^{K+1} }{(p-1) \left( (1-p)^K -1 \right)}\right) 
%\nonumber \\ & - p \log %\left( \frac{1-(1-p)^{K+1}}{p} \right)
%\end{align}
% \iscomment{
% Can we extract a KL divergence between $p$ and $(1-p)^$
% }
Observe that the formula is quickly computable for any value of $K$ and $p,$ making it attractive from a computational standpoint.  To assess how tight the lower bound is, we empirically compare it to an upper bound that is computed with a greedy algorithm in Figure \ref{fig:greedy_versus_bound_K15}.  For a given $p$ and $K,$ the greedy algorithm chooses $\alpha_0 = 1, \; \alpha_1 = 1,$ and sequentially chooses \begin{align} \alpha_{j} = \argmin_{\alpha \in \mathbb{N} \; : \; 1 \leq \alpha \leq 1 + \sum_{i = 1}^{j-1}  \alpha_i} I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)
\end{align}
for $2 \leq j \leq K$.  
\iscomment{justify the upper bound of $1+\sum_{i=1}^{j-1}\alpha_i$ on $\alpha_j$}


As seen in Figure \ref{fig:greedy_versus_bound_K15}, $I(X \; ; \; X - G)$ serves as a very tight lower bound when compared with the upper bound.  
A similar picture can be obtained for other values of $K$.
Therefore, we can think of $I(X \; ; \; X - G)$ and its closed-form expression (\ref{eq:closedform}) as an approximation to the solution of (\ref{eq:main2}).  This is surprising, because for a given $K$, it is not possible in general to choose $\alpha_i$s to make the pmf of $\sum_{i = 1}^{j-1} \alpha_i Z_i$ look like 
% a shifted version of 
the pmf of  $-G$ or a shifted version of it.

While finding the greedy solution $(\alpha_0,...,\alpha_K)$ requires $\Omega(2^K)$ time in the worst case, similar plots to Figure \ref{fig:greedy_versus_bound_K15} can be obtained for larger values of $K$ using a more computationally efficient variation of the greedy algorithm that is discussed in the longer version of this paper \cite{long}.

In order to prove the lower bound on the minimization of $I(X \; ; \; \alpha_0 X + \sum_{i=1}^K \alpha_i Z_i)$ in Theorem \ref{thm:main_lower_bound}, we form a convex relaxation of the minimization problem, perturb the relaxation to form a problem that is analytically solvable using KKT conditions, and use perturbation analysis to find a lower bound on the relaxation.  
This is then a lower bound on the original problem.  
The full proof is provided in Section V.

\kmcomment{if get rid of Figure \ref{fig:greedy_versus_bound_K15} and move the two lemma proofs in the proof of main result section to the appendix, then the paper will be 5 pages.}

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .06]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{upper bound (greedy)}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\label{fig:greedy_versus_bound_K15}
\end{figure}


\longversion{

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Ratio: Upper Bound to Lower Bound},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
legend pos = north west]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt4_greedy_opt_ratio_K15.dat};
\addlegendentry{K = 15}

\addplot [
line width=1pt,
color=blue!80!black
] table[x index=0,y index=1] {data/plt4_greedy_opt_ratio_K10.dat};
\addlegendentry{K = 10}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt4_greedy_opt_ratio_K5.dat};
\addlegendentry{K = 5}

\end{axis}    
\end{tikzpicture}


\caption{}
\label{fig:greedy_versus_bound_K15}
\end{figure}


}

%\begin{tikzpicture}
%\begin{axis} 
%[title ={Comparison of Bounds: $K = 15$},
%ylabel = mutual information, 
%xlabel = minor allele frequency (p),
%ymax = .001,
%legend pos=north west]

%\addplot [
%line width=1pt,
%color=red!80!black
%] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{upper bound}

%\addplot [
%line width=1pt,
%color=blue!80!black
%] table[x index=0,y index=1] %{data/plt2_bound.dat};
%\addlegendentry{lower bound}

%\end{axis}    
%\end{tikzpicture}
%\caption{}
%\label{fig:greedy_versus_bound_K15}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p1}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p1}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p001}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p001}
%\end{figure}


%The lower bound is formally proved in the appendix, but we outline the argument here, as it sheds light on the problem, and makes interesting use of convex optimization theory

\section{Efficiently Computable Schemes}

Theorem~\ref{thm:main_lower_bound} provides a lower bound to the 
mutual information between $X$ and the lab's observation $Y$ for any mixing coefficients $\alpha_0,...,\alpha_K$, thus providing a bound to the privacy levels that can be achieved.
However, 


\rdcomment{this may sound stupid, but i think it warrants a sentence here. `Theorem 1 gives us a lower bound on the mutual information between $X$ and ..., which would be the mixing ratio that provides the highest level of privacy. However, it does not provide any mixing scheme for approaching this lower bound.'}

While much faster than brute force search, the greedy algorithm used to obtain the upper bound requires $\Omega(2^K)$ time in the worst case.  At a high level, this is due to the fact that at the $j$th  step in the algorithm, computation of $I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)$ requires use of each support value in the pmf of $\alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i,$ and there are $\Omega(2^j)$ support values in the worst case.  This motivates the design of efficiently computable schemes, which can then be evaluated using the lower bound in Theorem \ref{thm:main_lower_bound}.

Perhaps the most natural approach is given by the uniform scheme, which we define to set $\alpha_i = 1$ for all $i \in [K]\cup\{0\}.$  This is the scheme used by the authors of \cite{Maddah-Ali} to obtain their results.  The scheme is explicitly defined given $K,$ so no algorithm is needed to compute it.  The performance of the scheme for a given $p$ and $K$ can be computed in $O(K)$ time using the formula in Lemma \ref{lem:uniform_schem_formula} which is given in the appendix.

The uniform scheme is important because it is optimal as $p \to 0$ as proved in Lemma \ref{lem:optimality_of_uniform}
and exemplified by the optimal curve in Figure \ref{fig:optimal_scheme_K5_minor_allele}.

\begin{lemma}
\label{lem:optimality_of_uniform}
For any $K \in \mathbb{N},$ there exists some $p^* > 0$ such that the uniform scheme is optimal for $p < p^*.$
\end{lemma}

%\rdcomment{i changed epsilon to $p^*$ here. epsilon is typically taken to mean a very small constant, which makes this result feel weak, i.e. this result is only true when p is arbitrarily small.}

At $p= 0.5,$ in Figure \ref{fig:optimal_scheme_K5_minor_allele}, the optimal solution is given by the binary scheme, which we define to set $\alpha_0 = 1$ and $\alpha_i = 2^{i-1}$ for all $i \in [K].$  Similar to the uniform scheme, the binary scheme is explicitly defined given $K.$  Also, similar to the uniform scheme, there exists a formula for computing its performance given $p$ and $K$ in $O(K)$ time.  This formula is given in Lemma \ref{lem:binary_scheme_performance} in the appendix.  It is interesting that such a formula exists because the pmf of $\sum_{i=1}^K 2^{i-1} Z_i$ has $2^K$ support values. 

Most importantly, the optimality of the binary scheme at $p = 0.5$ for $K=5$ shown in Figure \ref{fig:optimal_scheme_K5_minor_allele} generalizes to all $K$ as proved in Lemma \ref{lem:optimality_of_binary}.

\begin{lemma} \label{lem:optimality_of_binary}
	For any $K \in \mathbb{N},$ the binary scheme is optimal for $p = 0.5.$
\end{lemma}

Because the uniform scheme is optimal for $p \to 0$ and the binary scheme is optimal for $p = 0.5,$  it is natural to try and combine these schemes to interpolate the performance for $p$ in the range $0<p<0.5.$  Combining only the uniform scheme and the binary scheme does not produce a scheme that approaches the lower bound.  However, the general shape of the lower bound can be captured in polynomial time by combining the uniform scheme, the linear scheme, and the binary scheme where the linear scheme is defined as $\alpha_0 = 1$ and $\alpha_i = i$ for $i \in [K].$  We define the $(K,L,U)$-binary-linear-uniform scheme to set $\alpha_0 = 1$ and 
\begin{align} &\alpha_i = 1 \quad i \in \{1, ..., U\} \nonumber \\  &\alpha_{U+i} = i \quad i \in \{1, ..., L\} \nonumber \\
&\alpha_{U+L+i} = 2^{i-1} \quad i \in \{1, ..., K-U-L\}
\end{align}

%\rdcomment{should it be binary-linear-uniform above?}

For a given $K$ and $p,$ we define the $K$-binary-linear-uniform scheme as the $(K,L^*,U^*)$-binary-linear-uniform scheme where
\begin{align} & (L^*, U^*) = \argmin_{(L,U) \in ([K]\cup\{0\})^2 \; : \; L + U \leq K} \\ &  I\left(X \; ; \; X + \sum_{i=1}^{U} Z_i + \sum_{j=1}^{L} j Z_{U+j} +  \sum_{k=1}^{K-U-L} 2^{k -1} Z_{U+L+k}\right) \nonumber.
\end{align}
The $K$-binary-linear-uniform scheme is computed in $O(K^4)$ time using a generalization of the recursion used to prove Lemma \ref{lem:binary_scheme_performance}.  

We compare the performance of the uniform scheme, the binary scheme, the $K$-binary-linear-uniform scheme, and the scheme generated by the greedy algorithm in Figure \ref{fig:efficiently_computable_schemes}.  We have observed that the scheme generated by the greedy algorithm is much tighter than the   $K$-binary-linear-uniform scheme after the initial hump in the lower bound as $K$ increases.



\begin{figure}[h]
\label{fig:efficiently_computable_schemes}
\centering
\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .6,
legend pos = north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}


\end{axis}    
\end{tikzpicture}

\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .01]
%,
%legend pos=north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
%\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
%\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
%\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
%\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
%\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\end{figure}



%Greedy takes exponential time in $K$ to compute.

%Simpler schemes: uniform, binary, interpolation between uniform and binary.


%Maybe state theorems about uniform and binary. Or maybe just mention them and refer to the longer version


\section{Proof of Theorem~\ref{thm:main_lower_bound}}

% We now present the proof of Theorem \ref{thm:main_lower_bound}.  
\iscomment{No need for the proof environment here}

% \begin{IEEEproof}
    First, notice that choosing integral $\alpha_i \; : \;  i \in [K] \cup \{0\}$ in the optimization problem (\ref{eq:main}) is optimal due to Lemma \ref{lem:integer_sol_optimal}, which holds because scaling the $\alpha_i$'s does not change the mutual information.  
    %Lemma \ref{lem:integer_sol_optimal} holds because if $\alpha_i = \frac{c_i}{b_i} \; \forall i$ in (\ref{eq:main}) where $c_i, b_i$ are integral, then the solution $\alpha_i = \frac{c_i}{b_i} \left(\Pi_j b_j\right) \; \forall i$ is integral and the mutual information is preserved. 
    We will thus consider (\ref{eq:main}) with the constraint that $\alpha_i \in \mathbb{N}$ for $i \in [K] \cup \{0\}.$
    
    \begin{lemma}
        \label{lem:integer_sol_optimal}
        If an optimal solution to (\ref{eq:main}) exists, then there exists an optimal solution to (\ref{eq:main}) with $\alpha_i \in \mathbb{N}$ for $i \in [K] \cup \{0\}.$
    \end{lemma}
    
    Let $ Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i.$ We obtain the lower bound on $I(X \, ; \, \alpha_0 X + Z_{\alpha})= H(p) - H(X \, | \, \alpha_0 X+Z_{\alpha})$ in Theorem~\ref{thm:main_lower_bound} by finding a lower bound on $-H(X \, | \, \alpha_0 X+Z_{\alpha}).$  The optimization problem we consider is therefore
    \begin{align}
       \label{eq:integral_alpha_opt_prob}
        & \min_{\alpha_0,...,\alpha_K \in \mathbb{N}} -H\left(X \; \left| \; \alpha_{0} X+\sum_{k=1}^K \alpha_k Z_k \right. \right).
    \end{align}
    Observe that the pmf of the random variable $Z_{\alpha} = \sum_{i = 1}^K \alpha_i Z_i$ has probability $(1-p)^{K}$ at its highest support value. 
    More precisely, $\sum_{i=1}^k \alpha_K$ is the maximum value that $Z_\alpha$ can take, which occurs with probability $(1-p)^{K}$.
    % Furthermore, we notice that adding a constant to $Z_\alpha$ does not 
    % the following problem is clearly 
    A relaxation to (\ref{eq:integral_alpha_opt_prob}) can be then obtained by ignoring all constraint on the pmf of $Z_\alpha$ except for the maximum pmf value.
    Thus, a relaxation to (\ref{eq:integral_alpha_opt_prob}) is given by
    \begin{align}
       \label{eq:relax_inf1}
        \min_{D} \; &  -H\left(X \; | \; \alpha_0 X+D\right)
        \\\text{subject to:} \; & 
        \nonumber 
        % \\ 
        D \text{ is an integer-valued random variable} \nonumber
        % \nonumber \\ & D  \text{ has maximum support value at 0} 
        \\ & \Pr(D = 0) = (1-p)^K \nonumber
        \\ & \Pr(D = i) = 0 \; \text{ for $i > 0$}.
        \nonumber
    \end{align}
    Due to Lemma \ref{lem:alpha0_condition}, we can fix $\alpha_0 = 1$ in (\ref{eq:relax_inf1}) above without changing the optimal value.  Let $q_{(0)}$ be the probability at the maximum support value of $D$ and let $q_{(-i)}$ be the probability at the $i$th integer below the maximum support value of $D.$ Define
    \begin{align}
        & g_j(q) = (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right) 
	    \nonumber \\ & + p q_{(j+1)} \log \left(\frac{p q_{(j+1)}}{(1-p)q_{(j)} + p q_{(j+1)}} \right).
    \end{align}
    Written more explicitly  with $\alpha_0 = 1$ fixed, (\ref{eq:relax_inf1}) is given by
    \begin{align}
    \label{eq:relax_inf2}
	& \min_{q_{(-i)} \geq 0 : \; i \in \mathbb{N}\cup\{0\} } \sum_{j \in \{-n : \; n \in \mathbb{N}\}} g_j(q)
    \\ &  \text{subject to:} \quad \nonumber \\ & \quad q_{(0)} = (1-p)^K, \quad    \sum_{j} q_{(j)} = 1 \nonumber
	\end{align}  
    Note that the conditional entropy in the objective function is in a simplified form.   
    
    Observe that (\ref{eq:relax_inf2}) is an infinite dimensional convex minimization problem.  A solution to the KKT conditions with the added implicit constraint that $q_{(-i)}>0$ for $i \in \mathbb{N} \cup \{0\}$  is given by  $q_{(-i)} = (1-p)^K (1 - (1-p)^K)^i$ for $i \in \mathbb{N} \cup \{0\}$ which corresponds to $D = -G$ in (\ref{eq:relax_inf1}) where $G$ is a geometric random variable with success probability equal to $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\}.$  We do not use this observation directly to establish Theorem \ref{theorem:main_recursion} because no reference on the relation between KKT conditions and optimality in the infinite dimensional case was found.  
    
    Instead, we constrain $D$ to have distance no greater than $n \in \mathbb{N}$ between its maximum and minimum support values in (\ref{eq:relax_inf2}), derive a lower bound on the solution for each $n \in \mathbb{N},$ and use the resulting sequence of lower bounds to establish the result. The support constrained version of (\ref{eq:relax_inf2}) is given by 
    \begin{align}
    \label{eq:relax_const}
    & \min_{q_{(-i)} \geq 0 : \; i \in [n+1]\cup\{0\} }
    \sum_{j \in \{-m : \; m \in [n+1]\}} g_j(q) \\ &  \text{subject to:} \nonumber \\ & 
    \quad q_{(0)} = (1-p)^K, \quad q_{(-n-1)} = 0,  \quad    \sum_{j} q_{(j)} = 1. \nonumber
	\end{align}  

    Changing the implicit constraint in (\ref{eq:relax_const}) from $q_{(i)} \geq 0$ to $q_{(i)} > 0$ and the explicit constraint $q_{(-n-1)} = 0$ to $q_{(-n-1)} = \epsilon$ where $\epsilon \in \mathbb{R}_{>0}$ gives us
    \begin{align}
    \label{eq:relax_const_posq}
    & \min_{q_{(-i)} > 0 : \; i \in [n+1]\cup\{0\} }
    \sum_{j \in \{-m : \; m \in [n+1]\}} g_j(q)
    \\ &  \text{subject to:} \nonumber \\ & 
    \quad q_{(0)} = (1-p)^K, \quad q_{(-n-1)} = \epsilon, \quad    \sum_{j} q_{(j)} = 1. \nonumber
	\end{align}  

    Let $p^*$ be the optimal value of \ref{eq:relax_const} and let $p_{\epsilon}^*$ be the optimal value of \ref{eq:relax_const_posq} for a given $\epsilon.$ Due to the continuity of the objective function in (\ref{eq:relax_const}), it is not hard to show that $ p^* \geq \inf_{\epsilon \in \mathbb{R}_{>0}} p_{\epsilon}^*.$  At a high level, this is due to the fact that for any solution to  (\ref{eq:relax_const}), it follows that (\ref{eq:relax_const_posq}) can get arbitrarily close to it as $\epsilon \to 0$ due to the continuity of the objective function.  



    While we do not know the solution to (\ref{eq:relax_const}) or (\ref{eq:relax_const_posq}), we will perturb (\ref{eq:relax_const_posq}) to form a problem we can solve analytically, then use perturbation analysis to lower bound the optimal value of (\ref{eq:relax_const_posq}), and ultimately lower bound the optimal value of (\ref{eq:relax_const}).  The perturbed version of (\ref{eq:relax_const_posq}) is given by 
	\begin{align}
	\label{eq:relax_const_pert_posq}
    & \min_{q_{(-i)} > 0 : \; i \in [n+1]\cup\{0\} }
    \sum_{j \in \{-m : \; m \in [n+1]\}} g_j(q) \\	& 
	\text{subject to:} \nonumber \\
	& q_{(0)} = (1-p)^K, \quad q_{(-n-1)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ &     \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2} \nonumber
	\end{align}  
    where we have changed the constraint on the probability at the minimum support value, and the constraint on the sum of all the probabilities.
    We can solve this by solving the KKT conditions since the problem is convex, Slater's condition holds, and the objective function and constraint functions are differentiable on the domain $q_{(i)} > 0.$  
    
    We proceed to find the solution to the KKT conditions for (\ref{eq:relax_const_pert_posq}).  Let $f_0(q)$ be the objective function of (\ref{eq:relax_const_pert_posq}).  The Lagrangian is given by 
	\begin{align} 
	&L(q, v, \lambda) = f_0(q) 
	\nonumber \\ & + v_1 \left(\sum_i q_{(i)} - 1 + (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & + v_2 \left(q_{(0)} - (1-p)^K \right) 
	\nonumber \\ & + v_3 \left(q_{(-n-1)} - (1-p)^K (1 - (1-p)^K)^{n+1} \right). 
	\end{align}
	By Lemma \ref{lem:solve_KKT}, a solution to the KKT conditions is given by 
	\begin{align}
	\label{eq:KKT_conditions_sol}
	& q_{(-i)} =  (1-p)^K (1 - (1-p)^K)^{i}  \text{ for } i \in [n+1] \cup \{0\} 
	\nonumber \\ & v_1 = - p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & - (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right)
	\nonumber \\ & v_2 = (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & v_3 = p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right),
	\end{align}
    which is then an optimal solution to (\ref{eq:relax_const_pert_posq}).  %The optimal value for (\ref{eq:relax_const_pert_posq}) is therefore given by 
	%\begin{align} 
	%& \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
	%\nonumber \\ & - p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	%\nonumber \\ & = \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	%\nonumber \\ & - p \beta \alpha^i \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	%\end{align}
	Applying the geometric sum formula and simplifying,  the optimal value for (\ref{eq:relax_const_pert_posq}) is   
	\begin{align} 
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\end{align}
	where $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K.$  
	
	Using the perturbation analysis from Section 5.6.1 of \cite{boyd}, we see that the optimal value of (\ref{eq:relax_const_posq}) is lower bounded by
	\begin{align}
	\label{eq:relax_const_posq_bound}
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\nonumber \\ & - v_1^* \left( (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & - v_3^* \left(- (1-p)^K (1 - (1-p)^K)^{n+1} +\epsilon \right) 
	\end{align} 
	where $v_1^*$ and $v_3^*$ are the optimal lagrange multipliers for (\ref{eq:relax_const_pert_posq})
	we determined through the KKT conditions.
	
	Taking the infimum of (\ref{eq:relax_const_posq_bound}) over $\epsilon \in \mathbb{R}_{>0}$ yields the following lower bound on (\ref{eq:relax_const}):
	
	\begin{align}
	\label{eq:relax_const_bound}
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\nonumber \\ & - v_1^* \left( (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & - v_3^* \left(- (1-p)^K (1 - (1-p)^K)^{n+1} \right). 
	\end{align} 
	
	The sequence of optimal values returned by (\ref{eq:relax_const}) is monotonically decreasing in $n$ clearly.  Thus, taking the limit of the lower bound (\ref{eq:relax_const_bound}) as  $n \to \infty$ and simplifying yields the following lower bound on $-H(X \; | \; \alpha_0 X + Z_{\alpha})$ for any choice of $\alpha_i$'s: \begin{align} 
	\label{eq:lower_bound_neg_cond_ent}
	& -(p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right).
	\end{align}
	
	Finally, observe that
	$-H(X \; ; \; X - G)$ is equal to (\ref{eq:lower_bound_neg_cond_ent})
	where $G$ is a geometric random variable with
	$\Pr(G = i) = (1-p)^K(1 - (1-p)^K)^i$ for $i \in  \mathbb{N} \cup \{0\}.$
% \end{IEEEproof}	

\begin{lemma}
    \label{lem:alpha0_condition}
    Fixing $\alpha_0 = 1$ in (\ref{eq:relax_const}) can not increase the optimal value.
\end{lemma}

\begin{IEEEproof}
    Let $\alpha_0 \in \mathbb{N}.$ 
	Let $Z$ be any random variable such that its pmf has integral support and maximum support value at $t = 0.$  Let 
	\begin{align}
	& \hat{Z} = Z - S
	\end{align} 
	where $S = Z \mod{\alpha_0}.$ 
	We then have that 
	\begin{align}
	& I(X ; \alpha_0 X + 	Z)  \geq I(X ; \alpha_0 X + \hat{Z}).   
	\end{align} 
	because
	\begin{align} 
		& I(X ; \; \alpha_0 X + 	Z)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z} +  S)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z}, \; S)
		\nonumber \\ & = I(X ; \; S) + I(X ; \; \alpha_0 X + \hat{Z} \; | \; S)
		\nonumber \\ & = I(X ; \; \alpha_0 X + \hat{Z} \; | \; S)
		\nonumber \\ & = H(X \; | \; S)  - H(X \; | \; \alpha_0 X + \hat{Z}, \; S) 
		\nonumber \\ & = H(X)  - H(X \; | \; \alpha_0 X + \hat{Z}, \; S)
		\nonumber \\ & \geq H(X)  - H(X \; | \; \alpha_0 X + \hat{Z})
		\nonumber \\ & = I(X \; ; \; \alpha_0 X + \hat{Z})
	\end{align} 
	where the third line follows because given $\alpha_0 X + \hat{Z} + S,$ we have that 
	\begin{align}
	    S = ((\alpha_0 X + \hat{Z} + S) - \alpha_0) \mod  \alpha_0 
	\end{align}
	and
    \begin{align}
	    \alpha_0 X + \hat{Z} = (\alpha_0 X + \hat{Z} + S) - S.
	\end{align}
	Thus, any solution to (\ref{eq:relax_inf1}) with  $\alpha_0 = a$ can be transformed into a solution whose pmf had support values in $\{t a : \; t \in \mathbb{Z}\}$ without increasing the mutual information.   Therefore, for a fixed $\alpha_0,$ it suffices to only consider pmfs that have support values in $\{t \alpha_0 : \; t \in \mathbb{Z}\}$ in the optimization.  If $\alpha_0 = a ,$ any solution random variable $D$ with  support values in $\{t a : \; t \in \mathbb{Z}\}$ can be transformed into a solution with the same mutual information, $\alpha_0 = 1,$ and support values in $\{t : \; t \in \mathbb{Z}\}.$ This is accomplished by dividing $D$ by $a.$  Therefore it suffices to fix $\alpha_0=1$ in the optimization. 
\end{IEEEproof}
	
	\begin{lemma}
	\label{lem:solve_KKT}
	    A solution to problem (\ref{eq:relax_const_pert_posq}) is given by (\ref{eq:KKT_conditions_sol})
	\end{lemma}
	\begin{IEEEproof}
	Let $f_0(q)$ be the objective function of (\ref{eq:relax_const_pert_posq}).  The Lagrangian is given by 
	\begin{align} 
	&L(q, v, \lambda) = f_0(q) 
	\nonumber \\ & + v_1 \left(\sum_i q_{(i)} - 1 + (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & + v_2 \left(q_{(0)} - (1-p)^K \right) 
	\nonumber \\ & + v_3 \left(q_{(-n-1)} - (1-p)^K (1 - (1-p)^K)^{n+1} \right). 
	\end{align}
	
	The derivative of $f_0(q)$ with respect to $q_{(j)}$ is given by 
	\begin{align}
	& p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) \nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right)
	\end{align}  
	for $j \in \{-n, \; ..., \;  -1\}$ and the KKT conditions are given by 
	\begin{align}
	& q_{(0)} = (1-p)^K,
	\nonumber \\ & q_{(-n-1)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ &     \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2}
	\nonumber \\ & (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right) + v_1 + v_3 = 0 \quad 
	\nonumber \\ &  \text{for } j = - n -1
	\nonumber \\ & 	p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) 
	\nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+1)} + (1-p) q_{(j)}} \right)+ v_1 = 0 
	\nonumber \\ &  \forall j \in \{-n, \; ..., \;  -1\}
	\nonumber \\ & p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-1)} + p q_{(j)}} \right) + v_1 + v_2 = 0 
	\nonumber \\ & \text{for } j = 0.
	\end{align}
	

	
	The last three conditions can be rewritten as 
	\begin{align} 
	& (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+1)}}{q_{(j)}} + (1-p) } \right) + v_1 + v_3 = 0  
	\nonumber \\ &  \text{for } j = - n - 1
	\nonumber \\ & p \log \left(\frac{p }{(1-p)\frac{q_{(j-1)}}{q_{(j)}} + p } \right) \nonumber \\ & + (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+1)}}{q_{(j)}} + (1-p) } \right)   + v_1  = 0 
	\nonumber \\ & \forall j \in \{-n, \; ..., \;  -1\}
	\nonumber \\ & p \log \left(\frac{p }{(1-p) \frac{q_{(j-1)}}{q_{(j)}} + p } \right)  + v_1 + v_2  = 0 \quad \text{for } j = 0
	\end{align}
	which shows that if the ratio $\frac{q_{(j-1)}}{q_{(j)}}$ between consecutive variables is the same for all $j,$  then $v_1,$ $v_2$ can  be chosen so that of these derivatives equal $0$ for all $j.$  Picking \[\frac{q_{(j-1)}}{q_{(j)}} = (1 - (1-p)^K),\] a solution to these equations is then
	\begin{align}
	& q_{(-i)} =  (1-p)^K (1 - (1-p)^K)^{i}  
	\nonumber \\ & \text{for } i \in \{0, \; 1, \; ..., \; n+1 \} 
	\nonumber \\ & v_1 = - p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & - (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right)
	\nonumber \\ & v_2 = (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & v_3 = p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right).
	\end{align}
	\end{IEEEproof}
	
	\rdcomment{this may be similar to the IS comments, but this proof is a bit hard to read for me. i understand the first few paragraphs in words, but it is not trivial to me to see exactly how this formally changes the problem. i would suggest stating the problem, and then how the support-constraint changes the optimization, and so on. to be honest, if you're tight on space, i still think it would be more beneficial to dedicate more space to this `reduction' and then even leave some of the more mechanical parts of derivatives/KKT condition analysis out.

also, we arrived at this result through figures and drawings; can we add some of this into the proof? i think it would strengthen the appeal of this paper to hint at why the idea is actually intuitive and cute. as written, it feels more a set of mechanical manipulations of KKT conditions, and it loses the sort of elegance i typically associate with info theory papers. (this is not a comment on the result, it's just a comment on the presentation and how it makes me feel.) i really liked the drawings of the convolution of discrete measures, and how we're really chosing a measure that gets shifted to the left by 1 and rescaled by 1-p and shifted to the right by 1 and rescaled by p. can this be put in this section at all?}

\rdcomment{stupid question: can you tell me a little more why (12) is this derivative? at a glance, it seems to be that there's a ton of term cancellations... (it's like the terms inside the log don't depend on $q_j$ with the way the derivative is written, so all those terms cancel?) i fear that a unfastidious reviewer may just claim this is a fundamental error and give a poor review without analyzing it deeply. (this happens sometimes to me.)}



==> main_result10_19_20.tex <==
\section{Main Results}


%\begin{figure}
%\centering
%\includegraphics[width=0.9\linewidth]{performance_plot_K6_minor_allele}
%\caption{}
%\label{fig:performance_plot_K6_minor_allele}
%\end{figure}

In order to tackle the discrete optimization problem in (\ref{eq:main2}) in the entire interval $p \in [0,0.5]$, we seek to bound its optimal solution.
Our main result is the following lower bound.


% Our main result is a lower bound to (\ref{eq:main2})

\begin{theorem} \label{thm:main_lower_bound}
	For any $K\in \mathbb{N}$ and $p \in [0, 0.5],$  we have 
	\begin{align} 
	%& \min_{\alpha_i \in \mathbb{N}, \; i \in [K]\cup\{0\}}
	& \min_{\alpha \in \N^{K+1}}
	I(X \; ; \; \alpha_0 X +Z_\alpha) 
	\geq 
	I(X \; ; \; X - G),
	\end{align}
	where $G$ is a geometric random variable with
	$\Pr(G = i) = (1-p)^K(1 - (1-p)^K)^i$ for $i = 0,1,2,...$.
% 	success probability equal to $(1-p)^K$.
% 	and support equal to $\mathbb{N} \cup \{0\}.$
\end{theorem}

Intuitively, Theorem~\ref{thm:main_lower_bound} says that the noise distribution of $-G$ is worse than the worst-case noise $Z_\alpha$.
% for all $\alpha \in \N^{K+1}$.
This lower bound can in fact be explicitly computed as
% The formula for $I(X \; ; \; X - G)$ is given by 
\begin{align}
& I(X \; ; \; X - G)
% \nonumber \\ & 
= H(p) 
\nonumber \\ & - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{1-(1-p)^{K+1} }{(p-1) \left( (1-p)^K -1 \right)}\right) 
\nonumber \\ & - p \log \left( \frac{1-(1-p)^{K+1}}{p} \right)
\label{eq:closedform}
\end{align}
%\begin{align}
%& I(X \; ; \; X - G)
% \nonumber \\ & 
%= H(p) 
%\nonumber \\ & - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{1-(1-p)^{K+1} }{(p-1) \left( (1-p)^K -1 \right)}\right) 
%\nonumber \\ & - p \log %\left( \frac{1-(1-p)^{K+1}}{p} \right)
%\end{align}
% \iscomment{
% Can we extract a KL divergence between $p$ and $(1-p)^$
% }
Observe that the formula is quickly computable for any value of $K$ and $p,$ making it attractive from a computational standpoint.  To assess how tight the lower bound is, we empirically compare it to an upper bound that is computed with a greedy algorithm in Figure \ref{fig:greedy_versus_bound_K15}.  For a given $p$ and $K,$ the greedy algorithm chooses $\alpha_0 = 1, \; \alpha_1 = 1,$ and sequentially chooses \begin{align} \alpha_{j} = \argmin_{\alpha \in \mathbb{N} \; : \; 1 \leq \alpha \leq 1 + \sum_{i = 1}^{j-1}  \alpha_i} I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)
\end{align}
for $2 \leq j \leq K$.  At the $j$th step we consider all $\alpha$'s between $1$ and $1 + \sum_{i = 1}^{j-1} \alpha_i$ because $1 + \sum_{i = 1}^{j-1} \alpha_i$ is the highest choice for $\alpha$ that does not increase the number of support values $t$ where $H(X \; | \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i=t) = 0.$ 
\iscomment{justify the upper bound of $1+\sum_{i=1}^{j-1}\alpha_i$ on $\alpha_j$}


As seen in Figure \ref{fig:greedy_versus_bound_K15}, $I(X \; ; \; X - G)$ serves as a very tight lower bound when compared with the upper bound.  
A similar picture can be obtained for other values of $K$.
Therefore, we can think of $I(X \; ; \; X - G)$ and its closed-form expression (\ref{eq:closedform}) as an approximation to the solution of (\ref{eq:main2}).  This is surprising, because for a given $K$, it is not possible in general to choose $\alpha_i$s to make the pmf of $\sum_{i = 1}^{j-1} \alpha_i Z_i$ look like 
% a shifted version of 
the pmf of  $-G$ or a shifted version of it.

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Ratio: Upper Bound to Lower Bound},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
legend pos = north west]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt4_greedy_opt_ratio_K15.dat};
\addlegendentry{K = 15}

\addplot [
line width=1pt,
color=blue!80!black
] table[x index=0,y index=1] {data/plt4_greedy_opt_ratio_K10.dat};
\addlegendentry{K = 10}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt4_greedy_opt_ratio_K5.dat};
\addlegendentry{K = 5}

\end{axis}    
\end{tikzpicture}


\caption{}
\label{fig:greedy_versus_bound_K15}
\end{figure}


\iscomment{Maybe a nice figure to have here would be one comparing the pmfs of $-G$ and $Z_{\alpha^*}$.
}
\kmcomment{I'll get this plot as soon as I can}


While finding the greedy solution $(\alpha_0,...,\alpha_K)$ requires $\Omega(2^K)$ time in the worst case, similar plots to Figure \ref{fig:greedy_versus_bound_K15} can be obtained for larger values of $K$ using a more computationally efficient variation of the greedy algorithm that is discussed in the longer version of this paper \cite{long}.

At a high level, we prove the lower bound on the minimization of $I(X \; ; \; \alpha_0 X + \sum_{i=1}^K \alpha_i Z_i)$ in Theorem \ref{thm:main_lower_bound} by forming a convex relaxation of the minimization problem, perturbing the relaxation to form a problem that is analytically solvable using KKT conditions, and using perturbation analysis to find a lower bound on the relaxation.  
This is then a lower bound on the original problem.  
The full proof is provided in Section IV.

%\kmcomment{if get rid of Figure \ref{fig:greedy_versus_bound_K15} and move the two lemma proofs in the proof of main result section to the appendix, then the paper will be 5 pages.}

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .06]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{upper bound (greedy)}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\label{fig:greedy_versus_bound_K15}
\end{figure}


\longversion{

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Ratio: Upper Bound to Lower Bound},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
legend pos = north west]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt4_greedy_opt_ratio_K15.dat};
\addlegendentry{K = 15}

\addplot [
line width=1pt,
color=blue!80!black
] table[x index=0,y index=1] {data/plt4_greedy_opt_ratio_K10.dat};
\addlegendentry{K = 10}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt4_greedy_opt_ratio_K5.dat};
\addlegendentry{K = 5}

\end{axis}    
\end{tikzpicture}


\caption{}
\label{fig:greedy_versus_bound_K15}
\end{figure}


}

%\begin{tikzpicture}
%\begin{axis} 
%[title ={Comparison of Bounds: $K = 15$},
%ylabel = mutual information, 
%xlabel = minor allele frequency (p),
%ymax = .001,
%legend pos=north west]

%\addplot [
%line width=1pt,
%color=red!80!black
%] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{upper bound}

%\addplot [
%line width=1pt,
%color=blue!80!black
%] table[x index=0,y index=1] %{data/plt2_bound.dat};
%\addlegendentry{lower bound}

%\end{axis}    
%\end{tikzpicture}
%\caption{}
%\label{fig:greedy_versus_bound_K15}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p1}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p1}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p001}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p001}
%\end{figure}


%The lower bound is formally proved in the appendix, but we outline the argument here, as it sheds light on the problem, and makes interesting use of convex optimization theory






%Greedy takes exponential time in $K$ to compute.

%Simpler schemes: uniform, binary, interpolation between uniform and binary.


%Maybe state theorems about uniform and binary. Or maybe just mention them and refer to the longer version






==> main_result_old.tex <==
\section{Main Result}


%\begin{figure}
%\centering
%\includegraphics[width=0.9\linewidth]{performance_plot_K6_minor_allele}
%\caption{}
%\label{fig:performance_plot_K6_minor_allele}
%\end{figure}

Our main result is stated below.

\begin{theorem} \label{thm:main_lower_bound}
	For any $K\in \mathbb{N},$ $p \in [0, 0.5],$ and $\alpha_i \in \mathbb{N}, \; i \in [K],$  we have that 
	\begin{align} 
	& \min_{\alpha_i \in \mathbb{N}, \; i \in [K]} I(X \; ; \; X + \sum_{i=1}^{K} \alpha_i Z_i) 
% 	\nonumber \\ & 
	\geq 
	I(X \; ; \; X - 2G)
	\end{align}
	where $G$ is a geometric random variable with success probability equal to $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\}.$
\end{theorem}
The formula for $I(X \; ; \; X - 2G)$ is given by 
\begin{align}
& I(X \; ; \; X - 2G)
\nonumber \\ & = H(p) 
\nonumber \\ & - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
\end{align}
Observe that the formula is quickly computable for any value of $K$ and $p,$ making it attractive from a computational standpoint.  To assess how tight the lower bound is, we empirically compare it to an upper bound that is computed with a greedy algorithm in Figure \ref{fig:greedy_versus_bound_K15}.  For a given $p$ and $K,$ the greedy algorithm chooses $\alpha_1 = 1,$ and sequentially chooses \begin{align} \alpha_{j} = \argmin_{\alpha \in \mathbb{N} \; : \; 1 \leq \alpha \leq 1 + \sum_{i = 1}^{j-1}  \alpha_i} I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)
\end{align}
for $2 \leq j \leq K.$  As seen in Figure \ref{fig:greedy_versus_bound_K15}, $I(X \; ; \; X - 2G)$ serves as a very tight lower bound when compared with the upper bound.  We therefore view $I(X \; ; \; X - 2G)$ as an approximation to the original problem.

While the greedy algorithm requires $\Omega(2^K)$ time in the worst case, similar plots to Figure \ref{fig:greedy_versus_bound_K15} can be obtained for larger values of $K$ using a more computationally efficient variation of the greedy algorithm that is discussed in the longer version of this paper.

In order to prove the lower bound on the minimization of $I(X \; ; \; X + \sum_{i=1}^K \alpha_i Z_i)$ in Theorem \ref{thm:main_lower_bound}, we form a convex relaxation of the minimization problem, perturb the relaxation to form a problem that is analytically solvable using KKT conditions, and use perturbation analysis to find a lower bound on the relaxation.  This is then a lower bound on the original problem.  The full proof is in the Section V.

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .06]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{upper bound (greedy)}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\label{fig:greedy_versus_bound_K15}
\end{figure}

%\begin{tikzpicture}
%\begin{axis} 
%[title ={Comparison of Bounds: $K = 15$},
%ylabel = mutual information, 
%xlabel = minor allele frequency (p),
%ymax = .001,
%legend pos=north west]

%\addplot [
%line width=1pt,
%color=red!80!black
%] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{upper bound}

%\addplot [
%line width=1pt,
%color=blue!80!black
%] table[x index=0,y index=1] %{data/plt2_bound.dat};
%\addlegendentry{lower bound}

%\end{axis}    
%\end{tikzpicture}
%\caption{}
%\label{fig:greedy_versus_bound_K15}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p1}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p1}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.9\linewidth]{greedy_versus_bound_K15_ylim_0p001}
%\caption{}
%\label{fig:greedy_versus_bound_K15_ylim_0p001}
%\end{figure}


%The lower bound is formally proved in the appendix, but we outline the argument here, as it sheds light on the problem, and makes interesting use of convex optimization theory

\section{Efficiently Computable Schemes}

\rdcomment{this may sound stupid, but i think it warrants a sentence here. `Theorem 1 gives us a lower bound on the mutual information between $X$ and ..., which would be the mixing ratio that provides the highest level of privacy. However, it does not provide any mixing scheme for approaching this lower bound.'}

While much faster than brute force search, the greedy algorithm used to obtain the upper bound requires $\Omega(2^K)$ time in the worst case.  At a high level, this is due to the fact that at the $j$th  step in the algorithm, computation of $I(X \; ; \; X + \alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i)$ requires use of each support value in the PMF of $\alpha Z_{j} + \sum_{i = 1}^{j-1} \alpha_i Z_i,$ and there are $\Omega(2^j)$ support values in the worst case.  This motivates the design of efficiently computable schemes, which can then be evaluated using the lower bound in Theorem \ref{thm:main_lower_bound}.

Perhaps the most natural approach is given by the uniform scheme, which we define to set $\alpha_i = 1$ for all $i \in [K].$  This is the scheme used by the authors of \cite{Maddah-Ali} to obtain their results.  The scheme is explicitly defined given $K,$ so no algorithm is needed to compute it.  The performance of the scheme for a given $p$ and $K$ can be computed in $O(K)$ time using the formula in Lemma \ref{lem:uniform_schem_formula} which is given in the appendix.

The uniform scheme is important because it is optimal as $p \to 0$ as proved in Lemma \ref{lem:optimality_of_uniform}
and exemplified by the optimal curve in Figure \ref{fig:optimal_scheme_K5_minor_allele}.

\begin{lemma}
\label{lem:optimality_of_uniform}
For any $K \in \mathbb{N},$ there exists some $p^* > 0$ such that the uniform scheme is optimal for $p < p^*.$
\end{lemma}

\rdcomment{i changed epsilon to $p^*$ here. epsilon is typically taken to mean a very small constant, which makes this result feel weak, i.e. this result is only true when p is arbitrarily small.}

At $p= 0.5,$ in Figure \ref{fig:optimal_scheme_K5_minor_allele}, the optimal solution is given by the binary scheme, which we define to set $\alpha_i = 2^{i-1}$ for all $i \in [K].$  Similar to the uniform scheme, the binary scheme is explicitly defined given $K.$  Also, similar to the uniform scheme, there exists a formula for computing its performance given $p$ and $K$ in $O(K)$ time.  This formula is given in Lemma \ref{lem:binary_scheme_performance} in the appendix.  It is interesting that such a formula exists because the PMF of $\sum_{i=1}^K 2^{i-1} Z_i$ has $2^K$ support values. 

Most importantly, the optimality of the binary scheme at $p = 0.5$ for $K=5$ shown in Figure \ref{fig:optimal_scheme_K5_minor_allele} generalizes to all $K$ as proved in Lemma \ref{lem:optimality_of_binary}.

\begin{lemma} \label{lem:optimality_of_binary}
	For any $K \in \mathbb{N},$ the binary scheme is optimal for $p = 0.5.$
\end{lemma}

Because the uniform scheme is optimal for $p \to 0$ and the binary scheme is optimal for $p = 0.5,$  it is natural to try and combine these schemes to interpolate the performance for $p$ in the range $0<p<0.5.$  Combining only the uniform scheme and the binary scheme does not produce a scheme that approaches the lower bound.  However, the general shape of the lower bound can be captured in polynomial time by combining the uniform scheme, the linear scheme, and the binary scheme where the linear scheme is defined as $\alpha_i = i$ for $i \in [K].$  We define the $(K,L,U)$-binary-linear-uniform scheme to set
\begin{align} &\alpha_i = 1 \quad i \in \{1, ..., U\} \nonumber \\  &\alpha_{U+i} = i \quad i \in \{1, ..., L\} \nonumber \\
&\alpha_{U+L+i} = 2^{i-1} \quad i \in \{1, ..., K-U-L\}
\end{align}

\rdcomment{should it be binary-linear-uniform above?}

For a given $K$ and $p,$ we define the $K$-binary-linear-uniform scheme as the $(K,L^*,U^*)$-binary-linear-uniform scheme where
\begin{align} & (L^*, U^*) = \argmin_{(L,U) \in ([K]\cup\{0\})^2 \; : \; L + U \leq K} \\ &  I\left(X \; ; \; X + \sum_{i=1}^{U} Z_i + \sum_{j=1}^{L} j Z_{U+j} +  \sum_{k=1}^{K-U-L} 2^{k -1} Z_{U+L+k}\right) \nonumber.
\end{align}
The $K$-binary-linear-uniform scheme is computed in $O(K^4)$ time using a generalization of the recursion used to prove Lemma \ref{lem:binary_scheme_performance}.  

We compare the performance of the uniform scheme, the binary scheme, the $K$-binary-linear-uniform scheme, and the scheme generated by the greedy algorithm in Figure \ref{fig:efficiently_computable_schemes}.  We have observed that the greedy scheme generated by the greedy algorithm is much tighter than the   $K$-binary-linear-uniform scheme after the initial hump in the lower bound as $K$ increases.



\begin{figure}[h]
\label{fig:efficiently_computable_schemes}
\centering
\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .6,
legend pos = north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
\addlegendentry{lower bound}


\end{axis}    
\end{tikzpicture}

\begin{tikzpicture}[scale=0.8]
\begin{axis}
[width=0.47\textwidth,
height=0.36\textwidth,
title ={Comparison of Bounds: $K = 15$},
ylabel = mutual information, 
xlabel = minor allele frequency (p),
ymax = .01]
%,
%legend pos=north east]

\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt2_greedy.dat};
%\addlegendentry{greedy}

\addplot [
line width=1pt,
color=green!80!black
] table[x index=0,y index=1] {data/plt3_uniform.dat};
%\addlegendentry{uniform}

\addplot [
line width=1pt,
color=purple!80!black
] table[x index=0,y index=1] {data/plt3_linear.dat};
%\addlegendentry{linear}

\addplot [
line width=1pt,
color=orange!80!black
] table[x index=0,y index=1] {data/plt3_binary.dat};
%\addlegendentry{binary}

\addplot [
line width=1pt,
color=yellow!80!black,
dashed
] table[x index=0,y index=1] {data/plt3_binary_linear_uniform.dat};
%\addlegendentry{binary-linear-uniform}

\addplot [
line width=1pt,
color=blue!80!black,
dotted
] table[x index=0,y index=1] {data/plt2_bound.dat};
%\addlegendentry{lower bound}

\end{axis}    
\end{tikzpicture}
\caption{}
\end{figure}



%Greedy takes exponential time in $K$ to compute.

%Simpler schemes: uniform, binary, interpolation between uniform and binary.


%Maybe state theorems about uniform and binary. Or maybe just mention them and refer to the longer version

\section{Proof of Main Result}

We now present the proof of Theorem \ref{thm:main_lower_bound}, which makes interesting use of convex optimization theory.  

\rdcomment{this may be similar to the IS comments, but this proof is a bit hard to read for me. i understand the first few paragraphs in words, but it is not trivial to me to see exactly how this formally changes the problem. i would suggest stating the problem, and then how the support-constraint changes the optimization, and so on. to be honest, if you're tight on space, i still think it would be more beneficial to dedicate more space to this `reduction' and then even leave some of the more mechanical parts of derivatives/KKT condition analysis out.

also, we arrived at this result through figures and drawings; can we add some of this into the proof? i think it would strengthen the appeal of this paper to hint at why the idea is actually intuitive and cute. as written, it feels more a set of mechanical manipulations of KKT conditions, and it loses the sort of elegance i typically associate with info theory papers. (this is not a comment on the result, it's just a comment on the presentation and how it makes me feel.) i really liked the drawings of the convolution of discrete measures, and how we're really chosing a measure that gets shifted to the left by 1 and rescaled by 1-p and shifted to the right by 1 and rescaled by p. can this be put in this section at all?}
\begin{IEEEproof}
	Let $ T = \sum_{i = 1}^K \alpha_i Z_i.$ We obtain the lower bound on $I(X \; ; \; X + T)= H(p) - H(X \; | \; X+T)$ in Theorem \ref{thm:main_lower_bound} by finding a lower bound on $-H(X \; | \; X+T).$  In order to lower bound $-H(X \; | \; X+T),$ we begin by considering the original optimization problem with the added constraint that the distance between the minimum support value and the maximum support value in the PMF of $T$ is less than $2n+2$ where $n \in \mathbb{N}, \; n > 0.$  We will obtain a lower bound for this support constrained optimization problem, and use it to obtain a lower bound on the original optimization problem.  
	\iscomment{unclear why this can be done}
	
	To lower bound the support constrained optimization problem, we work with a relaxation of the support constrained  optimization problem.  Instead of requiring that the PMF for $T$ be generated by adding the sum of scaled Bernoulli random variables, we relax the problem to only require that the probability at the highest support value of the PMF of $T$ is equal to $(1-p)^K$ (this holds for any valid PMF of $T$).  
	
	We then obtain a lower bound on this relaxation of the support constrained optimization problem .  Finally, we take the limit of the lower bound as $n$ goes to infinity in order to obtain an lower bound on the original minimization problem.
	
	The support-constrained relaxation of the original problem is given below where the objective function is a simplified form of $-H(X \; | \; X+D)$ where $D$ is the noise distribution we are optimizing over. Here, $q_{(0)}$ is the probability at the maximum support value of $T$ and $q_{(-i)}$ is the probability at the $i$th integer below the maximum support value of $T.$  Due to the fact that $X, Z_i \in \{-1, 1\},$ we have that all support values are separated by two or more in any valid PMF of $T.$  Observe that the problem is a convex minimization problem.
	\iscomment{not clear how this was obtained:}
	\begin{align}
	& \min_{q_{(-2n-2)}, \; ..., \;  q_{(0)}} \sum_{j \in \{-2n-2, \; ...,\;  -2\}} 
	\nonumber \\ & (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+2)}} \right) 
	\nonumber \\ & + p q_{(j+2)} \log \left(\frac{p q_{(j+2)}}{(1-p)q_{(j)} + p q_{(j+2)}} \right)    \\
	\nonumber \\ &  \text{subject to:} \quad  q_{(j)} \geq 0 \; \; \forall j,  \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad q_{(-2n-2)} = 0, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1. \nonumber
	\end{align}  
	
	\iscomment{do we need the full formula for the conditional entropy above? makes it harder to parse}
	While we cannot solve this problem analytically, we will perturb it to form an optimization problem that we can solve analytically.  We will then use perturbation analysis to obtain a lower bound on the problem above.
	
	
	The perturbed problem is given below where we have changed the constraint on the probability at the minimum support value, and the constraint on the sum of all the probabilities.
	
	\begin{align}
	& \min_{q_{(-2n-2)}, \; ..., \;  q_{(0)}} \sum_{j \in \{-2n-2, \; ...,\;  -2\}} 
	\nonumber \\ &  (1-p)q_{(j)} \log \left(\frac{(1-p)q_{(j)}}{(1-p)q_{(j)} + p q_{(j+2)}} \right) 
	\nonumber \\ & +  p q_{(j+2)} \log \left(\frac{p q_{(j+2)}}{(1-p)q_{(j)} + p q_{(j+2)}} \right)    \\
	\nonumber \\	&  \text{subject to:} \quad  q_{(j)} \geq 0 \; \; \forall j,  \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & \quad q_{(-2n-2)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ & \quad    \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2} \nonumber
	\end{align}  
	
	
	Let $f_0(q)$ be the objective function above.  The Lagrangian is given by 
	
	\begin{align} 
	&L(q, v, \lambda) = f_0(q) 
	\nonumber \\ & + v_1 \left(\sum_i q_{(i)} - 1 + (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & + v_2 \left(q_{(0)} - (1-p)^K \right) 
	\nonumber \\ & + v_3 \left(q_{(-2n-2)} - (1-p)^K (1 - (1-p)^K)^{n+1} \right) 
	\nonumber \\ & - \sum_i \lambda_i q_{(i)}. 
	\end{align}
	The derivative of $f_0(q)$ with respect to $q_{(j)}$ is given by 
	\begin{align}
	& p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-2)} + p q_{(j)}} \right) \nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+2)} + (1-p) q_{(j)}} \right).
	\end{align}  
	for $j \in \{-2n, \; ..., \;  -2\}$ and the KKT conditions are therefore given by 
	\begin{align}
	&  q_{(j)} \geq 0 \; \; \forall j,  \quad q_{(0)} = (1-p)^K, 
	\nonumber \\ & q_{(-2n-2)} = (1-p)^K (1 - (1-p)^K)^{n+1}, 
	\nonumber \\ &     \sum_{j} q_{(j)} = 1 - (1 - (1-p)^K)^{n+2}
	\nonumber \\ & \lambda_j \geq 0 \quad \lambda_j q_{(j)} = 0 \quad \forall j 
	\nonumber \\ & (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+2)} + (1-p) q_{(j)}} \right) - \lambda_j + v_1 + v_3 = 0 \quad 
	\nonumber \\ &  \text{for } j = - 2n -2
	\nonumber \\ & 	p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-2)} + p q_{(j)}} \right) 
	\nonumber \\ & + (1-p) \log \left( \frac{(1-p) q_{(j)}}{p q_{(j+2)} + (1-p) q_{(j)}} \right) - \lambda_j + v_1 = 0 
	\nonumber \\ &  \forall j \in \{-2n, \; ..., \;  -2\}
	\nonumber \\ & p \log \left(\frac{p q_{(j)}}{(1-p)q_{(j-2)} + p q_{(j)}} \right) - \lambda_j + v_1 + v_2 = 0 
	\nonumber \\ & \text{for } j = 0
	\end{align}
	
	\rdcomment{stupid question: can you tell me a little more why (12) is this derivative? at a glance, it seems to be that there's a ton of term cancellations... (it's like the terms inside the log don't depend on $q_j$ with the way the derivative is written, so all those terms cancel?) i fear that a unfastidious reviewer may just claim this is a fundamental error and give a poor review without analyzing it deeply. (this happens sometimes to me.)}
	
	The last three conditions can be rewritten as 
	\begin{align} 
	& (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+2)}}{q_{(j)}} + (1-p) } \right) - \lambda_j + v_1 + v_3 = 0  
	\nonumber \\ &  \text{for } j = - 2n - 2
	\nonumber \\ & p \log \left(\frac{p }{(1-p)\frac{q_{(j-2)}}{q_{(j)}} + p } \right) + (1-p) \log \left( \frac{(1-p) }{p \frac{q_{(j+2)}}{q_{(j)}} + (1-p) } \right) 
	\nonumber \\ & - \lambda_j + v_1  = 0 \quad \forall j \in \{-2n, \; ..., \;  -2\}
	\nonumber \\ & p \log \left(\frac{p }{(1-p) \frac{q_{(j-2)}}{q_{(j)}} + p } \right) - \lambda_j + v_1 + v_2  = 0 \quad \text{for } j = 0
	\end{align}
	which shows that if the ratio $\frac{q_{(j-2)}}{q_{(j)}}$ between consecutive variables is the same for all $j$ and $\lambda_j = 0 $ for all $j,$ then $v_1,$ $v_2$ can  be chosen so that of these derivatives equal $0$ for all $j.$  Picking \[\frac{q_{(j-2)}}{q_{(j)}} = (1 - (1-p)^K),\] a solution to these equations is then
	\begin{align}
	& q_{(-2i)} =  (1-p)^K (1 - (1-p)^K)^{i}  
	\nonumber \\ & \quad \quad \text{for } i \in \{0, \; 1, \; ..., \; n+1 \} 
	\nonumber \\ & \lambda_i = 0 \quad \forall i
	\nonumber \\ & v_1 = - p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & - (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right)
	\nonumber \\ & v_2 = (1-p)\log \left( \frac{(1-p)(1 - (1-p)^K)}{(1-p)(1 - (1-p)^K) + p} \right) 
	\nonumber \\ & v_3 = p \log \left( \frac{p}{(1-p)(1 - (1-p)^K) + p} \right)
	\end{align}
	
	Because this is a convex optimization problem, this solution is optimal since it satisfies the KKT conditions.
	
	The optimal value for the optimization problem is therefore given by 
	\begin{align} 
	& \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
	\\ & - p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	\\ & = \sum_{i = 0}^{n} -(1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\\ & - p \beta \alpha^i \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\end{align}
	where $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K.$  
	Applying the geometric sum formula and simplifying, we obtain 
	\begin{align} 
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right).
	\end{align}
	
	
	
	%The optimal value for the optimization problem is therefore given by 
	%\begin{align} 
	%& -(1-p) \beta \alpha \frac{1 - \alpha^{2n+2}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	%\nonumber \\ & - p \beta \frac{1 - \alpha^{2n+2}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right).
	%\end{align}
	%after some simplification.
	
	Using the perturbation analysis from Section 5.6.1 of \cite{boyd}, we see that the optimal value of the support constrained relaxation of the original problem is lower bounded by
	\begin{align}
	& -(1-p) \beta \alpha \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p) \alpha + p }{(1-p) \alpha} \right) 
	\nonumber \\ & - p \beta \frac{1 - \alpha^{n+1}}{1 - \alpha} \log \left( \frac{(1-p)  \alpha + p }{ p } \right)
	\nonumber \\ & - v_1^* \left( (1 - (1-p)^K)^{n+2} \right) 
	\nonumber \\ & - v_3^* \left(- (1-p)^K (1 - (1-p)^K)^{n+1}  \right) 
	\end{align} 
	where $v_1^*$ and $v_3^*$ are the optimal lagrange multipliers for the perturbed problem which we determined above through the KKT conditions.
	
	The sequence of optimal values returned by the support constrained relaxation of the original problem is monotonically decreasing in $n$ clearly.  Thus, taking the limit of the bound as  $n \to \infty$ and simplifying yields the following lower bound on $-H(X \; | \; X + T)$ for any choice of $\alpha_i$'s: 	\begin{align} 
	& -(p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right).
	\end{align}
	
	Thus, a lower bound on mutual information is
	\begin{align} 
	& H(p) - (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right) 
	\nonumber \\ & - p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
	\end{align}
	for any choice of $\alpha_i$'s.
	
	Finally, observe that
	\begin{align}
	& H(X \; ; \; X - 2G) 
	\nonumber \\ & =\sum_{i = 0}^{\infty} (1-p) \beta \alpha^{i+1} \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{(1-p) \beta \alpha^{i+1}} \right) 
	\nonumber \\ & + p \beta \alpha^i \log \left( \frac{(1-p) \beta \alpha^{i+1} + p \beta \alpha^i }{ p \beta \alpha^i} \right)
	\nonumber \\ & = (p-1) \left( (1-p)^K - 1\right) \log \left( \frac{(p-1)(1-p)^K + 1}{(p-1) \left( (1-p)^K -1 \right)}\right)  
	\nonumber \\ & + p \log \left( \frac{(p-1)(1-p)^K + 1}{p} \right)
	\end{align}
	where $G$ is a geometric random variable with success probability $(1-p)^K$ and support equal to $\mathbb{N} \cup \{0\},$  and $\alpha = (1 - (1-p)^K)$ and $\beta = (1-p)^K$ as before.
\end{IEEEproof}

==> preliminaries10_19_20.tex <==


% \section{Exhaustive Search} 

\section{Problem Setting and Preliminaries}

Our goal is to characterize the mixing proportions $\alpha_0,...,\alpha_K$ that minimize the mutual information in (\ref{eq:main}).
Notice that we 
% can assume $\alpha_0 = 1$ and 
do not need to constrain the mixing proportions to add up to $1$, since scaling the observation $Y$
% since scaling $X+Z_\alpha$ 
does not change the mutual information.
Furthermore, restricting $\alpha_0,...,\alpha_K$ to be positive rational numbers does not change the optimal value (as they can be chosen arbitrarily close to any irrational number).
Finally, we notice that a rational-valued solution $(\alpha_0,...,\alpha_K)$ can be converted onto an integer-valued one with the same value of \ref{eq:main} by scaling by the least common denominator.
% positive integers does not change the solution to (\ref{eq:main}).
% \kmcomment{I don't know how to show this.  This is the thing that we thought looked like additive combinatorics.  We only proved this is the case of the relaxation}
% We refer to the longer version of this paper \cite{long} for details.
As a result, we can restrict ourselves to solving the discrete optimization problem
\al{
\min_{\alpha \in \N^{K+1}} I(X;\alpha_0 X+Z_\alpha),
\label{eq:main2}
}
\kmcomment{I changed this to $\alpha \in \N^{K+1}$ throughout}
where $\alpha = (\alpha_0,...,\alpha_K)$, $Z_\alpha = \sum_{i=1}^K \alpha_i Z_i$, and $X,Z_1,...,Z_K$ are independent ${\rm Ber}(p)$ random variables.



The optimization problem in (\ref{eq:main2}) 
is surprisingly complex. 
The symmetry between the variables $\alpha_0,...,\alpha_K$ may  suggest that $\alpha_i = 1$ for $i=0,...,K$  \kmcomment{I changed this index to start from 0 throughout this section} would be an optimal solution.
However, a brute-force solution to (\ref{eq:main2}) for small values of $K$ shows that optimal solutions $(\alpha_0,...,\alpha_K)$ vary widely for different values of $p$,
% have little structure
% To gain some initial understanding of the problem, we begin by solving it using exhaustive search for small values of $K$ 
as illustrated in Figure \ref{fig:optimal_scheme_K5_minor_allele}.  
Observe that the curve appears to be only piecewise smooth. At $p = 0.5,$ the optimal solution is given by $[1,1,2,4,8,16],$ at $p=0.25,$ the optimal solution is given by $[1,1,1,2,3,4],$ and at $p = 0.01,$ the optimal solution is given by $[1,1,1,1,1,1]$.  
% These examples are representative of what is known about the problem: the optimal solutions are fixed and known at $p = 0.5$ and $p \to 0$ as discussed in Section IV, while the optimal solutions appear to have little structure for other values of $p.$ 



As it turns out, the optimal solution to (\ref{eq:main2}) can be exactly characterized in the two extremes cases of $p$.
More precisely, if we define the \emph{uniform} scheme to be 
$\alpha_i = 1$ for $i=0,...,K$,
and we define the \emph{binary} scheme to be $\alpha_0 = 1$ and $\alpha_i = 2^{i-1}$ for $i=1,...,K$,
we have the following result.
\begin{theorem}\label{thm:extremes}
Fix some $K \in \N$.
% For any $K \in \mathbb{N},$ 
Then there exists some $p^* > 0$ such that the uniform scheme is optimal for $p < p^*$.
Moreover, the binary scheme is optimal for $p=0.5$.
\end{theorem}
We prove these results in the longer version of this paper \cite{long}.
Aside from the cases $p = 0.5$ and $p \approx 0$, there does not appear to be a simple expression for the optimal solution $\alpha$. 

Throughout the paper we use $\N$ to denote the set of natural numbers excluding $0,$ $\N_0$ to denote the set of natural numbers including $0,$ and $[N]$ to denote the set of natural numbers in $\{1, 2, ...,  N\}$ for an integer $N.$
% at arbitrary $p$ in the range $0 < p < 0.5.$ 
\kmcomment{I changed all the $\alpha$ vectors to include $\alpha_0$}
\iscomment{we need to be a bit careful because the optimal vectors in Figure 2 do not include $\alpha_0$}
\iscomment{
To discuss if we have space: convolution of discrete measures, exponential complexity of brute-force search
}


\longversion{

Notice that Equation \ref{eq:main} behaves very differently from the case where $Z_i$ is Gaussian.  In the Gaussian case, each $\alpha_i$ would be chosen as large as possible for all $i \in [K].$  However in our problem, if $\alpha_i > 1$ for all $i \in [K],$ then   
\begin{align} 
& I(X \; ; \; X + \sum_{i=1}^{K} \alpha_i Z_i) 
\nonumber \\ & = H(X) - H(X | X + \sum_{i=1}^{K} \alpha_i Z_i) = H(X) 
\end{align}
i.e. the scheme does not hide $X$ at all.  Therefore, if $\alpha_0 = 1,$ the solution to Equation \ref{eq:main} must have $\alpha_i = 1$ for at least one $i \in [K].$ 

\rdcomment{i might advocate for a little more discussion here: perhaps talk about how convolution of measures for discrete distributions is fundamentally a different problem than convolutions of continuous measures for this reason. i'll defer to IS's opinion on this tho.}

}

\begin{figure}[t]
\centering

\tikzstyle{every pin}=[fill=white,
	draw=black,
	font=\footnotesize]
	
\begin{tikzpicture}[scale=0.8]
\begin{axis} 
[width=0.46\textwidth,
height=0.36\textwidth,
% title ={Optimal Scheme: $K = 5$},
ylabel = mutual information, 
xlabel = minor allele frequency ($p$),
ymax = .2,
yticklabel style={
  /pgf/number format/precision=3,
  /pgf/number format/fixed},
]

\addplot [
line width=1pt,
color=blue!80!black
] table[x index=0,y index=1] {data/plt1_optimal.dat};
\addlegendentry{optimal}

\node[coordinate,pin=right:{$[1,1,1,1,1,1]$}] 
		at (axis cs:.01, 0.0423605362433) {};

\node[coordinate,pin=right:{$[1,1,1,2,3,4]$}] 
		at (axis cs:.25, 0.0942663435378) {};

\node[coordinate,pin=left:{$[1,1,2,4,8,16]$}] 
		at (axis cs:.5, 0.03125) {};




\addplot [
line width=1pt,
color=red!80!black
] table[x index=0,y index=1] {data/plt1_uniform.dat};
\addlegendentry{uniform}


\end{axis}   

\end{tikzpicture}
\caption{
Optimal value of 
% $I(X;X+Z_\alpha)$
(\ref{eq:main2}) 
for $K=5$ and $p \in [0,0.5]$.
At $p = 0.5,$ the optimal scheme is $\alpha = [1,1,2,4,8,16].$  At $ p = 0.25,$ the optimal scheme is $\alpha = [1,1,1,2,3,4].$  At $p = 0.01,$ the optimal scheme is $\alpha = [1,1,1,1,1,1].$
\iscomment{modify $\alpha$s to include $\alpha_0$? mention uniform scheme in caption}
\iscomment{Also, it looks like uniform goes below optimal for small $p$?}
\kmcomment{I was missing the p=.01 data point in the uniform curve so it looked wrong.  I fixed it now.}
}
\label{fig:optimal_scheme_K5_minor_allele}
\end{figure}


%\begin{figure}
%	\centering
%	\includegraphics[width=0.9\linewidth]{optimal_scheme_K5_minor_allele}
%	\caption{At $p = 0.5,$ the optimal scheme is $[1,2,4,8,16].$  At $ p = 0.25,$ the optimal scheme is $[1,1,2,3,4].$  At $p = 0.01,$ the optimal scheme is $[1,1,1,1,1].$}
%	\label{fig:optimal_scheme_K5_minor_allele}
%\end{figure}


==> references.tex <==


\begin{thebibliography}{10}

\bibitem{astronomical}
Z.~D. Stephens, S.~Y. Lee, F.~Faghri, R.~H. Campbell, C.~Zhai, M.~J. Efron,
  R.~Iyer, M.~C. Schatz, S.~Sinha, and G.~E. Robinson, ``Big data: Astronomical
  or genomical?,'' {\em PLOS Biology}, vol.~13, pp.~1--11, 07 2015.

\bibitem{cad}
P.~van~der Harst and N.~Verweij, ``Identification of 64 novel genetic loci
  provides an expanded view on the genetic architecture of coronary artery
  disease,'' {\em Circulation research}, vol.~122, no.~3, pp.~433--443, 2018.

\bibitem{diabetes}
A.~Mahajan 
% D.~Taliun, M.~Thurner, N.~R. Robertson, J.~M. Torres, N.~W. Rayner,
%   A.~J. Payne, V.~Steinthorsdottir, R.~A. Scott, N.~Grarup, 
  {\em et~al.},
  ``Fine-mapping type 2 diabetes loci to single-variant resolution using
  high-density imputation and islet-specific epigenome maps,'' {\em Nature
  genetics}, vol.~50, no.~11, 2018.

\bibitem{alzheimer}
R.~S. Desikan
% , C.~C. Fan, Y.~Wang, A.~J. Schork, H.~J. Cabral, L.~A. Cupples,
%   W.~K. Thompson, L.~Besser, W.~A. Kukull, D.~Holland, 
  {\em et~al.}, ``Genetic
  assessment of age-associated alzheimer disease risk: Development and
  validation of a polygenic hazard score,'' {\em PLoS medicine}, vol.~14,
  no.~3, 2017.

\bibitem{cirulli_rare}
E.~T. Cirulli and D.~B. Goldstein, ``Uncovering the roles of rare variants in
  common disease through whole-genome sequencing,'' {\em Nature Reviews
  Genetics}, vol.~11, no.~6, pp.~415--425, 2010.

\bibitem{diseaserisk}
W.~D. Hall, K.~I. Morley, and J.~C. Lucke, ``The prediction of disease risk in
  genomic medicine: Scientific prospects and implications for public policy and
  ethics,'' {\em EMBO reports}, vol.~5, no.~S1, pp.~S22--S26, 2004.

\bibitem{directtoconsumer}
S.~Hogarth, G.~Javitt, and D.~Melzer, ``The current landscape for
  direct-to-consumer genetic testing: legal, ethical, and policy issues,'' {\em
  Annu. Rev. Genomics Hum. Genet.}, vol.~9, pp.~161--182, 2008.

\bibitem{directtoconsumer2}
M.~A. Allyse, D.~H. Robinson, M.~J. Ferber, and R.~R. Sharp,
  ``Direct-to-consumer testing 2.0: emerging models of direct-to-consumer
  genetic testing,'' {\em Mayo Clinic Proceedings}, vol.~93, no.~1,
  pp.~113--120, 2018.

\bibitem{erlich}
Y.~Erlich and A.~Narayanan, ``Routes for breaching and protecting genetic
  privacy,'' {\em Nature Reviews Genetics}, vol.~15, no.~6, 2014.

\bibitem{23andmepharma}
N.~Martin, ``How {{DNA}} {Companies} {Like} {Ancestry} {And} {23andMe} {Are}
  {Using} {Your} {Genetic} {Data},'' {\em Forbes}, Dec. 2018.
% \newblock URL:
%   https://www.forbes.com/sites/nicolemartin1/2018/12/05/how-dna-companies-like-ancestry-and-23andme-are-using-your-genetic-data/.

\bibitem{Maddah-Ali}
A.~Gholami, M.~A. Maddah-Ali, and S.~A. Motahari, ``Private shotgun {{DNA}}
  sequencing,'' in {\em 2019 IEEE International Symposium on Information Theory
  (ISIT)}, pp.~171--175, IEEE, 2019.

\bibitem{Maddah-Ali2}
A.~Gholami, M.~A. Maddah-Ali, and S.~A. Motahari, ``Private shotgun {{DNA}}
  sequencing: A structured approach,'' in {\em 2019 Iran Workshop on
  Communication and Information Theory (IWCIT)}, pp.~1--6, IEEE, 2019.

\bibitem{Casci}
T. Casci, ``SNPs that come in threes.'' Nature Reviews Genetics, vol. 11, no. 8, 2010.

\bibitem{brca2}
R.~Wooster
% , G.~Bignell, J.~Lancaster, S.~Swift, S.~Seal, J.~Mangion,
%   N.~Collins, S.~Gregory, C.~Gumbs, G.~Micklem, 
  {\em et~al.}, ``Identification
  of the breast cancer susceptibility gene BRCA2,'' {\em Nature}, vol.~378, 
%   no.~6559, pp.~789--792, 
  1995.

\bibitem{nextgen}
S.~C. Schuster, ``Next-generation sequencing transforms today's biology,'' {\em
  Nature methods}, vol.~5, no.~1, pp.~16--18, 2008.

% \bibitem{privateDNAlong}
% K.~Mazooji, R.~Dong, and I.~Shomorony, ``Private {{DNA}} sequencing: Hiding
%   information in discrete noise,'' {\em available at
%   https://ilanshom.github.io/papers/private.pdf}.

\bibitem{boyd}
S.~Boyd and L.~Vandenberghe, {\em Convex Optimization}.
\newblock Cambridge: Cambridge University Press, 2004.

\end{thebibliography}

==> story.tex <==
\begin{description}
% 	\item[$\bullet$] Use of DNA is changing medicine and technology 
% 	\item[$\bullet$] DNA can tell people about their health and what illnesses they are susceptible to  
% 	\item[$\bullet$] However, people are concerned about the privacy of their DNA
	\item[$\bullet$] Introduce necessary DNA terminology and background: nucleotide, major/minor allele, SNP, sequencing process, fragment, read, sequencing machine
	\item[$\bullet$] One framework for keeping DNA private during sequencing process when not in possession of a sequencing machine is given by Maddah-Ali. Work was published at ISIT 2019.
	\item[$\bullet$] Explain Maddah-Ali's solution at high level like in abstract
	\item[$\bullet$] They design a scheme that keeps the mutual information between the reads and the SNP values of all the unknown individuals in the mixture below a threshold:
	\begin{align}
		\frac{I(X_{m,n}, m \in A^{(s)}, n \in [N]; \; R^{(s)})}{|A^{(s)}| N} \leq \beta
	\end{align}
	where $R^{(s)}$ is the set of reads sent to the sequencer $s,$ and $A^{(s)}$ is the set of unknown individuals sent to the sequencer $s,$ and $N$ is the number of SNPs, and $X_{m, n}$ is the $n$th SNP of unknown individual $m$ ($X_{m, n} = 1$ if major allele, $X_{m, n} = -1 $ if minor allele)
	\item[$\bullet$]  To satisfy the condition above, they design a scheme where sequencer $s$ receives a mixture of individuals' DNA where all included individuals are in equal proportion in the mixture
	\item[$\bullet$] Their protocol is called the all-but-one scheme.  It uses $M \geq 2$ third party sequencers that can't communicate to sequence $M$ unknown individuals. It sends all unknown individuals except unknown individual $i$ to sequencer $i.$  All individuals (known and unknown) sent to sequencer $i$ are in equal proportion in the mixture
	\item[$\bullet$] Given a set of reads for the SNP of interest, there is a bijective mapping between $\sum_{i \in A^{(s)}} X_{i, n} + \sum_{k \in [K]} Y_{k, n})$ and the number of reads present in the mixture that contain the major allele for SNP $n$ where $Y_{k,n}$ is the $n$th SNP of the $k$th known individual ($Y_{k, n} = 1$ if major allele, $Y_{k, n} = -1 $ if minor allele)
	\item[$\bullet$] They then show that the all-but-one scheme satisfies the privacy condition if 
	\begin{align}
		& \frac{I(X_{m, n}, m \in A^{(s)} ; \sum_{i \in A^{(s)}} X_{i, n} + \sum_{k \in [K]} Y_{k, n})}{M-1} 
		\nonumber \\ &  
		= \frac{H(Bin(M-1+K, p_n)) - H(Bin(K, p_n))}{M-1} \leq \beta
	\end{align}
	where $p_n$ is the major allele probability
	\item[$\bullet$] This is saying that the mutual information  for each SNP position normalized by the number of unknown individuals sent to a sequencer is upper bounded by $\beta,$ assuming no noise in the reading phase. That is why it is a sufficient condition (it is an upper bound on the mutual information assuming noisy reads).
	\item[$\bullet$] Their result shows that they can and add known individuals to guarantee desired privacy, and increase coverage depth in order to guarantee level of SNP reconstruction.
	%\item[$\bullet$] Emphasize: For each sequencer, there is an equal proportion of all included individuals in the mixture.
	\item[$\bullet$] The simplest version of their problem is when there are $2$ sequencers, and one unknown individual is sent to each sequencer:
	\begin{align}
	& I(X_{m, n}, m \in A^{(s)} ; \sum_{i \in A^{(s)}} X_{i, n} + \sum_{k \in [K]} Y_{k, n}) \leq \beta
	\end{align} is the sufficient condition for the privacy condition to hold for each of the two sequencers
	\item[$\bullet$] Re-emphaize: In their paper the sufficient condition for their privacy to hold is that the maximum mutual information over all SNPs is less than their privacy parameter $\beta.$  They use a scheme that uses same proportion of all individuals in a mixture in order to get results.
	\item[$\bullet$]  In practice, we are mostly concerned about the privacy of particular SNPs that could predict sensitive information about an individual	
	\item[$\bullet$] In this paper, we ask how we can minimize the mutual information $I(X ; X + \sum_{k \in [K]} \alpha_k Y_{k})$ for a particular SNP by varying the proportion $\alpha_k$ of each individual in the mixture.
	\begin{align} \label{eq:opt_problem} 
		\min_{\alpha_k \; : \; k \in [K]} I(X ; X + \sum_{k \in [K]} \alpha_k Y_{k})
	\end{align}
	\item[$\bullet$]  This analysis is applicable to maximizing the privacy of a particularly sensitive SNP (or group of sensitive SNPs with a particular minor allele probability).  
	\item[$\bullet$] This analysis is immediately applicable to the all-but-one scheme with $M=2,$  or equivalently, the scheme where there is only one unknown individual and one sequencer.
	\item[$\bullet$] These results give us an understanding of what is possible for each SNP minor allele probability, which is the natural information theoretic question that arises from Maddah-Ali's problem setup. 
	\item[$\bullet$] This is a fundamental information theoretic problem: we are simply asking how  to pick the coefficients of each Bernoulli random variable to hide a Bernoulli random variable of interest.  In other words, how can best design the noise?
	\item[$\bullet$] This is a hard discrete optimization problem. brute force search is not feasible because support size of noise could be exponential in $K$ (e.g. it is exponential for optimal scheme at $p = 0.5)$
	\item[$\bullet$] We can see there is a lot of richness in optimal schemes as $p$ varies after looking at solutions returned by brute force for small $K.$  Uniform scheme is optimal as $p \to 0,$ and binary scheme is optimal for $p = 0.5,$ but in between the optimal solution does not appear to have any clear pattern in general
	\item[$\bullet$]  Because this problem is so hard to approach, we aim to find an approximate solution.  To do this, we relax it to form a convex optimization problem and find a lower bound on the relaxation.  This lower bound ends up being the mutual information when the noise is a geometric random variable with a particular success probability parameter.   
	\item[$\bullet$] The mutual information using this geometric random variable appears to be a good approximation to the original problem because it is observed that the Bernoulli coefficients chosen by a greedy algorithm gives a very similar mutual information 
	\item[$\bullet$] 
	To show that the mutual information with geometric noise is a lower bound, we find a closed form solution to a perturbation of the relaxed optimization problem, then use perturbation analysis to show that it is a lower bound on the unperturbed relaxation
	\item[$\bullet$]It is interesting that the geometric distribution plays this role in our problem, because the geometric distribution is also the maximum entropy distribution when the support is constrained to be a subset of the natural numbers and the mean is constrained.  
	\item[$\bullet$]  Use of Geometric distribution for $T$ is in sharp contrast with Maddah-Ali's use of the uniform scheme which gives Binomial distribution for $T$ (Approximated by Gaussian).
	
	
	%\item[$\bullet$] Mention that we have asymptotic results comparing bound to uniform  scheme for certain parameter regimes, and that we have polynomial time algorithms (exp-lin-const) for computing schemes as well (greedy algorithm is not polynomial time)
\end{description}
